Automated Verification of CountDownLatch

The CountDownLatch (CDL) is a versatile concurrency mechanism that was first introduced in Java 5, and is also being adopted into C++ and C#. Its usage allows one or more threads to exchange resources and synchronize by waiting for some tasks to be completed before others can proceed. In this paper, we propose a new framework for verifying the correctness of concurrent applications that use CDLs. Our framework is built on top of two existing mechanisms, concurrent abstract predicate and fictional separation logic, with some enhancements such as borrowed heap and thread local abstraction. In addition, we propose a new inconsistency detection mechanism based on waits-for relation to guarantee deadlock freedom. Prior concurrency verification works have mostly focused on data-race freedom. As a practical proof of concept, we have implemented this new specification and verification mechanism for CDL in a new tool, called HIPCAP, on top of an existing HIP verifier. We have used this new tool to successfully verify various use cases for CDL.

==> 2macros.tex <==
%\usepackage{times,epsfig,color,latexsym,clrscode3e}
\usepackage{amsmath,amssymb,bm,mathtools}

\usepackage{relsize} %to make math symbols bigger/smaller

\usepackage{frameit,color,latexsym,graphics,wrapfig}
\usepackage{listings}
\usepackage{multirow}
\usepackage{lineno,amsthm}

%\usepackage{lgrind,proof}
%\usepackage{lineno}
%\usepackage{listings}
%\usepackage{multirow}
%\usepackage{amssymb}
\usepackage{graphicx}

\usepackage{xspace}

\usepackage{framed,color} %% for shaded

%\usepackage{hanging} %% for hangparas

\newcommand{\ptto}[3]{\ensuremath{{\btt{#1}}\,{\mapsto}\,{\btt{#2}}{\langle}{\btt{#3}}{\rangle}}}

%first-order logic predicates
\newcommand{\fopred}[2]{\ensuremath{{\btt{#1}}{({#2})}}}
\newcommand{\pred}[2]{\ensuremath{{\btt{#1}}{\langle}{#2}{\rangle}}}

\newcommand{\rpreds}[2]{\ensuremath{\btt{#1}({#2})}}
\newcommand{\rpredl}[3]{\ensuremath{\btt{#1}[{#2}]({#3})}} %% resource predicates: name[w*](v,P*,v*)

%\newcommand{\predf}[3]{\ensuremath{{\btt{#1}}
%( {\btt{#3}} )
%{\langle}{\btt{#2}}{\rangle}}}

\newcommand{\predf}[3]{\ensuremath{{#1}( {#3} ){\langle}{#2}{\rangle}}}
\newcommand{\predfI}[4]{\ensuremath{{#1}( {#3} ){\langle}{#2}{\rangle}@{#4}}}

%optional fractional permission
\newcommand{\predfo}[3]{\ensuremath{{#1}{[(#3)]}{\langle}{#2}{\rangle}}}
%\newcommand{\view}[2]{\ensuremath{\btt{#1}{\langle}{#2}{\rangle}}} % view=pred
\newcommand{\view}[2]{\pred{#1}{#2}}
\newcommand{\viewf}[3]{\pred{#1}{#2}{#3}}

\newcommand{\predt}{\ensuremath{\epsilon}}

\newcommand{\nil}{\btt{null}}

\def\sep{~\code{*}~}
\newcommand{\usep}[1]{\ensuremath{~\code{*}_{\{#1\}}~}} % compose and update

\newcommand{\codes}[1]{{{\scriptsize {\ensuremath{\tt #1}}}}} %small size
%\newcommand{\code}[1]{{{\ensuremath{\tt #1}}}}
\newcommand{\sm}[1]{\mbox{$#1$}}
\newcommand{\btt}[1]{{\ensuremath{\tt #1}}}
\newcommand{\emp}{\btt{emp}}
\newcommand{\failure}{\btt{FAIL}}
%\newcommand{\true}{\btt{true}}
\newcommand{\emps}{\btt{emp_s}}
\newcommand{\empt}{\btt{emp_t}}
\newcommand{\hoares}[1]{{{\scriptsize{\ensuremath{\textit {#1}}}}}} %small size
\newcommand{\hoare}[1]{{\ensuremath{\textit #1}}}
%\newcommand{\hoare2}[1]{{\scriptsize{\ensuremath{\textit #1}}}
%\newcommand{\hoare}[1]{}

\newcommand\nonterm[1]{\textit{#1}}
\newcommand\term[1]{\textit{#1}}
%\newcommand\term[1]{\code{#1}}
\newcommand\lit[1]{{\bf #1}}

\newcommand{\constr}{\ensuremath{\Phi}}

\def\pre{\constr_{\myit{pr}}}
\def\post{\constr_{\myit{po}}}

\newcommand{\requires}{\ensuremath{\code{requires}}}
\newcommand{\ensures}{\ensuremath{\code{ensures}}}
\newcommand{\res}{\ensuremath{\code{res}}}

\def\D{\Delta}

\newcommand{\myit}[1]{\textit{#1}}
\def\map{\myit{X{\!}Pure}}
\def\invmap{\myit{Inv}}

\def\ex{{\bf ex}}

\def\fresh{\myit{fresh}}
\def\unfold{\myit{unfold}}

\newcommand\V[1]{\ensuremath{\overrightarrow{#1}}}

%\newcommand{\self}{\btt{root}}
\newcommand{\self}{\btt{self}}
\newcommand{\veq}{\ensuremath{\equiv}}
\newcommand{\pure}{\ensuremath{\pi}}
\newcommand{\heap}{\ensuremath{\kappa}}
\newcommand{\ptr}{\ensuremath{\gamma}}
%\newcommand{\pconstr}{\ensuremath{\phi}} 
\newcommand{\pconstr}{\ensuremath{\pi}} 
\newcommand{\vperm}{\ensuremath{\nu}} 

\newcommand{\invf}[1]{\ensuremath{{1.0 {\geq} {#1} {>} 0.0}}}

\newcommand{\aheap}{\ensuremath{\iota}} % atomic heap
\newcommand{\arith}{\ensuremath{\alpha}}
\newcommand{\mset}{\ensuremath{\beta}}
\newcommand{\aterm}{\ensuremath{\alpha^t}}
\newcommand{\mterm}{\ensuremath{\beta^t}}

\newcommand{\mustset}{\ensuremath{M{\!}U{\!}S{\!}T}}
\newcommand{\mayset}{\ensuremath{M{\!}A{\!}Y}}
\newcommand{\empset}{\ensuremath{\{\}}}
\newcommand{\set}[1]{\ensuremath{\{#1\}}}



\newcommand{\own}[1]{\hoare{Own(\ensuremath{#1})}}% own(v,f)

%\newcommand{\fracperm}{\ensuremath{\pi}}
\newcommand{\fracperm}{\btt{\varepsilon}} %% 0<fracperm<1
\newcommand{\fracpermc}{\btt{\xi}} %% 0<fracperm<=1
\newcommand{\baseperm}{\btt{\beta}}
%\newcommand{\partperm}{\ensuremath{\boldsymbol{\varepsilon}}}
\newcommand{\partperm}{\ensuremath{\mathlarger{\mathlarger{\mathlarger{\varepsilon}}}}}
\newcommand{\permset}{\ensuremath{\Pi}}
\newcommand{\permsetemp}{\empset}
%\newcommand{\perm}[1]{\ensuremath{\pi(#1)}}
\newcommand{\perm}[1]{\ensuremath{(#1)}}

\newcommand{\entailS}[2]{\ensuremath{#1 \vdash #2}}
\newcommand{\entailH}[3]{\ensuremath{#1 \vdash #2 \sep #3}}

\newcommand{\entailW}[3]{\ensuremath{#1 \vdash_\omega #2 \Rightarrow  #3}}
\newcommand{\entail}[3]{\ensuremath{#1 \vdash #2 \Rightarrow  #3}}
\newcommand{\entailK}[5]{\ensuremath{#3 \vdash^{#1}_{#2}#4 \sep #5}}
\newcommand{\entailVV}[3]{\entailK{\heap}{V}{#1}{#2}{#3}}

\newcommand{\hc}[2]{\ensuremath{{#1}{::}#2}}
%\newcommand{\defs}{\stackrel{\text{\ensuremath{\Delta}}}{=}}
\newcommand{\defs}{\stackrel{\text{\ensuremath{\texttt{def}}}}{=}}


\newcommand{\hform}[3]{\ensuremath{{{#1}}{::}{{#2}}{\langle}{{#3}}{\rangle}}}
\newcommand{\hformf}[4]{\ensuremath{{{#1}}{::}{{#2}}{{(#4)}}{\langle}{{#3}}{\rangle}}}

\newcommand{\rulen}[1]{\ensuremath{{\bf \scriptstyle #1}}}
\newcommand{\entrulen}[1]{\underline{{\bf \rulen{#1}}}}
%\newcommand{\entrulen}[1]{}
\newcommand{\comment}{//}
%\newcommand{\comment}{}
%\textbackslash\textbackslash} % comment operator

\newcommand{\wwith}{{\bf inv}}

\def\foldK{\myit{fold}^{\heap}}
\newcommand{\foldKI}[1]{\myit{fold}^{#1}}

\newcommand{\foldKII}[2]{\myit{fold}^{#1}_{#2}}

\def\foldL{\myit{foldL}^{\heap}}
\newcommand{\foldLI}[1]{\myit{foldL}^{#1}}

\def\bagsubsume {\sqsubset}
\def\bagsubsumeeq {\sqsubseteq}
\def\bag{{\cal B}}
\def\bagunion{\cup}
\def\bagintersect{\cap}
%\def\bagunion{\sqcup}
%\def\bagintersect{\sqcap}
\def\bagsubsume {\sqsubset}
\def\bagsubtract{{-}}
\def\zerobag{\{{\bf 0}\}}
\newcommand{\compose}[1]{{\circ}_{ \{ {#1} \}}}
\newcommand{\composeS}[1]{{\circ}_{#1} }

\newcommand{\tick}{\ding{51}}
\newcommand{\cross}{\ding{55}}

\newcommand{\fv}[1]{FV({#1})}
\newcommand{\modifies}[1]{modifies({#1})}

\newcommand{\full}[1]{{@}{\it full}[{#1}]}
\newcommand{\val}[1]{{@}value[{#1}]}
\newcommand{\zero}[1]{{@}zero[{#1}]}
\newcommand{\half}[1]{{@}half[{#1}]}
\newcommand{\myspace}{\hspace{10pt}}
\newcommand{\mylspace}{\hspace{5pt}} % less space
\newcommand{\myvspace}{\hspace{1pt}} %very small space

\newcommand{\fork}{fork}
\newcommand{\join}{join}
\newcommand{\mthreadf}{\ensuremath{\mu}} % main thread
%% \newcommand{\cthreadf}{\ensuremath{\tau}} % child thread %%not used, to avoid colliion with tid
\newcommand{\locklevelf}{\ensuremath{\ell}}
\newcommand{\lockf}{\ensuremath{\ell}}
\newcommand{\alocklevel}{\ensuremath{\nu}}
\newcommand{\waitlevelf}{\ensuremath{\omega}}
\newcommand{\awaitlevel}{\lit{waitlevel}}
\newcommand{\locksetf}{\ensuremath{\psi}}
\newcommand{\alockset}{\lit{LS}}
\newcommand{\levelof}[1]{#1.mu}

\newcommand{\primed}[1]{isPrimed({#1})}

\newtheorem{thm}{Theorem}
\newtheorem{lmm}{Lemma}
\newtheorem{mydef}{Definition}
\newtheorem{cor}[thm]{Corollary}
%\newtheorem*{proof}{Proof}
%\newtheorem{example}[thm]{Example}

\def\rewrite{\leadsto}
\def\vfull{{\it @full}}
\def\vvalue{{\it @value}}
\def\vfail{{\it fail}}
\def\pre{\ensuremath{\constr_{pr}}}
\def\post{\ensuremath{\constr_{po}}}
\def\newpre{$\constr'_{pr}$}
\def\newpost{$\constr'_{po}$}
\def\vref{V_{ref}}
\def\vval{V_{val}}
\def\vmod{V_{m}}
\def\vfull{V_{full}}
\def\vpre{V_{pre}}
\def\vpost{V_{post}}

\newcommand{\verirulen}[1]{[\underline{{\bf \scriptstyle}\rulen{#1}}]}
\newcommand{\hlr}[3]{\ensuremath{\frac{\begin{array}{c}\verirulen{#1}\\[0.5ex]%[\underline{\rulen{#1}}]\\[0.5ex]
#2\end{array}}{\begin{array}{c}#3\end{array}}}}
\newcommand{\hlrs}[2]{\ensuremath{\begin{array}{c}\verirulen {#1} \\ #2\end{array}}}
\newcommand{\mysplit}[1]{\myit{split}(#1)}
\def\trans{\ensuremath{\hookrightarrow}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%>
%Taken from http://ownership-immutability.googlecode.com/svn-history/r76/trunk/oigj-paper-sources-in-tex/commands.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%>

\newcommand{\typerule}[2]{
\begin{array}{c}
  #1 \\
\hline
  #2
\end{array}}

\newcommand{\simplerule}[1]{
\begin{array}{c}
  #1
\end{array}}

% \small \footnotesize \scriptsize \tiny
% \codesize and \scriptsize seem to do the same thing.
% \newcommand{\code}[1]{\texttt{\textup{\footnotesize #1}}}
% \newcommand{\code}[1]{\texttt{\textup{\codesize #1}}}
\newcommand{\normalcode}[1]{\texttt{\textup{#1}}}
\def\codesmaller{\small}
\newcommand{\myCOMMENT}[1]{\COMMENT{\small #1}}
\newcommand{\code}[1]{\texttt{\textup{\codesmaller #1}}}

\newcommand\mynewcommand[2]{\newcommand{#1}{#2\xspace}}

\mynewcommand{\hA}{\code{A}} % inVariant definition
\mynewcommand{\hB}{\code{B}} % inVariant definition

\mynewcommand{\hI}{\code{I}} % iparam

% In the syntax: \hI or ReadOnly or Mutable or Immut
\mynewcommand{\hJ}{\code{J}}
\mynewcommand{\hO}{\code{O}}
\mynewcommand{\ho}{\code{o}}

\mynewcommand{\hX}{\code{X}} % vars
\mynewcommand{\hY}{\code{Y}} % vars
%\mynewcommand{\hC}{\code{C}} % class
%\mynewcommand{\hc}{\code{c}} % cooker
\mynewcommand{\hL}{\code{L}} % class decl
\mynewcommand{\hM}{\code{M}} % Method decl
\mynewcommand{\hN}{\code{N}} % Non-variable type
%\mynewcommand{\hm}{\code{m}} % method
\mynewcommand{\he}{\code{e}} % expression
\mynewcommand{\hv}{\code{v}} % value
\mynewcommand{\hl}{\code{l}} % location in the store
\mynewcommand{\lroot}{\code{l}_\top} % root
\mynewcommand{\lthis}{\code{l}_\smallcode{this}} % this
\mynewcommand{\hx}{\code{x}} % method parameter
\mynewcommand{\hf}{\code{f}} % field
\mynewcommand{\hF}{\code{F}} % types (vars or non vars) of a field
\mynewcommand{\hT}{\code{T}} % types (vars or non vars)
\mynewcommand{\hU}{\code{U}} % types (vars or non vars)
\mynewcommand{\hV}{\code{V}} % closed types
\mynewcommand{\hH}{\code{H}} % Heap
\mynewcommand{\hS}{\code{S}}
\mynewcommand{\hsub}{\code{/}} % substitute (reduction rules)
\mynewcommand{\hthis}{\code{this}} % this
\mynewcommand{\hclass}{\code{class}}
\mynewcommand{\hreturn}{\code{return}}
\mynewcommand{\hnew}{\code{new}}
\newcommand{\lt}{\code{<}}%{\mathop{\textrm{\tt <}}}
\newcommand{\gt}{\code{>}}%{\mathop{\textrm{\tt >}}}

\mynewcommand{\gap}{~ ~ ~ ~ ~ ~}


\mynewcommand{\st}{\ensuremath{\mathrel{{\leq}}}} %{\mathop{\textrm{\tt <:}}}

%\newcommand{\RULE}[1]{\textsc{\scriptsize{}#1}} %\RULEhape\scriptsize}
\newcommand{\RULE}[1]{\entrulen{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%<
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%<

\newcommand{\var}{v}
\newcommand{\vars}{V}
\newcommand{\locs}{L}
\newcommand{\loc}{l}
\newcommand{\procs}{P}
\newcommand{\proc}{p}
\newcommand{\stores}{M}
\newcommand{\mem}{\mu}
\newcommand{\intset}{\mathbb{Z}}

\newcommand{\myhalt}{\code{halt}}
\newcommand{\myskip}{\code{skip}}
%\newcommand{\assg}{\code{:=}}

\newcommand{\paren}[3]{\ensuremath{\langle {#1},{#2},{#3} \rangle}}
\newcommand{\step}{\ensuremath{\rightarrow_g}}
\newcommand{\stepwo}{\ensuremath{\rightarrow}} %step w/o g

\newcommand{\ptt}{\ensuremath{\mapsto}} %% points-to or maps-to
\newcommand{\pointer}[1]{\text{ptr(#1)}} %% pointer to #1 

\newcommand{\lpointer}[1]{\text{lptr(\ensuremath{#1})}} %% pointer to a lock #1 
\newcommand{\lock}{\ensuremath{\phi}}
\newcommand{\lset}[1]{ \ensuremath{ \{ #1 \} } } %% pointer to a lock #1 
\newcommand{\lockset}{\ensuremath{\Psi}}
\newcommand{\locks}{\ensuremath{\psi}}
\newcommand{\locksetemp}{\{ \}} %% empty lockset


\newcommand{\context}{\D}
\newcommand{\subst}{\sigma}

\newcommand{\tvmap}{\ensuremath{\phi}}
\newcommand{\Tvmap}{\ensuremath{\Phi}}

%\newcommand{\level}{\ensuremath{\mu}}
\newcommand{\level}{mu}

\newcommand{\ewedge}{\ensuremath{\#}} % exclusive wedge

\newcommand{\uwedge}[1]{\ensuremath{\wedge_{\{#1\}}}} % compose and update

%\newcommand{\eimply}[1]{\ensuremath{\#{\rightarrow}_{\{#1\}}}} % delayed-checking implification

%% \newcommand{\eimply}[1]{\ensuremath{{\rightarrow}_{\{#1\}}}} % delayed-checking implification
\newcommand{\eimply}[1]{\ensuremath{{\rightarrow}}} % delayed-checking implification, omit the list of parameters w*

\newcommand{\outline}{\textup{//}}

\newcommand{\saying}[1]{{\color{red}\textup{/*#1*/}}}

%% \newcommand{\wnsay}[1]{~{{\color{blue}({\bf WN:} \textit{#1}})}}
%% %\newcommand{\wnsay}[1]{}
%% \newcommand{\wnnay}[1]{}
\newcommand{\dksay}[1]{{{\color{red}{\bf DK:} \textit{#1}}}}
%\newcommand{\dksay}[1]{}
\newcommand{\dknay}[1]{}
\newcommand{\ymsay}[1]{{{\color{green}({\bf YM:} \textit{#1}})}}
\newcommand{\ymnay}[1]{}



\newcommand{\state}{\ensuremath{\sigma}}

\newcommand{\config}{\ensuremath{\Psi}}

\newcommand{\envir}{\ensuremath{\Gamma}}

\newcommand{\envirof}[1]{\ensuremath{\envir(#1)}}

\newcommand{\omape}{\ensuremath{\Omega}} %map object references to environment lists

\newcommand{\omapeof}[1]{\ensuremath{\omape(#1)}} %map object references to environment lists

\newcommand{\omapi}{\ensuremath{\kappa}} %map object references to integers

\newcommand{\omaplevel}{\ensuremath{L}} %map object references to integers

\newcommand{\omaplevelof}[1]{\omaplevel(#1)} %map object references to integers

\newcommand{\omapiof}[1]{\ensuremath{\omapi(#1)}} %map object references to integers

\newcommand{\threads}{\ensuremath{T}}

\newcommand{\ls}{\ensuremath{ls}}

\newcommand{\delayedls}{\ensuremath{\kappa}}

\newcommand{\delayedf}{\ensuremath{\gamma}}

\definecolor{Light}{gray}{.90}
\definecolor{Dark}{gray}{.78}

%\newcommand{\highlightd}[1]{\colorbox{Dark}{$\displaystyle #1$}} %highlight dark

\newcommand{\highlightd}[1]{\boxed{#1}} %highlight dark

\newcommand{\highlightl}[1]{\colorbox{Light}{$\displaystyle #1$}} % highlightr gray

%% \newcommand{\tid}{\ensuremath{\iota}} % child thread
\newcommand{\tid}{\ensuremath{\tau}} % child thread

\newcommand{\mytick}{\small \tick} 
\newcommand{\mycross}{\small \cross}

%% #1 points to #2 with permission #3
\newcommand{\permsto}[3]{{\ensuremath{{#1}\,{\xmapsto{#3}{#2}}}}}

\newcommand{\barriernophase}{ \ensuremath{ \mathsf{ barrier{(}{)} } } }

\newcommand{\barrier}[1]{ \ensuremath{ \mathsf{ barrier{(} } #1 \mathsf{ {)} } } }

\newcommand{\thread}[1]{ \ensuremath{ \mathsf{ thrd{\langle} } #1 \mathsf{ {\rangle} } } }

\newcommand{\dead}[1]{\ensuremath{\btt{dead}(#1)}}

\newcommand{\localmap}{\ensuremath{L}} %map barriers to local phases


\newcommand{\globalmap}{\ensuremath{G}} %map barriers to numbers of participants and global phases
\newcommand{\globalmapI}{\ensuremath{G_i}}

\newcommand{\localmapof}[1]{\ensuremath{\localmap(#1)}} 

\newcommand{\globalmapTof}[1]{\ensuremath{\globalmap_t(#1)}} 
\newcommand{\globalmapPof}[1]{\ensuremath{\globalmap_p(#1)}} 
\newcommand{\globalmapIof}[1]{\ensuremath{\globalmap_i(#1)}} 
\newcommand{\globalmapof}[1]{\ensuremath{\globalmap(#1)}}
 
\newcommand{\threadspec}{\ensuremath{\Theta}}

\newcommand{\RLess}{\em resource-less}
\newcommand{\RLoaded}{\em resource-loaded}
\newcommand{\RAmb}{\em resource-ambiguous}


==> abstract-old.tex <==
\begin{abstract}
In mainstream languages, threads are 
first-class in that they can be dynamically created,
stored in data structures, passed as parameters,
and returned from procedures.
However, existing verification systems support reasoning about
threads in a restricted way -- threads
are often represented by unique tokens
that can be neither split nor shared.
In this paper, we propose ``\myit{flow-aware}'' resource predicate,
a variant of concurrent abstract predicate,
to enable more expressive verification in support of first-class threads.
As a concurrent predicate, our flow-aware variant explicitly tracks
resources that flow into and out of its shared abstraction.
We show how resources of such a predicate can
be more flexibly split and transferred across procedure and 
thread boundaries.
While we were originally motivated by the need to support
first-class threads, our proposal for flow-aware
resource predicate is general.
We illustrate this by showing
how it can handle another popular concurrency
mechanism, known as \code{countDownLatch}. This mechanism is
very versatile, as it can be used
to mimic simple
barrier synchronization and
a variety of multicast communications.
We show how to use flow-aware predicate
to safely track both the \code{countDown} and 
\code{await} mechanisms, and their support for resource
exchanges. In the same vein, we show
how we can generalize
to hierarchical locking.
Lastly, we show the
soundness of our flow-aware resource predicates by proving
our code and specifications to be race-free,  deadlock-free
and resource-preserving (e.g. leak-free communication).
We have implemented flow-aware predicates in a tool, called {\toolname},
on top of an existing {\parahip} verifier.
Initial implementation efforts showed that
{\toolname} is more expressive,
whilst achieving comparable verification performance.

%\keywords{Deadlock, specification, verification, logic, concurrency, framework.}

\end{abstract}


==> app-3f-verify-proofs-w-perms.tex <==



\begin{verbatim}
   Latch(x,+P)  == ([x->0] -> P)
   Latch{f}(x,-P)  == DEC_f * -P * (x->m) & m>0no
   CNT{f,f2}(x,P) == DEC_f * {|x->n|}_f2 & m>=0  
                  \/ DEF_f * {|x->0|}_f2 * [i->0] & n=-1

Question : Do we need to track permission of thread-local resource?
      {|i->n|}


  CDL newCDL(n) with P
   requires n>0  
   ensures lc(res,+P) * lc{1}(res,-P) * CNT{1,1}(res,n)
   requires n=0  
   ensures  CNT{1,1}(res,-1)

 void countDown(CDL i) 
   requires lc{f1}(i,-P)*P*CNT{f2,f3}(i,n) & n>0
   ensures  CNT{f1+f2,f3}(i,n-1);
   requires CNT{f,f2}(i,-1) 
   ensures  CNT{f,f2}(i,-1);

  void await(i)
   requires lc(i,+P) * CNT{f,f2}(i,0) 
   ensures  P * CNT{f,f2}(i,-1);
   requires CNT{f,f2}(i,-1) 
   ensures  CNT{f,f2}(i,-1);

 shared2local(CDL c)
  requires CNT{1,1}(c,-1)
  ensures  c->CDL(0);
{
  # CNT{1,1}(c,-1)
  # DEC_1*[c->0]*{|c->0|}_1
  # DEC_1*KILL_1*[c->0]
  # c->CDL(0)
}


Splitting Lemma:
  lc(i,+P*Q) --> lc(i,+P)*lc(i,+Q) 
  lc{f1+f2}(i,-P*Q) --> lc{f1}(i,-P)*lc{f2}(i,-Q) 
  CNT{f1+f2,f3+f4}(i,n) & n1,n2>=0 & n=n1+n2 
      --> CNT{f1,f3}(i,n1)*CNT{f2,f4}(i,n2)

Normalization:
  CNT{f1,f2}(c,n) * CNT{f3,f4}(c,-1) & n<=0 
    ==> CNT{f1+f3,f2+f4a}(c,-1) // idempotent lemma 
  CNT{f1,f2}(c,n1) * CNT{f3,f4}(c,n2) & n=n1+n2 
    & n1,n2>=0 & n>=0  ==> CNT{f1+f3,f2+f4}(c,n)
  Latch(c,P) * CNT{f3,f4}(c,-1)  
    ==> %P * CNT{f3,f4}(c,-1)

Deadlock detection:
  CNT{_,_}(c,n) * CNT{_,_}(c,-1) & n>0  ==> DEADLOCK
  Latch{_}(c,-P) * CNT(c,-1)  ==> RACE-PROBLEM
\end{verbatim}


==> app-4-semantics.tex <==

The semantics of our separation heap formula is similar to the model given for separation logic
\cite{Reynolds:LICS02}, except that we have extensions to handle our
user-defined shape predicates.

To define the model we assume sets $\Locations$ of locations
(positive integer values), $\Val$ of primitive values, with $0
\in\Val$ denoting $\nil$, $\Var$ of variables (program and logical
variables), and \sm{\myit{ObjVal}} of object values stored in the
heap, with \sm{c[f_1{\mapsto}\nu_1,..,f_n{\mapsto}\nu_n]} denoting
an object value of data type \sm{c} where \sm{\nu_1,..,\nu_n} are
current values of the corresponding fields \sm{f_1,..,f_n}. Let
$\mo{s}{h}{\constr}$ denote the model relation, i.e. the stack $s$
and heap $h$ satisfy the constraint $\constr$, with $h,s$ from the
following concrete domains:
\[
\begin{array}{llllll}
h &\in~ \Store ~\defs& \Locations \rightharpoonup_{\myit{fin}} \myit{ObjVal}
%(\Flds \rightarrow \Val\,{\cup}\Locations)
&\qquad\qquad s &\in~ \Stack ~\defs& \Var \rightarrow \Val\,{\cup}\Locations
\end{array}
\]
%\\
Note that each heap \sm{h} is a finite partial mapping while each
stack \sm{s} is a total mapping, as in the classical separation
logic \cite{Reynolds:LICS02,Ishtiaq:POPL01}. Function $\dom(f)$
returns the domain of function $f$. Note that we use \sm{\mapsto} to
denote mappings, not the points-to assertion in separation logic,
which has been replaced by \hc{p}{\view{c}{v^*}} in our notation.
The model relation for separation heap formulas is defined below.
The model relation for pure formula \sm{s \models \pure}
%\sm{s \models_P \pure}
denotes that the formula \sm{\pure} evaluates to \sm{\true} in
\sm{s}.%, which is standard in classical logic and is omitted.
%
\begin{defn}\label{def.model}[Model for Separation Constraint]
\[
\begin{array}{ll}
\mos{\!\constr_1{\vee}\constr_2}  &\iffs \mos{\constr_1} ~\mbox{or}~ \mos{\constr_2}
\\
\mos{\!{\exists} v_{1..n} {\cdot} {\heap} {\wedge} \pure}   &\iffs
(\exists \nu_{1..n} {\cdot}
\mo{s[v_1{\mapsto}\nu_1,..,v_n{\mapsto}\nu_n]}{h}{{\heap}})
~\mbox{and}~
(s[v_1{\mapsto}\nu_1,..,v_n{\mapsto}\nu_n]\,{\mymodel}\,{\pure})
\\
%\mos{\exists v {\cdot}\constr} &\iffs v {\not\in}\dom(s),~\exists \nu \mo{\cdot s{+}\{v{\mapsto}\nu\}}{h}{\constr}
%\\
\mos{\!\heap_1{\sep}\heap_2}  &\iffs
\begin{array}[t]{l}
 \exists h_1,h_2 \cdot h_1 {\bot} h_2  ~\mbox{and}~
h=h_1{\cdot}h_2 ~\mbox{and}~\\
\mo{s}{h_1}{\heap_1}~\mbox{and}~\mo{s}{h_2}{\heap_2}
\end{array}
\\
\mos{\!\emp}  &\iffs \dom(h)=\emptyset
\\
\mos{\!\heap{\septract}\emp}  &\iffs
\exists h_1 \cdot h{\cdot}h_1=\emp ~\wedge~ \mo{s}{h_1}{\!\heap} 
%% \mos{\!\hc{p}{\view{c}{v_{1..n}}}} \hide{\hspace{-0.02in}\begin{array}[t]{l}
%% \mos{\hc{p}{\view{c}{v^*}}} \\
%% ~~c~is~a~data \end{array}}   &\iffs
%% \begin{array}[t]{l} \!\btt{data}~ c~{\{t_1\,f_1,..,t_n\,f_n\}} {\in}
%% {\myit{P}},~ \hide{s(p){>}0}%\\  \!% \!\mbox{and}~
%% h{=}[s(p) {\mapsto} r], \\  \mbox{and}~  r{=} c[f_1{\mapsto}s(v_1),..,f_n{\mapsto}s(v_n)]
%% \end{array}
%% \\
%% &\btt{or}~ (\view{c}{v_{1..n}}{\equiv}{\constr} ~\wwith~ \pi) {\in}
%% {\myit{P}} ~ \mbox{and}~ \mos{ [p{/}\self]{\constr}}
%% %
%% \hide{ \mos{\hc{p}{\view{c}{v^*}}} \hide{\hspace{-0.02in}\begin{array}[t]{l}
%% \mos{\hc{p}{\view{c}{v^*}}} \\
%% ~~c~is~a~view \end{array}}  &\iffs (\btt{view}~\view{c}{v^*}{\equiv}{ \constr}) \hide{~\wwith~
%% \pi} {\in} \myit{P} ~ \mbox{and}~ \mos{[p{/}\self]\,\constr} \hide{\quad
%% \mos{[\self{\mapsto}p]\,\pi} \quad p \in \dom(s)}}%
%% %
%% \\
%\mos{p_1 \oslash p_2} &\iffs \s{p_1} \oslash \s{p_2},~\mbox{where}~ \oslash{\in}\{=,\ne\}
\report{
%\mosp{p_1 \oslash p_2}  &\iffs s(p_1) \oslash s(p_2),~\mbox{where}~
%\oslash{\in}\{=,\ne\}
%\\
%\mosp{p \oslash \nil}  &\iffs s(p) \oslash 0,~\mbox{where}~ \oslash{\in}\{=,\ne\}
%\\
%\mosp{\pure}  &\iffs s \models_P \pure %hided on 6/3/2009
}
%\mosp{\pure_1 \wedge \pure_2}  &\iffs \mosp{\pure_1} ~\mbox{and}~ \mosp{\pure_2}
%\\
%\mosp{\phi}  &\iffs s \models_A \phi }
%\\
%\mosp{\neg \phi} &\iffs  s \not\mymodel \phi
\end{array}
\]
\end{defn}

\begin{verbatim}
How about LatchIn, LatchOut, Cnt

Do we need to model 
 thread-local {|i->n|}
 global       |i->m|

How is the semantics of fictional SL done.
Must we include some interpretation etc?
\end{verbatim}

%
Note that \sm{h_1{\bot}h_2} indicates \sm{h_1} and \sm{h_2} are
domain-disjoint, \sm{h_1{\cdot}h_2} denotes the union of disjoint
heaps \sm{h_1} and \sm{h_2}. The definition for
\sm{\mos{\hc{p}{\view{c}{v^*}}}} is split into two cases: (1) \sm{c}
is a data node defined in the program \sm{\myit{P}}; (2) \sm{c} is a
shape predicate defined in the program \sm{\myit{P}}. In the first
case, \sm{h} has to be a singleton heap. In the second case, the
shape predicate \sm{c} may be inductively defined.  Note  that the
semantics for an inductively defined shape predicate denotes the
least fixpoint, i.e., for the set of states (\sm{s,h}) satisfying
the predicate. The monotonic nature of our shape predicate
definition guarantees the existence of the descending chain of
unfoldings, thus the existence of the least solution.


\hide{
The heap abstraction \sm{\ex~i~{\cdot}~\beta ~|~
\bigvee(\exists v^*{\cdot}\pure)^*} given in last section has the
following model:
%
\begin{defn}[Model for Heap Approximation]
\[
\begin{array}{lll}
\!\!\mos{\!\!\bigvee (\exists v^*{\cdot}\pure)^*} &\iffs
\mosp{\bigvee(\exists v^*{\cdot}\pure)^*}
\\
\!\!\mos{\!\ex~i~{\cdot}~\beta} &\iffs
(p{=}i{\wedge}i{>}0){\in}\beta ~~\mbox{and}~~
\mo{s}{h{-}\{s(p)\}\!\!}{\!\![p/i]\beta}
\end{array}
\]
\end{defn}

Furthermore, we may soundly relate a separation formula \sm{\constr}
and its abstraction \sm{\beta} by the (semantic entailment) relation
\mos{\hmodels{\constr}{\beta}}, defined as follows :
%
\[
\forall
s,h\,{\cdot}\,(\hmodels{s,h}{\constr}\,{\implies}\,\hmodels{s,h}{\ex~i~{\cdot}~\beta ~|~
\bigvee(\exists v^*{\cdot}\pure)^*})
\]
}


==> applications.tex <==
%% \savesmallspace
\subsection{Verifying the Multi-join Pattern}
%% \savesmallspace

\wnsay{this section can be removed, and its ref moved to
related work}.

A program with multi-join pattern
allows a thread (joinee) to be shared and joined
in multiple threads (joiners). During the execution of the program,
the joiners wait for the joinee to finish its execution.
If joiners wait for an already-completed joinee, they proceed
immediately without waiting.
By joining with the joinee, the joiners expect
to receive certain resource transferred from the joinee.
The motivating program in Fig.~\ref{fig:mapreduce} is
an example of such a multi-join pattern.
The multi-join pattern also appears in the
context of asynchronous tasks.
For example, in C++11 (ISO/IEC 14882:2011),
a \code{shared\_future} task is designed to be shared between threads,
and to allow multiple concurrent get operations to wait
and obtain the shared result
after the asynchronous \code{shared\_future} task has finished its execution.
To the best of our knowledge, we are not aware
of a modular verification mechanism
%% any existing verification systems capable
%% of verifying the 
for the multi-join pattern.

As we have shown in previous sections, our approach
handles the multi-join pattern naturally.
%% One of the most important advantages of ``threads as resource''
%% is the ability to split and transfer threads' ownerships
%% to multiple joiners.
Our approach allows the ownership of the joinee to be split, shared, and joined
by multiple joiners, where each joiner obtains their corresponding
part of the joinee's resource upon join.
Although discussed in the context of fork/join programs,
``threads as resource'' can be
adapted to the context of asynchronous tasks
and to enable verification of programs
with concurrent get operations on \code{shared\_future} tasks as well.
For example, each  asynchronous \code{shared\_future} task
can be modeled as
%% (delayed)
resource (like threads),
and each get is similar to a join.

%% \input{appln-idiom}
%% \input{appln-liveness}
%% \input{lock}




==> appln-idiom.tex <==
\savespace
\subsection{Inductive Predicates and Threads as Resource}
\label{sec:predicate}
%% \savespace
\savesmallspace

\input{exp-shape}

%% \todo{Threads can be stored in data structures  and abstracted in shape predicates.}

Modeling threads as resource open opportunities for
applying current advances in separation logic,
which were originally designed for heap objects, to threads.
In this section, we describe how ``threads as resource''
together with inductive predicates~\cite{Gherghina:FM2011,Nguyen:VMCAI07}
can be used to naturally capture a commonly-used
programming idiom, called threadpool,
where threads are stored in data structures.

An example program is presented in Fig.~\ref{fig.shape}.
The program receives an input \code{n}, and then invokes \code{forkThreads} to
create \code{n} concurrent threads executing
the procedure \code{thread}.
For simplicity, we assume each thread will
have a read permission of the cell \code{x}
in the pre-condition and will return the read permission
in the post-condition.
The program will wait for all threads to finish their execution
by invoking \code{joinThreads}. At the end, as threads already
finished, it is safe to destroy the cell \code{x}.
In this program, each item in the threadpool
is a data structure of type \code{item}. Each \code{item}
will store a thread in its field \code{t}
and a pointer \code{next} to the next item
in the pool.
The \code{forkThreads} returns the first item
in the pool, while the \code{joinThreads}
receives the item and joins with all threads
in the pool.
In the program's specifications, ``\hoare{res}'' is used
to denote the returned result of a procedure and ``$\_$'' represents an unknown value.
%% tracking thread liveness is not the main focus and is omitted for brevity.

The key idea to verify this program is to use
an inductively defined predicate, called \code{pool} to abstract the threadpool.
As threads are modeled as resource, they can be naturally captured inside the predicate
in the same way as other heap resource, as follows:
\moresmallspace

\begin{small}
\noindent
\form{\code{pool(\self,x,n,M)} \defs \self{=}\code{null} \wedge \code{n{=}0} \wedge \code{M{>}0} }

\form{ \bigvee \exists \code{t,p} \cdot \permsto{\self}{\code{item(t,p)}}{} {\sep} {\color{blue} 
\thrdpredtwo{t}{\permsto{x}{\code{cell}(\textunderscore)}{\!{1/M}\!}{}}}}

%\permsto{t}{\thread{\permsto{x}{\code{cell}(\textunderscore)}{1/M}}{}}{} } }
\form{ {\sep} \code{pool(p,x,n{-}1,M)} }
\form{\qquad\textbf{inv}~\code{n}{\geq}\code{0} \wedge \code{M{>}0};}
\morespace
\end{small}

\noindent
The above predicate definition asserts that a \code{pool} can be empty
(the base case \code{\self{=}null})
or consists of a head item (specified by 
\code{\permsto{\self}{\code{item(t,p)}}{}}),
a thread node 
({\code{\color{blue} \thrdpredtwo{t}{\permsto{x}{\code{cell}(\textunderscore)}{\!{1/M}\!}{}} })
and a tail data structure which is also a \code{pool}.
The invariant \codeE{n{\geq}0 \wedge M{>}0} must hold for all
instances of the predicate.
Using the above definition and case analysis~\cite{Gherghina:FM2011},
the program can be verified
as functionally correct and data-race-free.
Although we use
%% a variant of 
linked lists here,
our approach easily adapts to other data structures,
such as arrays.
 %% to implement the threadpool.

\hide{
\subsection{Improving Delayed Lockset Checking}
\label{sec:delayed}

In previous sections, we described how ``threads as resource''
enhances the verification of functional correctness and data-race freedom of
concurrent programs. In this section,
we show how our ``threads as resource''
benefits the delayed
lockset checking (DLC) technique proposed in \cite{Le:ATVA13}.
More specifically, it makes the proof
more concise and natural, while it enables verifying
deadlock freedom of challenging programs
with non-lexically-scoped fork/join, locks, and multi-join.

The key idea of the DLC technique \cite{Le:ATVA13}
is that, for more expressive verification of
deadlock freedom,
lockset constraints in the precondition of a thread
are not checked at the fork point but are delayed
to be checked at the join points instead.
We can naturally support the technique
by extending our ``threads as resource'' to
additionally capture the delayed lockset constraints.
A thread node
\permsto{\term{v}}{ \thread{\delayedf ~ \eimply{w^*} ~ \constr} }{}
now additionally captures the delayed formula
$\delayedf$ which was delayed at a fork point and will be
checked at join point(s).
We present a set of sub-structural rules for a
thread node with a delayed formula, and enable
the thread node to be flexibly split and transferred.
Our improvement ensures
deadlock freedom of programs
with non-lexically-scoped fork/join, locks, and multi-join.
Due to space limitation, we refer readers
to Appendix~\ref{sec:delayed-app} for details.


%% Existing work for more expressive verification
%% of deadlock freedom.
%% Using threads as resource can improve it further.

}



==> appln-liveness.tex <==
\savesmallspace
\subsection{Thread Liveness and Resource Leakage}
\savesmallspace

Using our approach, threads' liveness can be precisely tracked.
For example, we could modify the program in Fig.~\ref{fig.shape}
to additionally keep track of already-completed (or dead) threads.
In the procedure \code{joinHelper}, after a thread is joined,
instead of destroying the corresponding item (line~29),
we could capture all items and their dead threads
in a $deadpool$~\footnote{Due to space limit, we refer interested readers
to {\tt deadpool} program in
our project webpage
%% {\toolurl}
for more details.}, inductively defined as follows:
\moresmallspace

\noindent
\form{\permsto{\self}{\code{deadpool}(n)}{} \defs \code{self{=}null} \wedge n{=}0 }

\form{ \bigvee \exists t,p \cdot \permsto{\self}{\code{item}(t,p)}{} {\sep} \permsto{p}{\code{deadpool}(n{-}1)}{} \wedge {\color{blue} \dead{t} } }

\form{\textbf{inv}~n{\geq}0;}
\moresmallspace



%% \morespace

%% Our approach is able to keep track of threads' liveness 
%% and their resources in a
%% precise manner. This is important for avoiding possible
%% leakages of thread resource. As an example,
%% consider the use of a resource split, prior
%% to the join operation.

%% {\color{blue}\hoare{ \outline ~ \{ \permsto{t}{\thread{ \constr_1 \sep  \constr_2 }}{} \}} }

%% This split would have released only resource R2 
%% from its thread after the join operation,
%% and would have lost track of the R1 via
%% a resource leakage. However, such scenarios are disallowed
%% by our verification system, since they lead
%% to t-inconsistent states.
%% \moresmallspace

%% %% \begin{verbatim}
%% %%   //t::thrd<R1* R2>
%% %%   //t::thrd<R1> * t::thrd<R2>
%% %%   join(t)
%% %%   // R2 * t::thrd<R1> & dead(t)
%% %% \end{verbatim}

%% This split would have allowed only resource $\constr_1$ to
%% This split would have allowed only resource $\constr_1$ to
%% be made available after the join operation,
%% and has indirectly lost resource $\constr_2$ in
%% a resource leakage. However, such a scenario is disallowed
%% by our verification system, as it is being
%% detected by a t-inconsistent state.


Our approach is also able to keep track of threads' resource in a
precise manner. This is important for avoiding
leakages of thread resource. As an example,
consider the use of a resource split, prior
to a join operation.\moresmallspace

{\color{blue}\hoare{ \outline ~ \{ \permsto{t}{\thread{ \constr_1 \sep  \constr_2 }}{} \}} }

{\color{blue}\hoare{ \outline ~ \{ \permsto{t}{\thread{ \constr_1 }}{} \sep \permsto{t}{\thread{ \constr_2 }}{} \}} }

\code{join(t);}

{\color{blue}\hoare{ \outline ~ \{ \constr_1 \sep \permsto{t}{\thread{ \constr_2 }}{} \wedge dead(t)  \}} }
\moresmallspace

%% \begin{verbatim}
%%   //t::thrd<R1* R2>
%%   //t::thrd<R1> * t::thrd<R2>
%%   join(t)
%%   // R2 * t::thrd<R1> & dead(t)
%% \end{verbatim}

This split causes the join operation to
release only resource $\constr_1$, whilst
$\constr_2$  remains trapped as resource inside a thread node.
This results in a resource leakage if the scenario
is permitted. However, such scenarios are disallowed
by our verification system, since they will be detected
as not being t-consistent.
\moresmallspace



==> approach-app.tex <==
The auxiliary function \myit{subst} is used to
substitute a discovered resource variable by
its corresponding definition. It is defined as follows:

\begin{equation*}
\begin{array}{c}
\myit{subst}(\hvardef,\D) \defs \code{fold\_left(} ~\code{fun}~ \D_1 ~ (\rsrvar,\D_2) \rightarrow \myit{apply}(\D_1,(\rsrvar,\D_2) )\code{)} ~ \D ~ \hvardef
\end{array}
\end{equation*}\savespace\savespace\savespace

\begin{equation*}
\begin{array}{c}
\myit{apply}(\emp \wedge \pure,(\rsrvar,\D) ) \defs \emp \wedge \pure \\
\myit{apply}(\rpreds{\btt{R}}{\code{v},\inflow \constr_1,\outflow \constr_2,\vlist{v}} \wedge \pure,(\rsrvar,\D) ) \defs
\code{let} ~ \constr_1' = \myit{apply}(\constr_1,(\rsrvar,\D) )  ~ \code{in}~ \\
\code{let} ~ \constr_2' = \myit{apply}(\constr_2,(\rsrvar,\D) )  ~ \code{in}~
\rpreds{\btt{R}}{\code{v},\inflow \constr_1',\outflow \constr_2',\vlist{v}} \wedge \pure \\
\myit{apply}(\heap_1 \sep \rsrvar \sep \heap_2 {\wedge} \pure,(\rsrvar,\D) ) \defs
\code{let} ~ \D_1 = \myit{apply}(\heap_1 \sep \heap_2 {\wedge} \pure,(\rsrvar,\D)) ~ \code{in} ~\D_1 \sep \D \\
\myit{apply}(\D_1 {\vee} \D_2,(\rsrvar,\D) ) \defs \myit{apply}(\D_1,(\rsrvar,\D) ) {\vee} \myit{apply}(\D_2,(\rsrvar,\D) ) \\
\myit{apply}(\D_1 \sep \D_2,(\rsrvar,\D) ) \defs \myit{apply}(\D_1,(\rsrvar,\D) ) \sep \myit{apply}(\D_2,(\rsrvar,\D) ) \\
\myit{apply}(\D_1 {\wedge} \pure,(\rsrvar,\D) ) \defs \myit{apply}(\D_1,(\rsrvar,\D) ) {\wedge} \pure \\
\myit{apply}({\exists} \code{v} {\cdot} \D_1,(\rsrvar,\D) ) \defs 
\code{let} ~ \myit{fresh} ~ \code{v}_1 ~ \code{in} ~
\code{let} ~ \rho = [\code{v}_1/\code{v}] ~ \code{in} ~
{\exists} \code{v}_1 {\cdot} ~\myit{apply}( \rho(\D_1),(\rsrvar,\D) )
\end{array}
\end{equation*}



\subsection{Forward Verification Rules}

\input{fwdrules}

%% In this section, 
We present selected Hoare-style verification rules
in Fig.~\ref{fig:fwdrules}. While previous approaches often
require specialized verification rule for each primitive,
%% (e.g. fork rule, join rule in \cite{Haack:AMAST08}),
our approach support all primitives under a single
\entrulen{CALL} rule. This greatly simplifies efforts
for implementing extended verification systems.
%%  for new concurrency
%% mechanisms.

\paragraph{Procedure Call}

In order to perform a procedure call (\entrulen{CALL}),
the caller should be in
a state $\D$ that can entail the pre-condition $\constr_{pr}$
of the callee (i.e the procedure $pn$).
$spec(pn)$ denotes the specification of the procedure $pn$.
For simplicity, we assume only pass-by-value parameters
since output parameters would require
full permissions of variables' resources,
to avoid data races.
For conciseness, we omit
the substitutions that link actual and formal parameters
of the procedure prior to the entailment.
The entailment (described in previous section) computes
the residue $\D_1$ and discovers resource bindings $\hvardef$.
The substitution $\myit{subst}(\hvardef,\constr_{po})$ is to replace
resource variables in the post-condition $\constr_{po}$
by their definition discovered in $\hvardef$.
The caller subsumes the substituted post-condition
with the residue $\D_1$ to form a new $\myit{consistent}$ state $\D_2$,
without any synchronization errors. 
%% \scsay{What do we mean by ``consistent'' here?}
%% Inflow resources are consumed during the entailment,
%% while outflow resources are introduced during the substitution.
%% \wnsay{can last line be omitted?}
%% \khanh{may need to talk about outflow and inflow here}.

\paragraph{Procedure Declaration}
Procedures are verified using the rule \entrulen{PROC}.
In other to verify the procedure body $\myit{e}$,
the pre-condition $\constr_{pr}$ is propagated through the body $\myit{e}$
and ends up in a state $\D_1$ which must entail
the post-condition $\constr_{po}$.
For simplicity, we described the rules in
Fig.~\ref{fig:fwdrules} with one pair of pre/post condition.
Muliple pre/post specifications can be handled
in the same way as \cite{Chin:HASE2007}.
We also ensure that each pre/post specification
is {\em resource-precise} with no ambiguous disjunction.

\paragraph{Lemma Normalization and Consistency}
We introduce lemmas for resource splitting and normalization.
The former is applied at branch points for forked processes,
guided by resource requirement of each thread.
The latter lemmas (for normalization) are applied 
exhaustively to each program point. We must ensure
that lemmas are resource-preserving and converging.
Consistency  checking is done on each normalized state
to determine
if some contradiction, such as double locking
or deadlock, has occurred. Due to 
%% our use of
over-approximation, these are potential synchronization errors.
%% All lemmas are checked for resource-preservation
%% to avoid resource leakage (or loss).
%% \wnsay{is consistency to avoid resource imprecision?}
%% \khanh{Need to talk about exhaustive application of normalization rules
%% and consistencies.}





==> concl.tex <==
%% In this paper, 
We proposed to model first-class threads as resource
to enable expressive treatment of threads' ownerships.
%% Similar to other types of resource,
%% such as ownerships of
%% heap objects and stack variables,
Our approach allows
resources of threads to be flexibly split,
combined, and transferred across procedure boundaries.
%% Modeling threads as resource has opened opportunities
%% for more expressive verification of programs
%% with dynamic thread creation and termination.
%% It enables verification of the multi-join
%% pattern where multiple joiners can join with the same
%% joinee in order to manipulate (read or write)
%% the resource of the joinee after join.
%% Furthermore, by combining threads as resource with predicate abstraction,
%% we can naturally capture the commonly-used threadpool idiom.
%% ``Threads as resource'' also improves
%% the existing delayed lockset checking technique
%% in order to verify deadlock freedom of intricate programs with
%% non-lexically-scoped fork/join, locks, and multi-join.
This enables verification of multi-join
pattern, where multiple joiners can share and join the same
joinee in order to manipulate (read or write)
the resource of the joinee after join.
%% Furthermore, we combined threads as resource
In addition, we demonstrated how threads as resource
is combined
with inductive predicates
to capture the commonly-used threadpool idiom.
Using a special {\em dead} predicate, we showed that
thread liveness can be
precisely 
tracked.
 %% in a precise manner.
%% We also presented how our approach improves
%% the existing delayed lockset checking technique
%% in order to verify intricate programs with
%% non-lexically-scoped fork/join, locks, and multi-join.
We have implemented our approach in a tool,
called {\toolname},
%%  on top of
%% %% the existing
%% {\sc{ParaHIP}} verifier, 
to verify partial correctness and
data-race freedom
%% and deadlock freedom
of concurrent programs with
non-lexically-scoped fork/join, first-class threads,
%% locks, 
and multi-join.
Our experiment showed that
{\toolname} is more expressive than {\sc{ParaHIP}}
while achieving comparable verification time.

As future work, we plan to exploit current advances
in resource synthesis (such as \cite{Calcagno:JACM11,Calcagno:APLAS09}) to
synthesize ``threads as resource''
specification automatically.


==> dead-lock.tex <==
%\vspace{-3mm}
\subsubsection{Ensuring Deadlock Freedom from Multiple Locks}
\label{sec:detect-deadlock}

The deadlock scenarios for a resource that may cycle
indefinitely through a finite number of states requires 
%% us to explicitly track the 
\code{wait-for} relation to be explicitly tracked 
in post-condition for each blocking method.
The key idea is to capture inter-lock
waits-for relation that reflects the order of locking,
as triggered
by each blocking command.
In the case of locks, the main 
blocking command is
the \code{acquire} primitive, which may 
depend on locksets that have been 
previously acquired. We precisely track a resource
\code{\LS{S}} which captures the set of locks that have
been acquired thus far, as follows:

\code{void acquire(l)}\\
\indent\quad \SPEC{\requires~\LockF{l}{P}{\fracperm} {\sep} \LS{S}}\\
\indent\quad \SPEC{\ensures~ \LockF{l}{P}{\fracperm} {\sep} \code{P} {\sep} \Held{l}{P}}\\
\indent\quad \SPEC{\qquad\qquad {\sep} \LS{\codeE{S{\cup}\{l\}}} {\sep} \WAIT{\codeE{S{\ra}l}};} %\\


\code{void release(l)}\\
\indent\quad \SPEC{\requires~\Held{l}{P} {\sep} \code{P} {\sep} \LS{S}}\\
\indent\quad \SPEC{\ensures~ \LS{S{-}\{l\}};} %\\

The \code{acquire} command adds \code{wait-for}
relation that may arise for the blocking primitive.
This is accumulated and checked for cycles, where possible.
An example of deadlock scenario is described next, with one thread
holding a lock needed by the other thread.
%% \begin{verbatim}
%%                l1 = create_lock()
%%                 l2 = create_lock()
%%                 # LockSet {}
%%    # LockSet {}        ||   # LockSet {}
%%    acquire(l1)         ||   acquire(l2) 
%%    # LockSet {l1}      ||   # LockSet {l2}
%%    acquire(l2)         ||   acquire(l1) 
%%    # WAIT{l2->l1}           # WAIT(l1->l2)
%%      * LockSet {l1,l2} ||     * LockSet {l1,l2}
%%    release(l2)         ||   release(l1)
%%    release(l1)         ||   release(l2)
%%    # WAIT{l2->l1}           # WAIT(l1->l2)
%%      * LockSet {}      ||     * LockSet {}
%%         # WAIT{l2->l1,l1->l2} * LockSet{}
%% \end{verbatim}


\begin{center}
\code{l1 = create\_lock(); l2 = create\_Lock()}

\code{\saying{\LSS{}}}
%% \hspace*{25mm}

\vspace{-12pt}
\[
{
\left(
\begin{tabular}{ l@{\extracolsep{\fill}}  || l@{\extracolsep{\fill}} }
%\code{\ldots} &~~\code{\ldots}\\
\code{\saying{\LSS{}}} &~~\code{\saying{\LSS{}}} \\
\code{acquire(l1);~~} &~~\code{acquire(l2);}\\
\code{\saying{\LSS{l1}}} &~~\code{\saying{\LSS{l2}}} \\
\code{acquire(l2);~~} &~~\code{acquire(l1);}\\
\code{\saying{\LSS{l1,l2} {\sep}}} &~~\code{\saying{\LSS{l2,l1}  {\sep} }} \\
\code{\saying{\quad\WAIT{\codeE{l1{\ra}l2}} }} &~~\code{\saying{\quad\WAIT{\codeE{l2{\ra}l1}}}} \\
\code{release(l1);~~} &~~\code{release(l1);}\\
\code{release(l2);~~} &~~\code{release(l2);}\\
\code{\saying{\LSS{}{\sep}}} &~~\code{\saying{\LSS{}  {\sep} }} \\
\code{\saying{\quad\WAIT{\codeE{l1{\ra}l2}} }} &~~\code{\saying{\quad\WAIT{\codeE{l2{\ra}l1}}}} \\
%\code{\ldots} &~~\code{\ldots}\\
\end{tabular}\right)\code{;}
}
\]

\code{\saying{\LSS{} {\sep} \WAIT{\codeE{l1{\ra}l2,l2{\ra}l1}} \sm{\longrightarrow} \ERR}}
\end{center}


==> entail-aux.tex <==
\begin{figure}%[b]
\begin{center}
\begin{minipage}{30pc}%{42pc}
\begin{frameit}
\begin{small}
\savespace\savespace\savespace\savespace

\begin{equation*}
\begin{array}{c}
\myit{freeEqn}([\code{u}_i/\code{v}_i]_{i=1}^n,\myit{V}) \defs %\\
\code{let} ~ \pure_i = (\code{if}~ \code{v}_i {\in} \myit{V} ~ \code{then} ~ \true ~ \code{else} ~ \code{v}_i = \code{u}_i) ~ \code{in} ~\bigwedge_{i=1}^n \pure_i %\\
\end{array}
\end{equation*}
\savespace\savespace\savespace\savespace\savespace\savespace

\begin{equation*}
\begin{array}{c}
\myit{apply}(\emp \wedge \pure,(\rsrvar,\D) ) \defs \emp \wedge \pure \\
\myit{apply}(\rpreds{\btt{R}}{\code{v},\inflow \constr_1,\outflow \constr_2,\vlist{v}} \wedge \pure,(\rsrvar,\D) ) \defs
\code{let} ~ \constr_1' = \myit{apply}(\constr_1,(\rsrvar,\D) )  ~ \code{in}~ \\
\code{let} ~ \constr_2' = \myit{apply}(\constr_2,(\rsrvar,\D) )  ~ \code{in}~
\rpreds{\btt{R}}{\code{v},\inflow \constr_1',\outflow \constr_2',\vlist{v}} \wedge \pure \\
\myit{apply}(\heap_1 \sep \rsrvar \sep \heap_2 {\wedge} \pure,(\rsrvar,\D) ) \defs
\code{let} ~ \D_1 = \myit{apply}(\heap_1 \sep \heap_2 {\wedge} \pure,(\rsrvar,\D)) ~ \code{in} ~\D_1 \sep \D \\
\myit{apply}(\D_1 {\vee} \D_2,(\rsrvar,\D) ) \defs \myit{apply}(\D_1,(\rsrvar,\D) ) {\vee} \myit{apply}(\D_2,(\rsrvar,\D) ) \\
\myit{apply}(\D_1 \sep \D_2,(\rsrvar,\D) ) \defs \myit{apply}(\D_1,(\rsrvar,\D) ) \sep \myit{apply}(\D_2,(\rsrvar,\D) ) \\
\myit{apply}(\D_1 {\wedge} \pure,(\rsrvar,\D) ) \defs \myit{apply}(\D_1,(\rsrvar,\D) ) {\wedge} \pure \\
\myit{apply}({\exists} \code{v} {\cdot} \D_1,(\rsrvar,\D) ) \defs 
\code{let} ~ \myit{fresh} ~ \code{v}_1 ~ \code{in} ~
\code{let} ~ \rho = [\code{v}_1/\code{v}] ~ \code{in} ~
{\exists} \code{v}_1 {\cdot} ~\myit{apply}( \rho(\D_1),(\rsrvar,\D) )
\end{array}
\end{equation*}\savespace\savespace\savespace

\begin{equation*}
\begin{array}{c}
\myit{subst}(\hvardef,\D) \defs \code{fold\_left(} ~\code{fun}~ \D_1 ~ (\rsrvar,\D_2) \rightarrow \myit{apply}(\D_1,(\rsrvar,\D_2) )\code{)} ~ \D ~ \hvardef
\end{array}
\end{equation*}\savespace\savespace\savespace\savespace\savespace

\begin{equation*}
\begin{array}{c}
\!\!\myit{isEmp}(\emp) \defs \true \quad
\myit{isEmp}(\heap {\wedge} \pure) \defs \myit{isEmp}(\heap) \quad
\myit{isEmp}(\heap_1 {{\sep}} \heap_2) \defs \myit{isEmp}(\heap_1){\wedge} \myit{isEmp}(\heap_2)\\
\myit{isEmp}(\D_1 \vee \D_2) \defs \myit{isEmp}(\D_1) {\wedge} \myit{isEmp}(\D_2) \qquad
\myit{isEmp}(\aheap) \defs \false ~~\myit{for}~\myit{atomic heap}~ \aheap
%\aheap = \permsto{\code{v}}{C(\vlist{v})}{\fracperm} \mid \term{P}(\code{v}) \mid  \rpredl{\btt{R}}{\vlist{v}}{\code{v},\overbar{\fconstr},\vlist{v}}\\
\end{array}
\end{equation*}\savespace\savespace\savespace

%% \begin{equation*}
%% \begin{array}{c}
%% \myit{match} (\rpreds{\btt{R}}{\code{x}_1, \vlist{v}_1}, \rpreds{\btt{R}}{\code{x}_2, \vlist{v}_2})
%% \defs
%% [\code{x}_1/\code{x}_2, \vlist{v}_1/\vlist{v}_2] %\\
%% \end{array}
%% \end{equation*}\savespace\savespace\savespace\savespace

\begin{equation*}
\begin{array}{c}
\myit{match} (\rpreds{\btt{R}}{\code{x}_1, \overbar{\fconstr}^1 , \vlist{v}_1}, \rpreds{\btt{R}}{\code{x}_2, \overbar{\fconstr}^2, \vlist{v}_2})
\defs
[\code{x}_1/\code{x}_2, \vlist{v}_1/\vlist{v}_2] %\\
\end{array}
\end{equation*}

\end{small}
\end{frameit}
\savesmallspace
\caption{Auxiliary Functions for Entailment}\label{fig:entail-aux}
\end{minipage}
%\savespace\savespace
\end{center}
\end{figure}


==> exp-mapreduce.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% \begin{wrapfigure}{r}{0.7\textwidth}
\begin{figure}[hbt]
%\savespace
%\savespace
%% \savespace
%\savespace
%\savespace
%{\footnotesize{\internallinenumbers[1]
\begin{center}
\begin{minipage}{19.25pc}%{42pc}
\begin{frameit}
\begin{small}
%BEGIn inc
{\internallinenumbers[1]
%
\!\!\code{data~node \{ int val; node next; \}}

\code{data~list \{ node head; \}}

\code{data~count \{ int val; \}}


\SPEC{\hoare{~\code{pred}~\code{ll}(\self,{n}) \veq \self{=}\code{null} \wedge n{=}0 }}

\SPEC{\hoare{~\bigvee \exists t,p \cdot \permsto{\self\!}{\!\code{node}(\_,q)}{} {\sep} {\code{ll}(q,n{-}1)} }}

\SPEC{\hoare{~~\textbf{inv}~n{\geq}0;}}

%\savespace

\code{}

\code{void~~countList(list~l)}

{\color{blue}\hoare{~\requires~~\permsto{\code{l}}{\code{list}(h)}{} \sep  {\code{ll}(h,n)} \wedge n{\geq}0 } }\\
{\color{blue}\hoare{~\ensures~~\permsto{\code{l}}{\code{list}(h)}{} \sep  {\code{ll}(h,n)} \wedge \res{=}n; } }

\codeE{\quad\{ \cdots \} }

\code{list~~createList(int~n)}

{\color{blue}\hoare{~\requires~~ n{\geq}0 } }\\
{\color{blue}\hoare{~\ensures~~\permsto{\res}{\code{list}(h)}{} \sep  {\code{ll}(h,n)}; } }

\codeE{\quad\{ \cdots \} }

\code{void~~mapper(list~l, list~o, list~e)}

{\color{blue}\hoare{\requires~\permsto{\code{l}\!}{\!\code{list}(h)}{} {\sep}  {\code{ll}(h,n)} {\sep} \permsto{\code{o}\!}{\!\code{list}(\code{null})}{} {\sep} \permsto{\code{e}\!}{\!\code{list}(\code{null})}{} } }
%
{\color{blue}\hoare{\!\hspace*{-1.5ex}\ensures~
%% \permsto{\code{l}}{\code{list}(h)}{} \sep  {\code{ll}(h,n)} \sep 
\permsto{\code{o}}{\code{list}(oh)}{} \sep {\code{ll}(oh,n_1)} \sep \permsto{\code{e}}{\code{list}(eh)}{} \sep} }
%
{\color{blue}\hoare{~~~~~~~~~~~~~~~~~{\code{ll}(eh,n_2)}  \wedge n{=}n_1{+}n_2; } }

\codeE{\quad\{ \cdots \} }


\code{void~~reducer(thrd~m, list~l, count c)}

%{\color{blue}\hoare{\requires~~\rpreds{Thrd}{ m,\permsto{l}{\code{list}(lh)}{} \sep  \permsto{lh}{\code{ll}(n)}{} \wedge n{\geq}0}{} } \sep  \permsto{c}{\code{count(\_)}}{} }
{\color{blue}\hoare{\requires~~\thrdpredtwo{m}{(\permsto{\code{l}\!}{\!\code{list}(h)}{} \sep  {\code{ll}(h,n)} {\wedge} n{\geq}0)}  \sep  \permsto{c\!}{\!\code{count(\_)}}{} }}

{\color{blue}\hoare{\ensures~~\hide{\permsto{m}{\dead{}}{}}\dead{m} \sep \permsto{l\!}{\!\code{list}(h)}{} \sep  {\code{ll}(h,n)} \sep  \permsto{c\!}{\!\code{count}(n)}{}; } }

\code{\{  join(m); \saying{multi-joined by the two reducers}}

\myspace\code{c.val~=~countList(l); \} }

\code{}

%BEGIn main
\code{void~~main() }

{\color{blue}\hoare{~~\requires~~\emp~~\ensures~~\emp;} }

%\hoare{requires~~\true} 

%\hoare{ensures~~{res=2};}

\code{\{ }\code{int~n = 10000;~~list~l = createList(n);}

\myspace\code{list ol = new list(null);~list el = new list(null);}

\myspace\code{count c1 = new count(0);~count c2 = new count(0);}

\myspace\code{\saying{creating threads}}

\myspace\code{thrd m = create\_thread(mapper);}
%% \saying{need to define}}

\myspace\code{thrd r1 = create\_thread(reducer);}
 %% \saying{need to define}}

\myspace\code{thrd r2 = create\_thread(reducer);}

\myspace\code{\saying{start map/reduce}}

\myspace\code{fork(m,l,ol,el);}

\myspace\code{fork(r1,m,ol,c1);}

\myspace\code{fork(r2,m,el,c2);}

\myspace\code{\saying{wait for it to finish}}

\myspace\code{join(r1);}

\myspace\code{join(r2);}


\myspace\SPEC{\code{assert(c1.val + c2.val = n);  \saying{valid}}}

%% \myspace\code{destroyAll();\khanh{if we use classical logic}} \\
\code{\} }

}
%END
\end{small}
\end{frameit}
%% \savespace
\savesmallspace
%}} %end 
\caption{Map/Reduce Pattern using Multi-join
%% \khanh{we elide the body of some procedures, which can be added later or in the appendix}
}
\label{fig:mapreduce}
\end{minipage}
\end{center}
\savespace\savespace
%\savespace\savespace
%% \end{wrapfigure}
\end{figure}
%\end{floatingfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> extensions.tex <==
In this section, we informally discuss how our soundness result
can be extended to threads and locks.

\paragraph{Threads}

Thread's \code{fork/join} is similar to {\CDL}'s
\code{coundDown/await}
in the following ways. In terms of resource flows,
a \code{fork} can be modeled as a \createlatch{} initialized
to 1 and immediately followed by a \code{countDown}, allowing
resource to inflow from the forker to the forkee's
thread abstraction.
A \code{join} is similar to an \code{await}, where
resource outflows from the joinee thread's abstraction
to the joiner.
Therefore, we extend the tagged memory model $\fpstate$
with a thread pool:

$ \fpstate \defs \pstack \times \fpheap \times \fpCDL \times \pgraph \times \fpthreads$

 $\fpthreads \defs \tids \times \ptagset \rightharpoonup \btt{THRD}(\tstates \times \flow \cdlR)) $

{\noindent} where $\tids$ is the set of unique thread identifiers
and $\tstates \defs \set{\btt{C},\btt{F},\btt{D}}$ is the set
of threads' states ($\btt{C}$ = created, $\btt{F}$ = forked,
and $\btt{D}$ = dead). The composition of threads can be defined
as the composition of its flow-aware resources, in a similar
way to CDLs.
However, the critical difference between threads
and CDLs is that while CDLs guarantee
that the inflow resource
is the same to the corresponding outflow resource,
the predicate transformer nature of threads does not give
such guarantee, but this occurs only at the {\createthrd}
command.
%%  have such a guanrantee
%% (since spawn threads can dispose
%% or create new resources). 
However, threads does guarantee race freedom
and resource-preservation for the \code{fork}
and \code{join} primitives.
As a result, we can freely use the resource-preserving
behaviour of the split lemmas.
%% since the inflow resource is consumed
%% by the abstraction and the outflow resource
%% can be soundly introduced by the sound
%% flow-aware split rules
%% (i.e. thread's execution acts as a predicate
%% transformer).


\paragraph{Locks} While CDLs are one-off controls that
cannot be reset,
locks are reusable (i.e. one can successively
invoke acquire/release pairs).
Additionally, in contrast to threads whose
states linearly go from \btt{C} (created),
to \btt{F} (forked), and end up
in \btt{D} (dead) state, after created,
locks can alternate indefinitely between the
\btt{H} (held) and \btt{U} (unheld) states.
To ensure deadlock freedom, we will also need to track the
lockset present for each given program fragment, and
then induce \code{wait-for} relation during the
blocking \code{acquire} commands. Any
cycle in this \code{wait-for} would denote a deadlock scenario,
and triggers a fault in the execution. Our soundness proof will
ensure that each proven program never fault (due to deadlock).
%% \khanh{may need to discuss deadlock freedom}

We can show the soundness properties of race-freedom
and resource preservation in our approach
by ensuring that outflow resource obtained by
acquire matches the inflow resource upon
the corresponding release\scnay{one of the two ``outflow'' should be ``inflow''?}. Data race freedom can be guaranteed
by proving that any program state
can be partitioned into those owned
by each thread and each lock.


==> fig-deadlock.tex <==
\savespace\savespace
\begin{wrapfigure}{l}{0.65\textwidth}
\begin{small}
\begin{center}
\code{c1 = \createlatch(1); c2 = \createlatch(1);}

\code{\CSPEC{\addperm{\WAIT{}}{1}{\sep}CNT(c1,1) {\sep} CNT(c2,1)  {\LRA}}}

\code{\CSPEC{CNT(c1,1) {\sep} CNT(c2,0) {\sep} CNT(c2,1) {\sep} CNT(c1,0) }}

%% \hspace*{25mm}

\vspace{-12pt}
\[
{
\left(
\begin{tabular}{ l@{\extracolsep{\fill}}  || l@{\extracolsep{\fill}} }
%\code{\ldots} &~~\code{\ldots}\\
\code{\CSPEC{CNT(c1,1){\sep}CNT(c2,0)}} &~~\code{\CSPEC{CNT(c2,1){\sep}CNT(c1,0)}}\\
\code{await(c2);~~} &~~\code{await(c1);}\\
\code{\CSPEC{CNT(c1,1){\sep}CNT(c2,-1)}} &~~\code{\CSPEC{CNT(c2,1){\sep}CNT(c1,-1)}}\\
\code{\CSPEC{\quad\sep\addperm{\WAIT{\codeE{c2{\ra}c1}}}{\fracperm_1}}}  &~~\code{\CSPEC{\quad\sep\addperm{\WAIT{\codeE{c1{\ra}c2}}}{\fracperm_2}}}  \\
\code{countDown(c1);~~} &~~\code{countDown(c2);}\\
\code{\CSPEC{CNT(c1,0){\sep}CNT(c2,-1)}} &~~\code{\CSPEC{CNT(c2,0){\sep}CNT(c1,-1)}}\\
\code{\CSPEC{\quad\sep\addperm{\WAIT{\codeE{c2{\ra}c1}}}{\fracperm_1}}}  &~~\code{\CSPEC{\quad\sep\addperm{\WAIT{\codeE{c1{\ra}c2}}}{\fracperm_2}}}  \\
%\code{\ldots} &~~\code{\ldots}\\
\end{tabular}\right)%\code{;}
}
\]

\code{\CSPEC{\quad CNT(c1,-1){\sep}CNT(c2,-1){\sep}\addperm{\WAIT{\codeE{c2{\ra}c1,c1{\ra}c2}}}{1} }} \\
\code{\CSPEC{{\color{red}{\DEADLOCK} detected by \errrulen{3} }}}
%\code{\saying{\qquad \WAIT{\codeE{c2{\ra}c1,c1{\ra}c2}} ${\longrightarrow}$ \DEADLOCK}}
\end{center}
\savespace\savespace\savesmallspace
\caption{An example of inter-latch deadlock %% detection via wait-for
}\label{fig.deadlock.waitfor}
\end{small}
\end{wrapfigure}

==> fig-equiv.tex <==
\begin{figure}[!t]
%% \savespace
\savespace
\begin{center}
\begin{minipage}{28pc}%{42pc}
\begin{frameit}
%% \savespace
%% \savespace
\savespace
\[
\begin{array}{c}
\permsto{t1}{\thread{ \permsto{x}{cell(2)}{} \sep  \permsto{y}{cell(1)}{} }}{} \\

\stackrel{\text{\ensuremath{\entrulen{R-THRD1}}}}{\Longleftrightarrow} \\

\permsto{t1}{\thread{ \permsto{x}{cell(2)}{} }}{} \sep \permsto{t1}{\thread{\permsto{y}{cell(1)}{} }}{} \\

\stackrel{\text{\ensuremath{\entrulen{R-FRAC}}}}{\Longleftrightarrow} \\

\permsto{t1}{\thread{ \permsto{x}{cell(2)}{0.6} \sep \permsto{x}{cell(2)}{0.4} }}{} \sep \permsto{t1}{\thread{\permsto{y}{cell(1)}{} }}{} \\

\stackrel{\text{\ensuremath{\entrulen{R-THRD1}}}}{\Longleftrightarrow} \\

\permsto{t1}{\thread{ \permsto{x}{cell(2)}{0.6}  }}{} \sep \permsto{t1}{\thread{\permsto{x}{cell(2)}{0.4} }}{} \sep \permsto{t1}{\thread{\permsto{y}{cell(1)}{} }}{} \\

\stackrel{\text{\ensuremath{\entrulen{R-FRAC},\entrulen{R-THRD1}}}}{\Longleftrightarrow} \\

\permsto{t1}{\thread{ \permsto{x}{cell(2)}{0.6}  }}{} \sep \permsto{t1}{\thread{\permsto{x}{cell(2)}{0.4} }}{} \sep \\
\permsto{t1}{\thread{\permsto{y}{cell(1)}{0.6} }}{} \sep \permsto{t1}{\thread{\permsto{y}{cell(1)}{0.4} }}{} \\

\stackrel{\text{\ensuremath{\entrulen{R-THRD1},\entrulen{R-THRD1}}}}{\Longleftrightarrow} \\

\permsto{t1}{\thread{ \permsto{x}{cell(2)}{0.6} \sep \permsto{y}{cell(1)}{0.6} }}{} \sep \\
\permsto{t1}{\thread{ \permsto{x}{cell(2)}{0.4} \sep \permsto{y}{cell(1)}{0.4} }}{}

\end{array} 
\]
\savespace


\end{frameit}
%% \savespace
\savespace
\caption{An Example of Resource Equivalence}\label{fig.equiv}
\end{minipage}
\savespace\savespace
\savespace
%% \savespace
%% \savespace\savespace
%% \savespace\savespace
%% \savespace\savespace
\savespace
\end{center}
\end{figure}


==> fig.latch.cone2.tex <==
\begin{wrapfigure}{l}{0.62\textwidth} 
%\begin{frameit}
\vspace{-2mm}
\begin{minipage}[c]{0.5\textwidth}
\centering
\code{c = \createlatch(2);}

\vspace{-12pt}
\[
\left(
\begin{tabular}{ 
  l@{\extracolsep{\fill}} || 
  l@{\extracolsep{\fill}} || 
  l@{\extracolsep{\fill}} }
\BCOMMENT{\SPEC{$T_1$}} & \BCOMMENT{\SPEC{$T_2$}} & \BCOMMENT{\SPEC{$T_3$}}\\
\BCOMMENT{\SPEC{\code{$h{:=}h_s\code{cos}\frac{\theta}{2}$;}}} & 
\BCOMMENT{\SPEC{\code{$r{:=}h_s\code{sin}\frac{\theta}{2}$;}}} & \\
\code{countDown(c);} & \code{countDown(c);} & \code{await(c);}\\
& & \BCOMMENT{\SPEC{\code{$V{:=}\frac{1}{3}\pi r^2 h$;~}}}\\
\end{tabular}\!\!\right)\!\!\code{;}
\]
\end{minipage}
%% \end{tabular}

%\end{frameit}
%% \vspace{-2mm}
\caption{A use-case of %% synchronization pattern with
  {\CDL}}
\label{fig:latch_wait_for_cons2}
\end{wrapfigure}





==> fpred-latch.tex <==
%% \subsection{Modelling \CDL}

A resource predicate instance \sm{\btt{R}[\vlist{w}](\code{x},\overbar{\fconstr},\vlist{v})} encapsulates in-flow and/or out-flow resources  (\sm{\overbar{\fconstr}}) that are accessible via \code{x}.  The 
\sm{\vlist{w}} denotes an optional list of logical variables, e.g. to link  in-flow pre-condition \code{P} and out-flow post-condition \code{Q}
in \thrdpredone{\vlist{\code{w}}}{\res}{P}{Q}{\vlist{\code{v}}},
while \vlist{v} captures a list of arguments (Sec~\ref{sec:thread}).
We use the flow annotation 
\codeE{\OM} to denote an inflow (from the
current thread) into the resource predicate,
while annotation 
\codeE{\OP} will denote an outflow 
from the resource predicate
(into the current thread).
We shall model each \code{CountDownLatch} \code{c}
with two resource predicates:
\codeE{Latch(c,\ldots)} and
\code{CNT(c,n)}. The first resource
predicate has two variants (i)
%\codeE{Latch(c,{\OM}P)} 
\LatchIn{c}{P}
for
\code{countDown} primitive to capture a
resource inflow,
(ii) %\codeE{Latch(c,{\OP}P)} 
\LatchOut{c}{P}
for \code{await} primitive to capture 
a resource outflow. 
Both these variants
may be freely split and
combined to support multiple synchronization points, as follows:
%\begin{verbatim}
%  Latch(c,-P*Q) <--> Latch(c,-P)*Latch(c,-Q)
%  Latch(c,+P*Q) <--> Latch(c,+P)*Latch(c,+Q)
%\end{verbatim}

\SPEC{\LatchIn{c}{(P{\sep}Q)} \sm{\longleftrightarrow} \LatchIn{c}{P} {\sep} \LatchIn{c}{Q}}

\SPEC{\LatchOut{c}{(P{\sep}Q)} \sm{\longleftrightarrow} \LatchOut{c}{P} {\sep} \LatchOut{c}{Q}}

\noindent
The other  resource predicate \code{CNT(c,n)} is used to track
the counter of the latch. 
\khanh{move the following to behind the definitions}
The presence of a positive counter
\codeE{CNT(c,n){\wedge}n{>}0} denotes a {\RLoaded} predicate.
However, a resource predicate \codeE{CNT(c,n){\wedge}n{<}0} with a negative counter
denotes a {\RLess} instance, whose
%% required
%% counting
synchronization has already completed. There is however
an ambiguous scenario, namely \codeE{CNT(c,0)},
which could denote either a
{\RLoaded} or a {\RLess} predicate instance.
We refer to this as a {\RAmb} instance.
%% \scsay{Do we have an example here?}. 
%% We define this as a {\RAmb} predicate instance:
%% \begin{mydef}[Resource-Ambiguous]\label{def:loaded}
%% A {\RAmb} predicate is a predicate which may or may not
%% capture some resource state. Each of its occurrences shall be tracked precisely to
%% avoid possible resource leakage. \scsay{This defn is  vague as it does not define what is  a {\RAmb} pred?}
%% \end{mydef}

Using these resource predicates,
\scnay{``These two'' refer to preds before defn 3; so maybe defn 3 can
be introduced later to flow better?} %
we can now
%% model and
create each \code{CountDownLatch} by the following method
which would be used to perform synchronization for
some resource \code{P}:\khanh{need to add
create\_latch() with P and remove all CountDownLatch()}.

\chsay{What is \code{with} in \code{create\_latch}'s definition?
It is not given in Fig. \ref{fig:proglang}. What are the return types 
and the parameters' types of the following methods?}

\code{\createlatch(n)~with~P}\\
\indent\quad \SPEC{\requires~\code{n{>}0}}\\
\indent\quad \SPEC{\ensures~ \LatchIn{res}{P} {\sep}\LatchOut{res}{P}{\sep}\code{CNT(res,n)}} \\
\indent\code{\{~return~new~CountDownLatch(n);\}}
%% \scnay{warning: syntax here is diff from Fig 2; new countDownLatch(..) has already been used in earlier examples..}

%% The second type of resource \code{CNT(c,n)}
%% is used to track the \code{countDown}

Each \code{countDown} can be made to decrement 
its positive counter \code{CNT(c,n)\sm{\wedge}n{>}0} and 
consume a resource via its \LatchIn{c}{P} predicate,
as shown in the first specification below. The second pre/post specification is
used if the counter \hide{\codeE{CNT(c,n){\wedge}n{\leq}0} }has 
completed its counting.
%% requirement.
%% become non-positive. 

%%\begin{verbatim}
%%  countDown(c)
%%   requires Latch(c,-P) * P * CNT(c,n) & n>0
%%   ensures CNT(c,n-1);
%%   requires CNT(c,n)<=0
%%   ensures  CNt(c,n);
%%\end{verbatim}

\code{countDown(c)}\\
\indent\quad \SPEC{\requires~\LatchIn{c}{P}{\sep}\code{P}{\sep}\code{CNT(c,n)}\sm{\wedge}\code{n{>}0}}\\
\indent\quad \SPEC{\ensures~ \code{CNT(c,n{-}1)};}\\
\indent\quad \SPEC{\requires~\code{CNT(c,n)}\sm{\wedge}\code{n\sm{\leq}0}}\\
\indent\quad \SPEC{\ensures~ \code{CNT(c,n)};}

\chsay{How about the case of \code{requires CNT(c,n) \sm{\wedge} n{>}0}, 
i.e. without resource P?}

Each \code{await} primitive would release its resource
from predicate \LatchOut{c}{P}, but
only if its counter has reached zero via \code{CNT(c,0)}. 
If the latch's counter has already reached a
negative number, \codeE{CNT(c,n){\wedge}n{<}0}, the \code{await} primitive performs
a no-op, as reflected in the second pre/post specification.
%%\begin{verbatim}
%%  await(c)
%%   requires Latch(c,+P) * CNT(c,0)
%%   ensures  CNT(c,-1) * P;
%%   requires CNT(c,n) & n<0
%%   ensures  CNT(c,n);
%%\end{verbatim}

\code{await(c)}\\
\indent\quad \SPEC{\requires~\LatchOut{c}{P}{\sep}\code{CNT(c,0)}}\\
\indent\quad \SPEC{\ensures~ \code{CNT(c,{-}1)}{\sep}\code{P};}\\
\indent\quad \SPEC{\requires~\code{CNT(c,n)}\sm{\wedge}\code{n{<}0}}\\
\indent\quad \SPEC{\ensures~ \code{CNT(c,n)};}

To support concurrent forking of threads, we allow
non-negative counter predicates to be split; while non-positive
counters are always combined, where possible, to maintain a normalized
state.

\chsay{Why do we need to split latch's count across threads? 
Can you give an example for this split?}

%%\begin{verbatim}
%%CNT(c,n) & a,b>=0 & n=a+b    --> CNT(c,a) * CNT(c,b)
%%CNT(c,a) * CNT(c,b) & a,b<=0 --> CNT(c,a+b)
%%Latch(c,+P) * CNT(c,n) & n<0 --> P  
%%\end{verbatim}

\SPEC{\code{CNT(c,n)}\sm{\wedge}\code{a,b}\sm{{\geq}0}\sm{\wedge}\code{n{=}a{+}b} \sm{\longrightarrow} \code{CNT(c,a)}{\sep}\code{CNT(c,b)}}
\\
\indent
\SPEC{\code{CNT(c,a)}{\sep}\code{CNT(c,b)}\sm{\wedge}\code{a,b}\sm{{\leq}0} \sm{\longrightarrow} \code{CNT(c,a{+}b)}}


%% \subsubsection{Ensuring Resource-Preservation}




==> fwdrules.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NEW forward Verification Rules 
\begin{figure*}%[b]
\savespace
\savespace
\begin{center}
\begin{minipage}{25pc}%{37pc}%{42pc}
\begin{frameit}
\begin{small}
\savespace
\savespace
\[
%\hspace{-3mm}
\begin{array}{c}
%%%%%%%%%%%%%%%%%%%%
%PROC
%%%%%%%%%%%%%%%%%%%%
\begin{array}{c}
\frac{
\begin{array}{c}
[\entrulen{PROC}]\\

\hoare{ \{ \constr_{pr} \wedge \bigwedge(\code{v}'=\code{v}) \} }

%\hspace{3pt}
~\myit{e}~
%\hspace{3pt}
%\\

\hoare{ \{ \D_1 \} }

%\\%
\qquad

\entailS{\D_1}{\constr_{po}}

\end{array}
}{
\begin{array}{c}

\vdash

\nonterm{t} ~ 
\term{pn}(\overbar{\nonterm{t}~\term{v}}) ~ \lit{requires} ~\constr_{pr} ~\lit{ensures}~
\constr_{po}\lit{;}
~\{~\nonterm{e}~\}



\end{array}
}
%\qquad
%\\
\end{array} %& \entrulen{PROC} \vspace{2mm} 
\\ 

%%%%%%%%%%%%%%%%%%%%
%NORMAL CALL
%%%%%%%%%%%%%%%%%%%%
\begin{array}{c}
\frac{
\begin{array}{c}

[ \entrulen{CALL}]\\

spec(pn) := \code{pn}(\vlist{w}) ~ \lit{requires} ~\constr_{pr} ~\lit{ensures}~
\constr_{po}\lit{;}

\\

\entailH{\D}
        {\constr_{pr}}
        {(\hvardef,\D_1)}

\quad

\D_2 \defs \D_1 \sep \myit{subst}(\hvardef,\constr_{po})

\quad

\D_2  ~\myit{is~ consistent}

\end{array}
}{
\begin{array}{c}

\hoare{ \{ \D \} }

\hspace{3pt}
\hoare{ {\nonterm{pn}} \lit{(} \vlist{\code{w}} \lit{)} }

\hspace{3pt}

\hoare{ \{ \D_2 \} }

\end{array}
}
\qquad
%\\
\end{array} %& \entrulen{CALL} \vspace{2mm} \\ 

\hide{
%%%%%%%%%%%%%%%%%%%%
%FORK
%%%%%%%%%%%%%%%%%%%%
\begin{array}{c}
\frac{
\begin{array}{c}

spec(pn) := \code{pn}(w^*) ~ \lit{requires} ~\constr_{pr} ~\lit{ensures}~
\constr_{po}\lit{;}

\\

\entailS{\D}{\constr_{pr} \rewrite \D_1}

\quad

\D_2 \defs \D_1 \sep \permsto{\term{v}}{ \thread{\constr_{po}} }{} 

\quad

\D_2  ~is~ t{-}consistent

\end{array}
}{
\begin{array}{c}

\hoare{ \{ \D \} }

\hspace{3pt}
\hoare{ {\nonterm{v}} := \lit{fork} \lit{(} \nonterm{pn} \lit{,}
	\term{w}^* \lit{)} }
\hspace{3pt}

\hoare{ \{ \D_2 \} }

\end{array}
}
\qquad
%\\
\end{array} & \entrulen{FORK} \vspace{2mm} \\ 

%%%%%%%%%%%%%%%%%%%%
%JOIN-1
%%%%%%%%%%%%%%%%%%%%
\begin{array}{c}
\frac{
\begin{array}{c}

\D_2 \defs  \D \sep \constr_{po} \wedge \dead{v}

\quad

\D_2  ~is~ t{-}consistent

\end{array}
}{
\begin{array}{c}

\hoare{ \{ \D \sep \permsto{\term{v}}{ \thread{\constr_{po}} }{} \} }

\hspace{3pt}
\hoare{ {\lit{join}} \lit{(} \term{v} \lit{)} }
\hspace{3pt}

\hoare{ \{\D_2 \} }

\end{array}
}
\qquad
%\\
\end{array} & \entrulen{JOIN-1}  \vspace{2mm} \\

%%%%%%%%%%%%%%%%%%%%
%JOIN-2
%%%%%%%%%%%%%%%%%%%%
\begin{array}{c}
\begin{array}{c}

\hoare{ \{ \D \wedge \dead{v} \} }

\hspace{3pt}
\hoare{ {\lit{join}} \lit{(} \term{v} \lit{)} }
\hspace{3pt}

\hoare{ \{ \D \wedge \dead{v} \} }

\end{array}

\qquad
%\\
\end{array} & \entrulen{JOIN-2} \\ 

} %%END HIDE


\end{array}
\]
\end{small}
\savespace
\end{frameit}
\savesmallspace
%\savespace
\caption{Selected Verification Rules}\label{fig:fwdrules}
\end{minipage}
\savespace\savespace
\savespace\savespace
%\savespace\savespace
\end{center}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> h-lock.tex <==
\vspace{-2mm}
\subsubsection{Hierarchical Locks}
%So far, we have only considered coarse-grained locks where
%the lock predicates are being split fractionally to support the
%\code{acquire} operation. 
Different from the coarse-grained locks we have seen so far,
we shall now consider a novel class
of locks, called hierarchical locks, that can support locks of varying levels
of granularities. The trick to supporting such locks is to allow
the resource contents of the lock to be split and combined, as follows:
%% , where appropriate
%% through the following lemma:
%% \begin{verbatim}
%%   // fractional split
%%   Lock(id,.P@f) <--> Lock(id,.P@f1) * Lock(id,.P@f2) & f=f1+f2
%% \end{verbatim}

%% \SPEC{\it$\LockG{l}{R}{f} \sm{\longleftrightarrow} \LockG{l}{R}{f_1} {\sep} \LockG{l}{R}{f_2} {\wedge} f{=}f_1{+}f_2$}
\SPEC{\it$\Lock{l}{(P{\sep}Q)} \sm{\longleftrightarrow} \Lock{l}{P} {\sep} \Lock{l}{Q}$}

%% As an example of its utility, a composite lock with resource
%% \codeE{P{\sep}Q} could be made to support a split of the form:
Instead of one lock, the above split now supports two
fine-grained locks.
%% This approach would have allowed us to reason 
%% about concurrency primitives
%% that can support hierarchical locks.
%% This flexibility allows us to support both coarse-grained
%% and fine-grained locking.
The lock creation method would now
have the following specification
with an extra predicate
\code{\LockRef{res}{P}} where un-annotated
parameter \code{P} serves as a 
reference for the original resource of the lock.
%% when it was first created.
%% We believe this approach (which splits resources rather than
%% the predicate itself) is more general since it could be used to support 
%% hierarchical locking, with both coarse-grain 
%% and fine-grain locks. 

\code{create\_lock()~\SPEC{with~P}}\\
\indent\quad \SPEC{\requires~\code{P}}\\
\indent\quad \SPEC{\ensures~ \Lock{res}{P}{\sep}\LockRef{res}{P};} %\\

Our operation to acquire locks would
now be specified as:
%% have the following specification:

\code{void acquire(l)} \SPEC{\code{with P}}\\
\indent\quad \SPEC{\requires~\Lock{l}{P}}
\indent\quad \SPEC{\ensures~ \code{P} {\sep} \HeldE{l}{P};} %\\

After acquiring the lock, resource \code{P} is made available together
with a predicate \code{\HeldE{l}{P}} which indicates the hierarchical
lock\footnote{Hierarchical locks using \code{\HeldE{l}{P}}
may be made to 
co-exist with the coarse-grained
locks using \code{\Held{l}{P}}.
For simplicity, we omit this consideration.} 
that has been acquired. This {\RLoaded} predicate marks
the actual lock portion that has been held by the thread, and
is different in that its resource can be joined and
split, as follows:
%% which invoked the \code{acquire} operation.
%% It can be moreover joined and split,
%% like the other {\RLoaded} predicate.

\SPEC{\it$\HeldE{l}{(P{\sep}Q)} \sm{\longleftrightarrow} \HeldE{l}{P} {\sep} \HeldE{l}{Q}$}

Using it, the \code{release}
primitive is capable of returning some
arbitrary lock resource, as captured by
the following specification.

\code{void release(l) \SPEC{with P}}\\
\indent\quad \SPEC{\requires~\HeldE{l}{P} {\sep} \code{P}}
\indent\quad \SPEC{\ensures~ \Lock{l}{P};} %\\

The lock disposal itself requires the earlier
\code{LockREF} predicate, to help
%% as a reference
 %% to help recall 
return the original
coarse-grained lock.

\code{void dispose(l)}\\
\indent\quad \SPEC{\requires~\Lock{l}{P} {\sep}\LockRef{l}{P}}\\
\indent\quad \SPEC{\ensures~ \UnHeld{l} {\sep} \code{P};} %\\

Due to our use of local reasoning (without
%% the use of
global lock store), each of the primitives used for
hierarchical locking 
is currently \underline{not} resource-preserving. In fact, each
\code{create\_lock} would have to be eventually paired
with a corresponding \code{dispose} for the two calls to
be resource-preserving. Similarly, each \code{acquire}
(or set of \code{acquire} operations) would have to be balanced
by its corresponding \code{release} (or set of 
\code{release} operations),  to help ensure that
the net resource consumed/produced
is zero for the entire program.
Synchronization errors themselves are detected by two lemmas:

\SPEC{\it$\LockRef{l}{P} {\sep} \UnHeld{l} {{\wedge} \codeE{\neg(\code{P}{=}\code{\emp})}}  ~\sm{\longrightarrow}~ \ERR $}

\SPEC{\it$\HeldE{l}{P} {\sep} \HeldE{l}{Q} {\wedge} \code{UNSAT(P{\sep}Q)}  ~\sm{\longrightarrow}~ \ERR $}

These lemmas ensure that there are no double locking and that 
%% the entire 
single lock scenario is deadlock-free. In case we have multiple locks, we can
place them together as a composite lock. Using
hierarchical locking, we can request for the locks at finer
granularity. A good thing is that any potential
deadlock is detected using just the synchronization lemmas.
If multiple separate locks have been created, we will have
to maintain a 
%% declare a total ordering on the lock resource to ensure no cycle in its 
waits-for graph to ensure deadlock-freedom by detecting
cycles, as illustrated in Sec~\ref{sec:detect-deadlock}.
%% in prior works at \cite{Leino:ESOP2010,Le:ATVA13}.

%% The concept of hierarchical locking also subsumes read/write locks, since
%% we may split the captured resource fractionally:
%%  %% as follows:

%% \SPEC{\it$\Lock{l}{P} \sm{\longleftrightarrow} \Lock{l}{P{\at}\,0.5} {\sep} \Lock{l}{P{\at}\,0.5}$}

%% With this use of fractional resources, 
%% our mechanism can now support multiple reader locks
%% concurrently, but would only support unique writer locks. Any locking
%% %% synchronization
%% errors are automatically detected by our synchronization lemma on the
%% \code{Held} predicate.

%% \begin{verbatim}
%%    acquire(l)
%%       requires Lock(l,.P)@f
%%       ensures  Lock(l,.P)@f * P * Held(l,-P);
%% \end{verbatim}

%% \begin{verbatim}
%%    release(l)
%%       requires Held(l,-P) * P
%%       ensures  emp;
%% \end{verbatim}

%% \begin{verbatim}
%%    dispose(l)
%%       requires Lock(l,.P)
%%       ensures  UnHeld(l);
%% \end{verbatim}



==> header.tex <==
\usepackage{algpascal}
\usepackage{ifthen}
\usepackage{times,frameit,epsfig,amsmath,color,latexsym,graphics,wrapfig}
\usepackage{amssymb,centernot,multicol,multirow,mathtools}
%% clrscode3e
\usepackage{algorithm,algpseudocode}
%% \newcommand{\wnsay}[1]{{{\color{blue}({\bf WN:} \textit{#1})}}}
%% \newcommand{\wnnay}[1]{}
\newcommand{\chsay}[1]{{{\color{BlueGreen}({\bf Chanh:} \textit{#1})}}}
\newcommand{\chnay}[1]{}
\newcommand{\cgsay}[1]{{{\color{magenta}({\bf Cris:} #1)}}}
\newcommand{\cgnay}[1]{}
\newcommand{\scsay}[1]{{{\color{cyan}({\bf SC:} \textit{#1})}}}
\newcommand{\scnay}[1]{}
\newcommand{\khsay}[1]{{{\color{cyan}({\bf Khanh:} \textit{#1})}}}
\newcommand{\khnay}[1]{}

%% \usepackage{algorithmic}
%%\usepackage{algc}

%% \usepackage{algpseudocode}
%% \floatname{algorithm}{Procedure}
%% \usepackage{longtable}
%\usepackage{listings}
%\algsetup{
%linenodelimiter=.
%}
%\usepackage{program}

\newcommand{\cimplies}{\approx\!\!>}
%%%%%%%%%%%%%%%%


%used in disjunctive predicates specialization
\newcommand{\QED}{\ensuremath{~\Box}}
%\newcommand{\relsp}{\ensuremath{\hookrightarrow\!\!\!{\textit{sp}}}}
%arrow for specialising predicate
\newcommand{\arrowsp}{\ensuremath{-\!{\textrm{\small sp}\!{\rightarrow}}}}
%arrow for specialising formula
\newcommand{\arrowsf}{\ensuremath{-\!{\textrm{\small sf}\!{\rightarrow}}}}
%arrow for specialising formula (closure)
\newcommand{\arrowsfclosure}{\ensuremath{-\!{\textrm{\small sf}\!{{\rightarrow}}^*}}}
%arrow for specialising formula (multiple steps)
\newcommand{\arrowmsf}{\ensuremath{-\!{\textrm{\small msf}\!{\rightarrow}}}}
%arrow for optimised predicate specialisation
\newcommand{\arrowosp}{\ensuremath{-\!{\textrm{
\small osp}\!{\rightarrow}}}}
%arrow for optimised formula specialisation
\newcommand{\arrowosf}{\ensuremath{-\!{\textrm{\small osf}\!{\rightarrow}}}}
%arrow for filtering pruning conditions
\newcommand{\arrowfilter}{\ensuremath{-\!{\textrm{\small filter}\!{\rightarrow}}}}
%arrow for initialising heap
\newcommand{\arrowinitheap}{\ensuremath{-\!{\textrm{\small ih}\!{\rightarrow}}}}
%arrow for initialising formula
\newcommand{\arrowinitform}{\ensuremath{-\!{\textrm{\small if}\!{\rightarrow}}}}
%arrow for inferring specialised predicate
\newcommand{\arrowspi}{\ensuremath{-\!{\textrm{\small isp}\!{\rightarrow}}}}
%arrow for normalisation
\newcommand{\arrownormalise}{\ensuremath{-\!{\textrm{\small norm}\!{\rightarrow}}}}

% predicate specialisation rule
\newcommand{\predspec}[4]{\ensuremath{{#1} ~|~ {#2} ~{\arrowsp}~ {#3} ~|~ {#4}}}
%formula specialisation rule
\newcommand{\formspec}[4]{\ensuremath{{#1} ~|~ {#2}~{\arrowsf}~ {#3}~|~ {#4}}}
% optimised predicate specialisation rule
\newcommand{\opredspec}[4]{\ensuremath{{#1} ~|~ {#2} ~{\arrowosp}~ {#3} ~|~ {#4}}}
% optimised formula specialisation rule
\newcommand{\oformspec}[4]{\ensuremath{{#1} ~|~ {#2}~{\arrowosf}~ {#3}~|~ {#4}}}

%formula specialisation closure rule
\newcommand{\formspecclosure}[4]{\ensuremath{{#1} ~|~ {#2}~{\arrowsfclosure}~ {#3}~|~ {#4}}}
%multi-step formula specialisation rule
\newcommand{\mformspec}[3]{\ensuremath{{#1} ~{\arrowmsf}~ {#2}~|~ {#3}}}
\newcommand{\mformspecA}[2]{\ensuremath{{#1} ~{\arrowmsf}~ {#2}}}
%special rule for formula specialisation
\newcommand{\formspecdisj}[3]{\ensuremath{{#1} ~{\arrowsf}~({#2})\vee ({#3})}}
%pruning condition filtering rule
\newcommand{\filter}[4]{\ensuremath{#1,#2 \vdash #3 ~{\arrowfilter}~#4}}
% heap initialisation rule
\newcommand{\initheap}[3]{\ensuremath{ {#1}  ~{\arrowinitheap}~ {#2} ~|~ {#3}}}
%% \newcommand{\savespace}{\vspace{-2mm}}
% formula initialisation rule
%\newcommand{\initform}[4]{\ensuremath{\!\! {\exists} {#1}{\cdot} ({#2})  ~{\arrowinitform}~ {\exists} {#1}{\cdot} ({#3} \,|\, {#4})\!\!}}
\newcommand{\initform}[3]{\ensuremath{{#1}   ~{\arrowinitform}~ {#2} \,|\, {#3}}}
%inferring specialised predicate
\newcommand{\infspec}[2]{\ensuremath{{#1} ~{\arrowspi}~ {#2}}}
%normalisation
\newcommand{\normalise}[2]{\ensuremath{{#1} ~{\arrownormalise}~ {#2}}}

%predicate specialisation rule name
\newcommand{\sprulen}[1]{[\underline{{\bf \scriptstyle SP-}\rulen{#1}}]}
%formula specialisation rule name
\newcommand{\sfrulen}[1]{[\underline{{\bf \scriptstyle SF-}\rulen{#1}}]}
%initialisation rule name
\newcommand{\initrulen}[1]{[\underline{{\bf \scriptstyle INIT-}\rulen{#1}}]}
%improved predicate specialisation rule name
\newcommand{\isprulen}[1]{[\underline{{\bf \scriptstyle OSP-}\rulen{#1}}]}
%improved formula specialisation rule name
\newcommand{\isfrulen}[1]{[\underline{{\bf \scriptstyle OSF-}\rulen{#1}}]}
%specialised predicate inference rule name
\newcommand{\spirulen}[1]{[\underline{{\bf \scriptstyle ISP-}\rulen{#1}}]}
%normalisation rule name
\newcommand{\normaliserulen}[1]{[\underline{{\bf \scriptstyle NORM-}\rulen{#1}}]}
\newcommand{\sarule}[1]{[\underline{{\bf \scriptstyle SA-}\rulen{#1}}]}
\newcommand{\hoareSa}[5]{\ensuremath{\hide{[#1]~}{\vdash}~\{#2\}~{#3}~\{#4,#5\}}}
\newcommand{\pstateN}{\ensuremath{\Delta}}
\newcommand{\prestate}[1]{\ensuremath{\phi_{#1}}}
\newcommand{\pstate}[1]{\ensuremath{\Delta_{#1}}}
\newcommand{\reldef}[1]{\ensuremath{\beta_{#1}}}
\newcommand{\magicW}{\ensuremath{-\!\!{\sep}}}
\newcommand{\imply}{\ensuremath{\Rightarrow}}
\newcommand{\implyLeft}{\ensuremath{\Leftarrow}}
%% \newcommand{\implyeq}{\ensuremath{\Leftrightarrow}}
\newcommand{\implyeq}{\ensuremath{\equiv}}
\newcommand{\conjUnify}{\ensuremath{\Rightarrow_{\wedge}}}
\newcommand{\disjUnify}{\ensuremath{\Rightarrow_{\vee}}}
\newcommand{\eqUnify}{\ensuremath{\Rightarrow_{\equiv}}}
\newcommand{\refBase}{\ensuremath{\Rightarrow_{B}}}
\newcommand{\refCase}{\ensuremath{\Rightarrow_{C}}}
%standard error calculus rule
\newcommand{\entailEC}[4]{\ensuremath{#1 \vdash #2 \,{\sep}\,(#3,#4)}}
\newcommand{\doma}{\ensuremath{\mathcal{D}}}
%error calculus rule name
\newcommand{\ecrulen}[1]{[\underline{{\bf \scriptstyle EC-}\rulen{#1}}]}
\newcommand{\eerulen}[1]{[\underline{{\bf \scriptstyle EE-}\rulen{#1}}]}
\newcommand{\pecrulen}[1]{[\underline{{\bf \scriptstyle SE-}\rulen{#1}}]}
\newcommand{\secrulen}[1]{[\underline{{\bf \scriptstyle SEC-}\rulen{#1}}]}
%reason
%\newcommand{\rn}{\ensuremath{\Re}}
\newcommand{\ern}{\ensuremath{\Re}}
\newcommand{\rn}{\ensuremath{\Psi}}
%residue
\newcommand{\RA}{\ensuremath{\mathcal{R}}}
\newcommand{\DP}{{\cal D}}
\newcommand{\NONE}{{\cal \top}}
\newcommand{\UNK}{U}
\newcommand{\heappred}{heaps}
\newcommand{\UPRE}{\UNK^{pre}}
\newcommand{\UPOST}{\UNK^{post}}
\newcommand{\domE}{\ensuremath{\mathcal{E}}}
\newcommand{\alA}{\ensuremath{\mathcal{A}}}
\newcommand{\funcF}{\ensuremath{\mathcal{F}}}
\newcommand{\enctx}{\ensuremath{\Delta}}
\newcommand{\fss}{\myit{fss}}
\newcommand{\inv}{\myit{invert}}
\newcommand{\ok}{\myit{OK}}
%\newcommand{\ok}{\ensuremath{\surd}}
\newcommand{\may}{\myit{MAY}}
\newcommand{\must}{\myit{MUST}}
\newcommand{\eor}{\ensuremath{\lor}}
\newcommand{\cmblor}{\ensuremath{\vee}}
\newcommand{\cmbblor}{\ensuremath{\bigvee}}
\newcommand{\cmbbror}{\ensuremath{\bigcup}}
\newcommand{\eand}{\ensuremath{\land}}
\newcommand{\elor}{\ensuremath{\sqcup}}
\newcommand{\eland}{\ensuremath{\sqcap}}
\newcommand{\eror}{\ensuremath{\cup}}
\newcommand{\ebigror}{\ensuremath{\bigcup}}
\newcommand{\erand}{\ensuremath{\circ}}
\newcommand{\eunion}{\ensuremath{\cup}}
\newcommand{\ebunion}{\ensuremath{\bigcup}}
\newcommand{\orderF}{\ensuremath{\preceq}}

\newcommand{\flow}{\ensuremath{\tau}}
%\newcommand{\mustF}{\myit{\_\_Error}}
%\newcommand{\mayF}{\ensuremath{\top}}
%\newcommand{\okF}{\myit{\_\_OK}}
\newcommand{\okF}{\ensuremath{\surd}}
\newcommand{\mustF}{\ensuremath{{\mho}_{\scriptsize\it must}}}
\newcommand{\mustFs}{\ensuremath{{\mho}_{\scriptsize\it [must]}}}
\newcommand{\contraFs}{\ensuremath{{\mho}_{\scriptsize\it [contra]}}}
%\newcommand{\mayF}{\ensuremath{\top}}
\newcommand{\mayF}{\ensuremath{{\mho}_{\scriptsize\it may}}}
\newcommand{\mayFs}{\ensuremath{{\mho}_{\scriptsize\it [may]}}}
\newcommand{\botF}{\ensuremath{\bot}}
\newcommand{\topF}{\ensuremath{\top}}
\newcommand{\loopF}{\ensuremath{\infty}}

\newcommand{\subtype}{~\ensuremath{<:}~}

\newcommand{\err}{\ensuremath{\Upsilon}}
%\newcommand{\errt}{\ensuremath{\varsigma}}
\newcommand{\errt}{\ensuremath{\tau}}
\newcommand{\prim}{\ensuremath{\zeta}}

%available set of disjuncts
\newcommand{\availSet}{\myit{L}}
%available set of pruning conditions
\newcommand{\prunSet}{\myit{R}}
\newcommand{\infprun}{{\cal R}}
%singleton separation node
%% \newcommand{\pto}{\mapsto}
\newcommand{\pto}{{\scriptsize\ensuremath{\mapsto}}}
\newcommand{\sepnodeF}[3]{\ensuremath{{#1}{\pto}#2(#3)}}
\newcommand{\sepnode}[3]{\ensuremath{\btt{#1}{\pto}\btt{#2}(\btt{#3})}}
%% \newcommand{\sepnodeC}[3]{\ensuremath{\btt{#1}{\pto}\btt{#2}(\btt{#3})}}
\newcommand{\sepnodei}[3]{\ensuremath{#1{\pto}#2(#3)\btt{@F}}}
%separation predicate
\newcommand{\seppredF}[2]{\ensuremath{#1(#2)}}
\newcommand{\seppred}[2]{\ensuremath{\btt{#1}(\btt{#2})}}
%% \newcommand{\seppredU}[2]{\ensuremath{\btt{#1}(#2)}}
\newcommand{\seppredi}[2]{\ensuremath{#1(#2)\btt{@F}}}
%pruning context (invariant I)
\newcommand{\prunCtx}{\myit{C}}
%improved pruning context (implied,contradicted)
\newcommand{\iprunCtx}{{\cal S}}
%implied by context
\newcommand{\implCtx}{\myit{I}}
% strongly implied by context
\newcommand{\implCtxS}{\ensuremath{\myit{I}_{\myit{S}}}}
% weakly implied by context
\newcommand{\implCtxW}{\ensuremath{\myit{I}_{\myit{W}}}}
%contradicted by context
\newcommand{\contCtx}{\myit{F}}
%pruning condition
\newcommand{\pruncond}[2]{\ensuremath{#1{\leftarrow}#2}}
%retrieving invariant
\newcommand{\retrieveInv}[2]{\ensuremath{{\cal I}nv(#1,#2)}}
\newcommand{\Inv}{\ensuremath{{\cal I}nv}}
\newcommand{\infinv}{\ensuremath{{\cal I}}}
%conjunctive branch
\newcommand{\cbranch}{\sigma}
%label conjunctive branch
\newcommand{\pbranch}[3]{\ensuremath{ {#1}  : {#2} | {#3}}}
%specialised heap
\newcommand{\sheap}{\ensuremath{\hat{\heap}}}
\newcommand{\sbranch}{\ensuremath{\hat{\cbranch}}}
\newcommand{\sD}{\ensuremath{\hat{\D}}}
%% \newcommand\nonterm[1]{\textsf{#1}}
%% \newcommand\term[1]{\textit{#1}}
%% \newcommand\lit[1]{{\bf #1}}
%% \newcommand{\self}{\btt{root}}
%\newcommand{\root}{\btt{root}}
\newcommand{\report}[1]{ }
\newcommand{\techrep}{technical report \cite{Chin:Exc08}}
\newcommand{\paper}[1]{#1}
\newcommand{\acm}[1]{ }
%%%%%%%%%%%%%%%%
\newcommand{\ABS}[1]{{\ensuremath{\large\bf\alpha}}(#1)}
\newcommand{\CONC}[1]{{\ensuremath{\large\bf\gamma}}(#1)}
\newcommand{\St}{{\cal S}}
\newcommand{\DD}{{\cal D}}
\newcommand{\pset}[1]{{\ensuremath{\bf\wp}}(#1)}
\newcommand{\static}{\code{{\bf static}}}
\newcommand{\dynamic}{\code{\bf dynamic}}
%% \newcommand{\hide}[1]{}
\newcommand{\hideie}[1]{}
%% \newcommand{\nil}{\btt{null}}
\newcommand{\res}{\btt{res}}
%% \newcommand{\emp}{\btt{emp}}
\newcommand{\empS}{\ensuremath{\emptyset}}
%% \newcommand{\veq}{\ensuremath{\equiv}}
\def\root{\btt{root}}
%\newcommand{\root}{\btt{root}}
%% \newcommand{\wwith}{\btt{inv}}
\newcommand{\equivimp}{\ensuremath{\Longleftrightarrow}}
\newcommand{\ndet}{\ensuremath{\wedge}}
\newcommand{\puret}{\ensuremath{\pi}}
%% \newcommand{\pure}{\ensuremath{\pi}}
%\newcommand{\simp}{\ensuremath{\textrm{--}\!\btt{*}}}
\newcommand{\simp}{{\bf ;}}
\newcommand{\minv}{\ensuremath{\iota}}
%% \newcommand{\ptr}{\ensuremath{\gamma}}
%% \newcommand{\heap}{\ensuremath{\kappa}}
\newcommand{\Heap}{\ensuremath{\Omega}}
%% \newcommand{\constr}{\ensuremath{\Phi}}
\newcommand{\PP}{\hat{\constr}}
\newcommand{\newconstr}{\ensuremath{\nonterm{Q}}}
%% \newcommand{\pconstr}{\ensuremath{\phi}}
%\newcommand{\sat}[1]{\myit{SAT}(#1)}
\newcommand{\hmodels}[2]{\ensuremath{#1\,{\models}\,#2}}
%% \newcommand{\entail}[2]{\ensuremath{#1{\vdash}#2}}
\newcommand{\entailD}[3]{\ensuremath{#1{\vdash}#2\,{\sep}\,#3}}
%% \newcommand{\entailH}[3]{\ensuremath{#1{\vdash}#2\,{\sep}\,#3}}
%% \newcommand{\entailSA}[5]{\ensuremath{[{#1}]~#2~{\vdash}~#3\,{\yields}\,(#4,#5)}}
\newcommand{\entailSA}[5]{\ensuremath{#2~{\vdash}~#3\,{\yields}\,(#4,#5)}}
%\newcommand{\entailE}[4]{\ensuremath{#2{\vdash}#3\,{\sep}\,#4}}
\newcommand{\entailE}[4]{\ensuremath{#2{\vdash}_{#1}#3\,{\sep}\,#4}}
\newcommand{\entailV}[3]{\entailE{V}{#1}{#2}{#3}}
%% \newcommand{\entailK}[5]{\ensuremath{#3{\vdash}^{#1}_{#2}#4\,{\sep}\,#5}}
\newcommand{\entailKE}[5]{\ensuremath{#3{\vdash}^{#1}_{#2}#4\,{\yields}\,#5}}
%% \newcommand{\entailVV}[3]{\entailK{\heap}{V}{#1}{#2}{#3}}
\newcommand{\entailVVE}[3]{\entailKE{\heap}{V}{#1}{#2}{#3}}
%% \newcommand{\myit}[1]{\textit{#1}}
%% \newcommand{\mytt}[1]{\texttt{#1}}
\newcommand{\U}{\ensuremath{{\btt{U}}}}
\newcommand{\Le}{\ensuremath{{\btt{L}}}}
\newcommand{\Sh}{\ensuremath{{\btt{S}}}}
\newcommand{\SAO}{\ensuremath{{\btt{S}}}}
\newcommand{\UHP}{\ensuremath{{\btt{U}}}}
\newcommand{\FIL}[2]{\ensuremath{{\code{filter}}(#1,#2)}}
\newcommand{\rc}{{\myit{r}}}
\newcommand{\I}{{\myit{I}}}
\newcommand{\M}{{\myit{M}}}
\newcommand{\Li}{{\myit{L}}}
\newcommand{\at}{\btt{@}}
\newcommand{\andthen}{\btt{\small\bf then}}
\newcommand{\thenkey}{\btt{\small\bf then}}
\newcommand{\letkey}{\btt{\small\bf let }}
\newcommand{\inkey}{\btt{\small\bf in}}
\newcommand{\assumekey}{\btt{\small\bf assume}}
\newcommand{\casekey}{\btt{\small\bf case}}
\newcommand{\tranU}{\ensuremath{\,\Longrightarrow_T\,}}
\newcommand{\isview}{\myit{IsView}}
\newcommand{\isdata}{\myit{IsData}}
%% \newcommand{\view}[2]{\ensuremath{\btt{#1}{\langle}{#2}{\rangle}}}
\newcommand{\casetwo}[4]{\ensuremath{\btt{case{\{}}{#1{\Rightarrow}#2}{;}{{~#3{\Rightarrow}}#4}\btt{\}}}}
\newcommand{\casemany}[4]{\ensuremath{\btt{case{\{}}{#1{\Rightarrow}#2}{;\ldots;}{{~#3{\Rightarrow}}#4}\btt{\}}}}
\newcommand{\caseone}[2]{\ensuremath{\btt{case\{}{#1{\Rightarrow}#2}\btt{\}}^*}}
%% \newcommand{\hc}[2]{\ensuremath{{#1}{::}#2}}
%% \newcommand{\hx}[1]{\hc{\code{x}}{#1}}
%\def\sourcelang{\code{Jinja{-}B}}
\def\sourcelang{\code{SrcLang}}
\def\corelang{\code{Core{-}U}}
\def\erule{\ensuremath{\Leftrightarrow}}
\def\trule{\ensuremath{\Rightarrow_T}}
\def\trulefst{\ensuremath{\Rightarrow_{T_1}}}
\def\sep{\code{*}}
\def\sepimpl{\ensuremath{\code{-\!\!\!\!-\!\!\!*}}}
\def\primeV{\myit{prime}}

\mathchardef\mhyphen="2D

%% \newcommand{\rulen}[1]{\ensuremath{{\bf \scriptstyle [#1]}}}
%% \newcommand{\entrulen}[1]{[\underline{{\bf \scriptstyle ENT-#1}}]}
%% \newcommand{\eentrulen}[1]{[\underline{{\bf \scriptstyle EENT-#1}}]}
\newcommand{\saass}[1]{[\underline{{\bf \scriptstyle MIS{\mhyphen}#1}}]}
\newcommand{\synRule}[1]{[\underline{{\bf
\scriptstyle Syn{\mhyphen}#1}}]}
\newcommand{\safvrule}[1]{[\underline{{\bf \scriptstyle SA{\mhyphen}#1}}]}
\newcommand{\norm}[1]{[\underline{{\bf \scriptstyle NORM{\mhyphen}#1}}]}
\newcommand{\htrulen}[1]{[\underline{{\bf \scriptstyle FV-#1}}]}
%% \newcommand{\verirulen}[1]{[\underline{{\bf \scriptstyle FV-}\rulen{#1}}]}
%% \newcommand{\hform}[3]{\ensuremath{{\btt{#1}}{::}{\btt{#2}}{\langle}{\btt{#3}}{\rangle}}}
%% \newcommand{\hformn}[3]{\ensuremath{{\btt{#1}}{\mapsto}{\btt{#2}}{\langle}{\btt{#3}}{\rangle}}}
%% \newcommand{\hformp}[3]{\ensuremath{{\btt{#2}}{\langle}{\btt{#1},\btt{#3}}{\rangle}}}
%% %\newcommand{\pred}[2]{\ensuremath{{\btt{#1}}{\langle}{\btt{#2}}{\rangle}}}
%% \newcommand{\pred}[2]{\seppred{\btt{#1}}{#2}}
%\newcommand{\ptto}[3]{\ensuremath{{\btt{#1}}\,{\mapsto}\,{\btt{#2}}{\langle}{\btt{#3}}{\rangle}}}
%\newcommand{\ptto}[3]{\sepnode{\btt{#1}}{\btt{#2}}{\btt{#3}}}
%% \newcommand{\ptto}[3]{\sepnode{#1}{\btt{#2}}{#3}}
\newcommand{\transit}{\rightarrow}
\newcommand{\arrimp}{\ensuremath{\,\btt{*}\!\!\!\rightarrow}\,}
%% \newcommand{\state}[1]{\ensuremath{{\langle}#1{\rangle}}}
%% \newcommand{\drule}[2]{\ensuremath{\frac{#1}{#2}}}
\def\smallarr{\ensuremath{\hookrightarrow_{s}}}
\def\bigarr{\ensuremath{\hookrightarrow_{b}}}
\newcommand{\bigstep}[2]{\ensuremath{\state{#1}{\bigarr}\state{#2}}}
\newcommand{\smallstep}[2]{\ensuremath{\state{#1}{\smallarr}\state{#2}}}
\newcommand{\multismallstep}[2]{\ensuremath{\state{#1}{\hookrightarrow_{s}^*}\state{#2}}}
\newcommand{\smallbigstep}[2]{\ensuremath{\state{#1}{\hookrightarrow}\state{#2}}}
\newcommand{\dyn}[2]{\ensuremath{\state{#1}{\hookrightarrow}\state{#2}}}
\newcommand{\dyns}[2]{\ensuremath{\state{#1}{\hookrightarrow^*}\state{#2}}}
\newcommand{\dynf}[1]{\ensuremath{\state{#1}{\not\hookrightarrow^*}}}
\newcommand{\dynerr}[1]{\ensuremath{\state{#1}{\hookrightarrow}{\btt{nullErr}}}}
\def\postst{\myit{Post}}



%used in heap constraint solving
\def\rewrite{\leadsto}
%\def\map{\myit{map}}
\def\FV{\myit{FV}}
\def\addr{\myit{addr}}
\def\map{\myit{X{\!}Pure}}
\def\mappair{\myit{X{\!}Pure}_P}
\def\mapview{\ensuremath{\myit{X{\!}Pure}_V}}
\def\mapself{\myit{mapself}}
\def\mapi{\myit{mapI}}
\def\mapviewi{\myit{mapvI}}
\def\mapselfi{\myit{mapsI}}
\def\findu{\myit{find}}
\def\fold{\myit{fold}_V}
\def\foldN{\myit{fold}}
\def\foldK{\myit{fold}^{\heap}}
%% \newcommand{\foldKI}[1]{\myit{fold}^{#1}}
\def\unfold{\myit{unfold}}
\def\alias{\myit{alias}}
\def\merge{\myit{merge}}
\def\overlap{\myit{overlap}}
\def\ex{{\bf ex}}

%def\M{\myit{M}}
%def\C{\myit{C}}
%def\I{\myit{I}}
%def\E{\myit{E}}
%def\A{\myit{A}}
%def\B{{\myit{B}}}
\def\D{\Delta}
%def\S{{\cal S}}
%def\H{{\cal H}}
%def\W{{\cal M}}
%\def\loop{\ensuremath{\alpha}}
\def\myloop{\ensuremath{\alpha}}
\def\arity{\myit{arity}}
\def\max{\myit{max}}
\def\fresh{\myit{fresh}}
\def\where{\btt{where}}
\def\bag{{\cal B}}
\def\bagunion{\sqcup}
\def\bagintersect{\sqcap}
\def\bagsubsume {\sqsubset}
\def\bagsubtract{-}
\def\zerobag{\{{\bf 0}\}}
\newcommand{\load}[1]{\mytt{load}{\langle}#1{\rangle}}
\newcommand{\store}[1]{\mytt{store}{\langle}#1{\rangle}}
%\def\store{\mytt{store}}
%\newcommand{\const}[1]{\mytt{const}{\langle}#1{\rangle}}
%\def\iconst{\mytt{iconst}}
\def\invoke{\mytt{invoke}}
\def\invokeTail{\mytt{invoke}_{Tail}}
\def\new{\btt{new}}
\def\dispose{\btt{dispose}}
\def\bool{\code{bool}}
\def\int{\code{int}}
\def\longint{\code{long}}
\def\float{\code{float}}
\def\double{\code{double}}
\def\fixpt{\myit{fixpt}}
\def\rec{\mytt{Rec}}
\def\void{\code{void}}
\def\type{\myit{type}}
\def\reference{\mytt{ref}}
\def\object{\btt{object}}
\def\objectset{{\rm\bf ObjectType}}
\def\mn{\myit{m}}
\def\F{{\cal F}}%stack frame size
\def\phiinv{\phi_{\myit{inv}}}
\def\phirec{\phi_{\myit{rec}}}
\def\pre{\constr_{\myit{pr}}}
\def\post{\constr_{\myit{po}}}
\def\prehat{\hat{\constr}_{\myit{pr}}}
\def\posthat{\hat{\constr}_{\myit{po}}}
\def\T{\Gamma}%type for the stack frame
\def\eqt{\myit{eq}_\tau}
\def\stk{\pi} %current stack frame
\def\FS{\Pi}  %the stack of frames
\def\true{\code{true}\,}
\def\false{\code{false}\,}
%\def\a{\alpha}
\def\a{a}
\def\restrict{\myit{enrich}}%context enhance
\newcommand{\rulename}[1]{(\sm{#1})}
\newcommand{\parg}[1]{\ensuremath{{\langle}#1{\rangle}}}
\newcommand{\hash}{\ensuremath{{\scriptstyle \#}}}
%\newcommand{\hash}{\ensuremath{{\small \#}}}
\newcommand{\num}[1]{|#1|}
\newcommand{\ifEq}[2]{\mytt{if}~#1~#2}
\newcommand{\whileEq}[1]{\mytt{while}~#1}
\newcommand{\myif}[3]{\code{if}~#1~\code{then}~#2~\code{else}~#3}
\newcommand{\mylet}[3]{\code{let}~#1 \code{=} #2~\code{in}~#3}
\newcommand{\mymethcall}[3]{(#1~\V{#2})~\code{with}~\V{#3}}
\newcommand{\mylambda}[2]{\lambda{#1}.#2} 	
\newcommand{\myblk}[1]{\code{BLK}(#1)}
\newcommand{\mywhile}[2]{\code{while}~#1~\code{do}~#2}
\newcommand{\mydowhile}[2]{\code{do}~#1~\code{while}~#2}
\newcommand{\mytry}[3]{\code{try}~#1~\code{catch}~(#2)~#3}
\newcommand{\mytrytwocatch}[5]{\code{try}~#1~\code{catch}~(#2)~#3~\code{catch}~(#4)~#5}
\newcommand{\mytryfinally}[2]{\code{try}~#1~\code{finally}~#2}
\newcommand{\myfinally}[2]{#1~\code{finally}~#2}
\newcommand{\myty}[1]{\code{ty}(#1)}
\newcommand{\mynew}[1]{\code{new}~#1}
\newcommand{\mybreak}[1]{\code{break}~#1}
\def\mybrk{\code{brk}}
\newcommand{\mylookup}[1]{\code{lookup}#1}
\newcommand{\myreturn}[2]{\code{ret}{-}#1~#2}
\newcommand{\mycoreret}[2]{\code{ret}{-}#1\##2}
\newcommand{\mycontinue}[1]{\code{continue}~#1}
\def\mycont{\code{cont}}
\def\myret{\code{ret}}
\newcommand{\mythrow}[1]{\code{throw}~#1}
\newcommand{\mybind}[3]{\code{bind}~#1~\code{to}~#2~\code{in}~#3}
\def\mybool{\code{bool}}
\def\mynorm{\code{norm}}
\def\myhalt{\code{halt}}
\def\myexc{\code{exc}}
\newcommand{\myEx}[1]{\code{Ex}(#1)}
\newcommand{\escape}[1]{\myit{escape}(#1)}
\def\myIOexc{\code{IOExc}}
\def\myFileIOexc{\code{FileIOExc}}
\def\myint{\code{int}}
\def\mynull{\code{null}}
\def\myString{\code{String}}
\def\myObject{\code{Obj}}
\def\mynullPtr{\code{nullPtrExc}}
\def\myothers{\code{others}}
\def\skipcmd{\mytt{nop}}
%% \newcommand{\defs}{\ensuremath{=_{df}}}
\newcommand{\snd}[1]{\myit{snd}(#1)}
\newcommand{\guarding}{{\ensuremath{\rightarrow}}}
\newcommand{\nonneg}[1]{\myit{notneg}(#1)}
%% \newcommand{\code}[1]{{\small {\ensuremath{\tt #1}}}}
%\newcommand{\sm}[1]{\mbox{$#1$}}
%% \newcommand{\sm}[1]{{\small \mbox{$#1$}}}
%% \newcommand{\btt}[1]{{\ensuremath{\tt #1}}}
%% %\newcommand{\todo}[1]{{\bf(* #1 *)}}
%% \newcommand{\todo}[1]{{\small{{\color{red} TO DO: \textit{#1}}}}}
%% \newcommand{\nodo}[1]{}
\newcommand{\passref}{\btt{ref}}
\newcommand{\pt}{{\ensuremath{\dagger}}}
\newcommand{\defpred}{\btt{pred}}
\newcommand{\deflemma}{\btt{lemma}}
\newcommand{\defprog}{\btt{Prog}}
\newcommand{\ensures}{\btt{ensures}}
\newcommand{\requires}{\btt{requires}}
\newcommand{\infer}{\btt{infer}}
\newcommand{\xpure}[1]{\btt{XPURE}({#1})}
%% \newcommand{\case}{\btt{case}}
\newcommand{\requiresC}{\btt{requires_C}}
%\newcommand{\assumekey}{\btt{assme}}
\newcommand{\NI}{{\sm\hash}}
%% \newtheorem{thm}{Theorem}[section]
%% \newtheorem{lemma}[thm]{Lemma}
\newtheorem{pty}{Property}
%% \newtheorem{cor}[thm]{Corollary}
%% \newtheorem{defn}{Definition}%[section]
%% \newtheorem{idfn}{Informal Definition}
%% \def\proof{\vspace{-0.2cm}\noindent{\bf Proof}\hspace*{0.5cm}}
%\newcommand{\tverb}[1]{\mbox{\verb|#1|}}

%\newcommand{\tcv}[2]{#1\,\vdash\,#2}
\newcommand{\tcv}[3]{#1\,\vdash\,#2,\,#3}
\newcommand{\tcvT}[2]{\tcv{}{#1}{#2}}


%frame bound inference
\newcommand{\fsr}[5]{#1 \vdash_{\small\myit{F}} #2 \rightsquigarrow #3, #4, #5}
\newcommand{\fsinf}[3]{\ensuremath{\frac{\begin{array}{c}[\underline{\rulen{FS-#1}}]\\[0.5ex]
#2\end{array}}{#3}}}
%\newcommand{}[1]{\ensuremath{{\bf \scriptstyle #1}}}

%abstract state inference
\newcommand{\asr}[4]{#1 \vdash_{\small\myit{A}} #2 \rightsquigarrow #3, #4}
\newcommand{\asinf}[3]{\ensuremath{\frac{\begin{array}{c}[\underline{\rulen{AS-#1}}]\\[0.5ex]
#2\end{array}}{#3}}}

%stack space inference
\newcommand{\ssrA}[2]{\ssr{\myit{a}}{#1}{#2}}
\newcommand{\ssr}[3]{#1 \vdash_{\small\myit{S}} #2 \rightsquigarrow #3}
\newcommand{\ssinf}[3]{\ensuremath{\frac{\begin{array}{c}[\underline{\rulen{SS-#1}}]\\[0.5ex]
#2\end{array}}{#3}}}

%heap space inference
\newcommand{\hsrX}[5]{#5,#1 \vdash_{\myit{H}} #2 \rightsquigarrow #3,#4}
\newcommand{\hsr}[4]{\hsrX{#1}{#2}{#3}{#4}{\myit{a}}}
%\newcommand{\hsr}[4]{\myit{a},#1 \vdash_{\myit{H}} #2 \rightsquigarrow #3,#4}
\newcommand{\hsinf}[3]{\ensuremath{\frac{\begin{array}{c}[\underline{\rulen{HS-#1}}]\\[0.5ex]
#2\end{array}}{#3}}}

%op semantics
\newcommand{\oprerr}[5]{\ensuremath{\config{#1}{#2}{#3}{#4}\hookrightarrow #5}}
%\newcommand{\config}[4]{\ensuremath{{\langle}{#1},{#2},{#3},{#4}{\rangle}}}
%\newcommand{\opr}[8]{\ensuremath{\config{#1}{#2}{#3}{#4} \hookrightarrow \config{#5}{#6}{#7}{#8}}}
%\newcommand{\oprd}[4]{\opr{\FS}{#1}{\O}{#2}{\FS}{#3}{\O}{#4}}
%% \newcommand{\config}[4]{\ensuremath{{\langle}{#1},{#2},{#3},{#4}{\rangle}}}
\newcommand{\opr}[8]{\ensuremath{\config{#1}{#2}{#3}{#4} \hookrightarrow \config{#5}{#6}{#7}{#8}}}
\newcommand{\oprd}[4]{\opr{#1:\FS}{\O}{#2}{\ss,\mem}{#3:\FS}{\O}{#4}{\ss,\mem}}
\newcommand{\oprds}[6]{\opr{#1:\FS}{\O}{#2}{\ss,\mem}{#3:\FS}{#4}{#6}{\ss,#5}}
\newcommand{\oprc}[5]{\config{#1}{#2}{#3}{#4}\hookrightarrow^* {#5}}
\newcommand{\oprule}[3]{\ensuremath{\frac{\begin{array}{c}[\underline{\rulen{OP-#1}}]\\[0.5ex]
#2\end{array}}{#3}}}

\def\EI{\epsilon}
\def\G{\Gamma}
\def\S{\Sigma}
\def\Y{\Upsilon}
\def\L{\Lambda}
\def\O{\omega}
\def\i{\iota}
\def\mem{\btt{h}}%available heap space
\def\ss{\btt{s}}%available stack space
\def\MemErr{\btt{MemInadequate}}
\def\OF{\btt{FrameErr}}
\def\cf{\myit{f}}
\def\ret{\btt{ret}}
\def\size{\myit{size}}
\def\cxt{\btt{cxt}}
\newcommand\reqs[4]{\ensuremath{#1 \vdash #2 \rightsquigarrow #3,#4 }}
%% \newcommand\V[1]{\ensuremath{\overrightarrow{#1}}}
\def\asg{:=}


\def\G{\Gamma}
%\def\res{\myit{res}}
%\def\nochange{\myit{no}\!{\cal X}}
\def\nochange{\myit{nochange}}
\def\FSV{\myit{V}}
\def\sep{\ensuremath{*}}
\newcommand\eq[3]{\ensuremath{\myit{eq}_{#1}(#2,#3)}}
\newcommand{\tj}[5]{#1,#2\,{\vdash}\,#3~{::}~#4, #5}
%\newcommand{\tr}[3]{\ensuremath{\frac{\begin{array}{c}[\underline{\rulen{S-#1}}]\\[0.5ex]
%#2\end{array}}{#3}}}
\newcommand{\Dnorm}[3]{\ensuremath{\frac{\begin{array}{c}#1\end{array}}{\begin{array}{c}#2~\Rightarrow~#3\end{array}}}}
\newcommand{\Deq}[2]{\ensuremath{\frac{\begin{array}{c}#1\end{array}}{\begin{array}{c}#2\end{array}}}}
\newcommand{\Dopt}[2]{\ensuremath{\frac{\begin{array}{c}#1\end{array}}{\begin{array}{l}#2\end{array}}}}
\newcommand{\stj}[3]{#1\,{\vdash}\,#2~{::}~#3}
\newcommand{\stjv}[3]{#1\,{\vdash_v}\,#2{::}#3}
%% \newcommand{\trans}[2]{\ensuremath{\begin{array}{l}
%% #1 \\ \trule~#2 \\
%% \end{array}}}
%% \newcommand{\transB}[2]{\ensuremath{\begin{array}{l}
%% #1 \\ \Rightarrow~#2 \\
%% \end{array}}}
%\newcommand{\trans2}[2]{#1 & \Rightarrow~#2 \\}
\newcommand{\gr}[3]{\ensuremath{\frac{\begin{array}{c}\underline{\rulen{#1}}\\[0.5ex]
#2\end{array}}{\begin{array}{c}#3\end{array}}}}
\newcommand{\simpgr}[3]{\ensuremath{\frac{\begin{array}{c}#2\end{array}}{\begin{array}{c}#3\end{array}}}}
\newcommand{\simplegr}[1]{\ensuremath{\begin{array}{c}#1\end{array}}}
\newcommand{\tr}[3]{\ensuremath{\frac{\begin{array}{c}[\underline{\rulen{#1}}]\\[0.5ex]
#2\end{array}}{#3}}}
%% \newcommand{\hlr}[3]{\ensuremath{\frac{\begin{array}{c}\verirulen{#1}\\[0.5ex]%[\underline{\rulen{#1}}]\\[0.5ex]
%% #2\end{array}}{#3}}}
%% \newcommand{\hlrieee}[3]{\ensuremath{\frac{\begin{array}{c}%\verirulen{#1}\\[0.5ex]%[\underline{\rulen{#1}}]\\[0.5ex]
%% #2\end{array}}{#3}}}
\newcommand{\htriple}[3]{\ensuremath{\vdash \{#1\}\,#2\,\{#3\}}}
%\newcommand{\rulen}[1]{\ensuremath{{\bf \scriptstyle #1}}}
\newcommand{\iview}[2]{\ensuremath{#1{\langle}#2{\rangle}}} %use it rather than tt
\newcommand{\ihc}[2]{\ensuremath{#1{::}#2}}                 %use it rather than tt
\newcommand{\subtr}[3]{\entailH{#1}{#2}{#3}}
%\newcommand{\subtr}[3]{\ensuremath{#1\,{\vdash}\,#2,#3}}


%static semantics
\newcommand{\raws}[9]{{#1} ; {#2} ; {#3} ;{#4} \vdash {#5} :: {#6} , {#7},{#8} ,{#9}}
\newcommand{\rawss}[5]{\T ; \D; \L; \Y  \vdash {#1} :: {#2} , {#3}, {#4}, {#5}}

%from sound-cav.tex
\newcommand{\mymodel}{\models}
\def\Flds{\myit{Fields}}
\def\Store{\myit{Heaps}}
\def\StoreType{\myit{HeapType}}
\def\Stack{\myit{Stacks}}
\def\Locations{\myit{Loc}}
\def\Val{\myit{Val}}
\def\Var{\myit{Var}}
\newcommand{\mo}[3]{#1,#2 \mymodel #3}
\newcommand{\notmo}[3]{#1,#2 \not\mymodel #3}
\newcommand{\mos}[1]{\ensuremath{\mo{s}{h}{#1}}}
\newcommand{\mosp}[1]{\ensuremath{{s}\mymodel{#1}}}
\def\iffs{\small \btt{ iff~}}
\def\dom{\myit{dom}}
\def\loc{\iota}
\newcommand{\s}[1]{[\![#1]\!]s}
\def\inv{\bigtriangledown}
\def\getP{\myit{getProperty}}
\newcommand{\view}[2]{\ensuremath{#1{\langle}{#2}{\rangle}}}
\newcommand{\menv}[2]{\frac{\begin{array}{c}#1\end{array}}{#2}}
\def\fresh{\myit{fresh}}
\def\freeze{\myit{\bf freeze}}
\newcommand{\myfreeze}[1]{\ensuremath{\freeze(#1)}}
\def\length{\myit{length}}
\def\Ssub{\ensuremath{\sqsubseteq}}
\def\bagconstr{\varphi}
\def\bag{\ensuremath{\code{B}}}
\newcommand{\atom}{\alpha}
\newcommand{\yields}{\leadsto}
\newcommand{\status}{\Upsilon}
\newcommand{\anon}{\ensuremath{\_\,}}
\newcommand{\unsat}[1]{\bf \footnotesize{\scriptstyle{UNSAT}}(\ensuremath{#1})}
\newcommand{\sat}[1]{\bf \footnotesize{\scriptstyle{NSAT}}(\ensuremath{#1})}
\newcommand{\pureentail}[3]{\ensuremath{#1 ~{\vdash}~ #2 ~{\yields}~ #3}}
\newcommand{\sepentailO}[3]{\ensuremath{#1 ~{\vdash}~ #2 ~{\sep}~ #3}}
\newcommand{\sepentail}[4]{\ensuremath{#1 ~{\vdash}~ #2 ~{\yields}~ (#3,#4)}}
\newcommand{\pureentailT}[3]{\ensuremath{#1 ~{\vdash}_{T}~ #2 ~{\yields}~ #3}}
\newcommand{\ent}{\ensuremath{{\vdash}}}
\newcommand{\entC}{\ensuremath{{\vdash}_{C}}}
\newcommand{\entE}{\ensuremath{{\vdash}_{E}}}
\newcommand{\sepentailC}[4]{\ensuremath{#1 ~{\entC}~ #2 ~{\yields}~ (#3,#4)}}
\newcommand{\pureentailC}[3]{\ensuremath{#1 ~{\entC}~ #2 ~{\yields}~ #3}}
\newcommand{\pureentailE}[3]{\ensuremath{#1 ~{\entE}~ #2 ~{\yields}~ #3}}
% below does not work for verbatim
% \newenvironment{verbtiny}{\begin{scriptsize}\begin{verbatim}}{\end{verbatim}\end{scriptsize}}

\newcommand{\sepentailL}[4]{
\ensuremath{
\begin{array}[t]{l}
{#1} \\
\quad{{\vdash}~ #2} \\
\quad{{\yields}~ (#3)#4}
\end{array}
}
}

\newcommand{\sepentailLS}[2]{
\ensuremath{
\begin{array}[t]{l}
{#1} \\
\quad{{\vdash}~ #2}
\end{array}
}
}

\newcommand{\sepentailCL}[4]{
\ensuremath{
\begin{array}[t]{l}
{#1} \\
\quad{{\entC}~ #2} \\
~{{\yields}~ (#3,#4)}
\end{array}
}
}


\newcommand{\mustmsg}[1]{\ensuremath{\mustF[#1]}}
\newcommand{\maymsg}[1]{\ensuremath{\mayF[#1]}}
\newcommand{\okmsg}[1]{\ensuremath{\okF[#1]}}
\newcommand{\Ra}{\Rightarrow}
\newcommand{\ra}{\rightarrow}

\newcommand{\form}[1]{\ensuremath{\it #1}}
\newcommand{\formC}[1]{\ensuremath{\code{#1}}}
%% \newcommand{\toolname}{{\sc{ShapeInfer}}}
\newcommand{\BugAssist}{BugAssist}
\newcommand{\ShapeSyn}{\textbf{SS}}


%% \newcommand{\ass}{\ensuremath{\longrightarrow}}
\newcommand{\ass}{\ensuremath{\implies}}
\newcommand{\horn}{\ensuremath{\sigma}}
\newcommand{\Horn}{\RA\hide{\mathcal{C}}}
\newcommand{\WHorn}{\mathcal{W}}
\newcommand{\IWHorn}{\mathcal{W_I}}
\newcommand{\IHorn}{\mathcal{C_I}}
\newcommand{\pdef}{\ensuremath{\implies}}
\newcommand{\frm}[1]{\btt{{#1}\btt{@F}}}
\newcommand{\dl}[2]{\btt{DL_{#1}}({#2})}
\newcommand{\hpred}[1]{\code{P}({#1})}
\newcommand{\hpreds}{\mathcal{P}}
\newcommand{\setptr}{\mathcal{S}}
\newcommand{\isetptr}{\mathcal{I}}
\newcommand{\setheap}{\mathcal{K}}
\newcommand{\setpure}{\ensuremath{\gamma}}
\newcommand{\hpredd}{\ensuremath{\Gamma}}
\newcommand{\sheaps}{\ensuremath{h}}
\newcommand{\sstack}{\ensuremath{s}}
\newcommand{\force}{\ensuremath{\models}}
\newcommand{\DL}[1]{\code{DL}(\form{#1})}
\newcommand{\DLl}[1]{\code{DL}^l(\form{#1})}
\newcommand{\DLg}[1]{\code{DL}^g(\form{#1})}
\newcommand{\PTO}[1]{\code{PTO}(\form{#1})}
\newcommand{\NIL}[1]{\code{NIL}(\form{#1})}
\newcommand{\PTR}[1]{\code{PTR}(\form{#1})}
\newcommand{\absd}[1]{\ensuremath{\alpha}(\form{#1})}
\newcommand{\DLsplit}[1]{\code{SPLIT}(\form{#1})}
\newcommand{\DLcomb}[1]{\code{COMB}(\form{#1})}
\newcommand{\reach}{\ensuremath{\bigtriangledown}}
\newcommand{\setvars}[1]{\ensuremath{\bar{#1}}}
\newcommand{\freevars}[1]{\ensuremath{\btt{Vars}({#1})}}
\newcommand{\iniSol}{{\sc{FindIniSol}}}
\newcommand{\cclosue}{{\sc{CClosure}}}
\newcommand{\ewf}{{\sc{ExtrWFC}}}
\newcommand{\cmb}{{\sc{ComC}}}
%% \newcommand{\join}{{\sc{Join}}}
\newcommand{\bounded}[3]{{\code{bounded}}(#1,#2,#3)}
\def\nimply{\centernot\imply}
\def\conju{\xrightarrow{\mbox{\tiny{$\wedge$-unif}}}}
\newcommand{\equu}[2]{\xRightarrow{\mbox{\tiny{$[\btt{#1,#2}]$}}}_{\equiv}}
\newcommand{\equup}[2]{\xRightarrow{\mbox{\tiny{$[#1,#2]$}}}_{\code{P\equiv}}}
\newcommand{\conjut}[5]{\ensuremath{#1 \wedge
#2\conjUnify^{#3}(#4,#5)}}
\newcommand{\disjut}[5]{\ensuremath{#1 \wedge
#2\disjUnify^{#3}(#4,#5)}}
\newcommand{\conjutC}[4]{\ensuremath{#1{\wedge}#2{\conjUnify^{#3}}#4}}
\newcommand{\disjutC}[4]{\ensuremath{#1{\wedge}#2{\disjUnify^{#3}}#4}}
\newcommand{\equtC}[6]{\ensuremath{(\code{#1,#2})\equu{#4}{#5}^{\code{#3}}~\code{#6}}}
\newcommand{\pequtC}[4]{\ensuremath{\code{#1}\equup{\code{#2}}{\code{#3}}~\code{#4}}}
\def\predset{\ensuremath{{\cal P~}}}
\newcommand{\dpsubst}[2]{#2_{[#1]}}
\def\assumpset{\ensuremath{{\cal R}}}
\def\pdefset{\ensuremath{\Gamma}}
\newcommand{\proofsketch}[1]{{\noindent \bf
Proof Sketch\,:~}#1{\QED}}


==> lock.tex <==
%\vspace{-4mm}
\subsection{Locks}% : Concurrency with Cyclic Resources}

Thus far, we have looked at resource predicates with deterministic
flows and those that would transition via a finite number of states,
before they reach a {\RLess} state. We shall now 
look at how flow-aware predicates can be used to model
locks, a concurrency mechanism that may cycle through
its lock/unlock states indefinitely.
%% Moreover, as each lock captures a resource
%% which may be acquired and then released, we shall use a
%% new flow annotation \codeE{\OD} to denote the fact that
%% the resource predicate could support either an 
%% inflow or an outflow request.
%% In the case of lock
%% invariant, we shall use \codeE{\Lock{l}{R}} to denote
%% a lock \code{l} whose resource could either be
%% subjected to an inflow or outflow.
The concept of dynamically allocated locks have been proposed
in \cite{Gotsman:APLAS07,Hobor:thesis2011,Jacobs:POPL11} where
each lock is allowed to carry a resource invariant. We  first see how the same coarse-grained locking mechanism
can be modelled naturally
using flow-aware predicates. More importantly, we shall also
see how we may generalize our flow-aware resource predicate
formalism to support more complex hierarchical and read/write
locks.

%% higher-orderness, where a heap node carries other heap nodes,
%% has been proposed in the literature. Typical examples are 
%% lock nodes that carry
%% the locks' resource invariants 
%% However, thread nodes and lock nodes are fundamentally different.
%% First, locks and threads are used differently.
%% %% a thread having a lock node can obtain the lock's invariant when acquiring the lock, and
%% %% return the invariant when releasing the lock.
%% While the resource inside a lock node can be repeatedly acquired/released,
%% %% after each pair of lock acquisition and release,
%% the resource inside a thread node can be obtained 
%% only once when the thread is joined.
%% Second, unlike the resource in a lock node which is exclusively
%% acquired by a single thread,
%% the resource in a thread node can be split and shared among
%% multiple joiners.

Let us start with a dynamic lock creation method
using:
 %% the following specification:

\code{create\_lock()~\SPEC{with~P}}\\
\indent\quad \SPEC{\requires~\code{P}}
\indent\quad \SPEC{\ensures~ \Lock{res}{P};} %\\

The lock itself is typically implemented in a
global memory,
%% whose access can be 
shared by concurrent threads.
A typical way to split such locks is to perform it fractionally
on the predicate itself, as follows:

%% \begin{verbatim}
%%   // fractional split
%%   Lock(id,.P)@f <--> Lock(id,.P)@f1 * Lock(id,.P)@f2 & f=f1+f2
%% \end{verbatim}

\noindent
\SPEC{\it$\LockF{l}{P}{{\fracperm}} \sm{\longleftrightarrow} \LockF{l}{P}{\fracperm_1} {\sep} \LockF{l}{P}{\fracperm_2} {\wedge} \fracperm{=}\fracperm_1{+}\fracperm_2$}

Note that each fractional permission \code{\fracperm}
is bounded by \codeE{0{<}{\fracperm}{\leq}1.0}.
Such an approach results in a coarse-grained lock that
protects the entire lock invariant.
Concurrency primitive to acquire a lock would reserve the
entire lock invariant for access, and mark it with
the \code{\Held{l}{P}}. In actual implementation,
this is typically done by storing the identity of the 
thread that is holding the lock.

\code{void acquire(l)}\\
\indent\quad \SPEC{\requires~\LockF{l}{P}{\fracperm}}\\
\indent\quad \SPEC{\ensures~ \LockF{l}{P}{\fracperm} {\sep} \code{P} {\sep} \Held{l}{P};} %\\

The \code{release} primitive to surrender a held lock would use
this {\RLoaded}  \code{\Held{l}{P}} predicate to allow 
the resource \code{P} to be
transferred back into the lock invariant.

\code{void release(l)}\\
\indent\quad \SPEC{\requires~\Held{l}{P} {\sep} \code{P}}
\indent\quad \SPEC{\ensures~ \emp;} %\\

Lock disposal itself is straightforward, and could be used
to explicitly release the entire lock.

\code{void dispose(l)}\\
\indent\quad \SPEC{\requires~\Lock{l}{P}}
\indent\quad \SPEC{\ensures~ \UnHeld{l} {\sep} \code{P};} %\\

The termination of lock is marked by the {\RLess} \UnHeld{l} predicate.
Using it, we can easily capture synchronization error
scenarios (including deadlock), with the help of two
lemmas:
%% \begin{verbatim}
%%   Held(l,-P) * UnHeld(l)  --> ERROR
%%   Held(l,-P) * Held(l,-P) --> ERROR (double-lock)
%% \end{verbatim}

\SPEC{\it$\Held{l}{P} {\sep} \UnHeld{l} 
\hide{{\wedge} \codeE{\neg(\code{P}{=}\code{\emp}})}  ~\sm{\longrightarrow}~ \ERR $}

\SPEC{\it$\Held{l}{\codeE{P_1}} {\sep} \Held{l}{\codeE{P_2}} {\wedge} \codeE{UNSAT(P_1{\sep}P_2)}  ~\sm{\longrightarrow}~ \ERR $}

The first lemma detects an intra-lock 
deadlock scenario whereby primitive dispose was
invoked whilst the lock is being held. The second lemma detects a
scenario when the lock is acquired multiple times. We signal this as
an error for non-reentrant locks. 

There are three subtle differences between past proposals on locking
and ours based on flow-aware predicates. Firstly, lock resources 
are now being tracked explicitly and precisely.
Secondly, synchronization errors, such as intra-lock
deadlocks, are
now detected during normalization of
our flow-aware resource predicates. Lastly, the explicit
tracking of resources can help support multiple
reader locks, by using fractional resources, as follows:

\code{void acquire\_read(l)}\\
\indent\quad \SPEC{\requires~\LockF{l}{P}{\fracperm}}\\
\indent\quad \SPEC{\ensures~ \LockF{l}{P}{\fracperm} {\sep} \code{P{\at}{\fracN}} {\sep} \HeldR{l}{P}{\fracN};} %\\


\code{void release\_read(l)}\\
\indent\quad \SPEC{\requires~\HeldR{l}{P}{\fracN} {\sep} \code{P{\at}{\fracN}}}
\indent\quad \SPEC{\ensures~ \emp;} %\\

%\vspace{-2mm}

\input{dead-lock}
\input{h-lock}

\hide{%%%no-need-here%%%

\subsubsection{Soundness}
\label{sec:soundness-lock}

While CDLs are one-off controls that
cannot be reset,
locks are reusable (i.e. one can successively
invoke acquire/release pairs).
Additionally, in contrast to threads whose
states linearly go from \btt{C} (created),
to \btt{F} (forked), and end up
in \btt{D} (dead) state, after created,
locks can alternate indefinitely between the
\btt{H} (held) and \btt{U} (unheld) states.
To ensure deadlock freedom, we will also need to track the
lockset present for each given program fragment, and
then induce \code{wait-for} relation during the
blocking \code{acquire} commands. Any
cycle in this \code{wait-for} would denote a deadlock scenario,
and triggers a fault in the execution. Our soundness proof will
ensure that each proven program never fault (due to deadlock).
%% \khanh{may need to discuss deadlock freedom}

We can show the soundness properties of race-freedom
and resource preservation in our approach
by ensuring that outflow resource obtained by
acquire matches the inflow resource upon
the corresponding release\scnay{one of the two ``outflow'' should be ``inflow''?}. Data race freedom can be guaranteed
by proving that any program state
can be partitioned into those owned
by each thread and each lock.

}%%%end-of-hide-no-need-here%%%

==> model.tex <==
\hide{
General components: Heap - stack

Specific compoents:
 - For thread: threadpool
 - For CountDownLatch: latchmap
 - For lock: lockmap
It's good if we could generalize them
to become resourcemap: thread/latch/locl -> (state x resource)

(assume non-fractional permissions, simple heap object)
}


Our basic memory model is extended from the model
proposed in \cite{Villard:APLAS09}.
In our basic memory model, formulas are interpreted
over the set $\state \in \pstate$, defined as follows:\morespace

$\pstate \defs \pstack \times \pheap \times \pCDL \times \pgraph$

$\pheap \defs \ploc \rightharpoonup \btt{Cell}(\pval)$

$\pstack \defs \pvar \rightharpoonup \pval $

$\pCDL \defs \platch \rightharpoonup \btt{CDL}(\pval \times \boolset \times \inflow \cdlR \times \outflow \cdlR) $

$\pgraph \defs \pset{\platch \times \platch} $
\morespace

$\pstack$ and $\pheap$ capture stack and heap in a program state.
$\pCDL$ captures a set of latches in the state,
while $g \in \pgraph$ captures the state' wait-for graph,
i.e. $g$ represents a directed graph where
$(c_1,c_2) \in g $ when the {\CDL} $c_1$'s
blocking \code{await} operation must complete
before the {\CDL} $c_2$'s count reaches 0.
%% blocking \code{await} to complete first.
In other works, the completion of $c_1$ must be scheduled before 
that of $c_2$.
Let $acyclic(g)$ denote the fact
the graph $g$ is acyclic.
Boolean set: $\boolset \defs \set{\btt{T},\btt{F}}$

The memory model is equipped with a composition law $\circ$ of
a separation algebra defined as follows:
$(s_1,h_1,l_1,g_1)$ $\circ$ $(s_2,h_2,l_2,g_2)$ $\defs$
$(s_1 \uplus s_2, h_1 \uplus h_2, l_1 \circ_l l_2, g_1 \circ_g g_2) $
where $\uplus$ is the disjoint union while
$ l_1 \circ_l l_2$ and $g_1 \circ_g g_2$ are defined below.
We write $\state_1 \# \state_2$ when $\state_1 \circ \state_2 \in \pstate$.
\morespace

\begin{scriptsize}

%RULE1
{\noindent}
$(l_1 \circ_l  l_2)(v) \defs  \btt{CDL}(k_1{+}k_2, b_1 \& b_2, \inflow(\constr_1 {\sep} \constr_2),\outflow(\constr_1' {\sep} \constr_2')) ~~\btt{if}~~ $

\myspace\myspace $l_1(v) {=} \btt{CDL}(k_1,b_1, \inflow \constr_1,\outflow \constr_1')  \wedge l_2(v) {=} \btt{CDL}(k_2,b_2,\inflow \constr_2, \outflow \constr_2')$

\myspace\myspace $\wedge (b1=\btt{F} \vee k_2 {\leq} 0)$

%% %RULE2
%% {\noindent}
%% $(l_1 \circ_l  l_2)(v) \defs  \btt{CDL}(k_1{+}k_2,\outflow(\constr_1 {\sep} \constr_2)) ~~\btt{if}~~$

%% \myspace\myspace $l_1(v) {=} \btt{CDL}(k_1,\outflow \constr_1)  \wedge l_2(v) {=} \btt{CDL}(k_2,\outflow \constr_2) \wedge k_1{+}k_2{\leq}0 $

%% %RULE3
%% {\noindent}
%% $(l_1 \circ_l  l_2)(v) \defs  \btt{CDL}(k_1{+}k_2,\inflow(\constr_2 {\wand} \constr_1)) ~~\btt{if}$

%% \myspace\myspace $l_1(v) {=} \btt{CDL}(k_1,\inflow \constr_1)  \wedge l_2(v) {=} \btt{CDL}(k_2,\outflow \constr_2) \wedge (k_1{\leq}0 \vee k_2{\geq}0) \wedge$ 

%% \myspace\myspace $\constr_2 {\preceq} \constr_1 $

{\noindent}
$(l_1 \circ_l  l_2)(l) \defs  \fault, \myit{otherwise} $

%% {\noindent}
%% $\constr_2 \preceq \constr_1 \defs \exists \constr \cdot \constr_2 \sep \constr {=} \constr_1 $

{~}

{\noindent}
$(g_1 \circ_g  g_2) \defs g_1 {\bagunion} g_2 ~~\btt{if}~~ \myit{acyclic}(g_1 \bagunion g_2)$

{\noindent}
$(g_1 \circ_g  g_2) \defs \fault, ~~\myit{otherwise} $

\end{scriptsize}\morespace

%% \khanh{In other words, for \btt{CDL}, there is never the case
%% that there are more outflow resources than inflow resources.}
%% \khanh{This is the interpretation for the split lemmas}

In the above model, $\pheap$ and $\pstack$ are standard.
$\pCDL$ consists of latches (\btt{CDL}).
A CDL has a value (indicating its count) and
a flow-aware resource $\flow \cdlR$
whose $\cdlR$ is indirectly associated to $\pheap$.
Flow types are defines as: $\flow \defs \inflow \mid \outflow$.
%% \khanh{indeed CDL should refer to a sort R instead
%% of resource R, in order to cut the knot as described
%% in Gotsman APLAS'07. However, we currently ignore that}
Interpretations of important formulas are as follows
($\state$ {=} (s,h,l,g)):



\begin{scriptsize}
\[
\begin{array}{lll}
\!\!\! (s,h,l,g) \models v1 {=} v2 & \!\!\! \!\!\!\btt{iff} \!\!\! 
& v1,v2 \in \myit{dom}(s) \wedge s(v1){=}s(v2) \\

\!\!\! (s,h,l,g) \models \emp & \!\!\! \!\!\!\btt{iff} \!\!\!
& \myit{dom}(h) {=} \emptyset \\

\!\!\! (s,h,l,g) \models \permsto{v1}{\btt{Cell}(v2)}{} & \!\!\!\!\!\! \btt{iff} \!\!\!
& v1,v2 \in \myit{dom}(s) \wedge \myit{dom}(h) {=} \set{s(v)} \\

\!\!\! & &  \wedge h(s(v1)) {=} s(v2)  \\

\!\!\! (s,h,l,g) \models \btt{Latch}(v,\inflow \constr) &\!\!\! \!\!\! \btt{iff} \!\!\!
& v \in \myit{dom}(s) \wedge \myit{dom}(l) {=} \set{s(v1)} {\wedge} \myit{dom}(h) {=} \emptyset   \\
\!\!\! & & {\wedge} \exists k,b \cdot l(s(v)) {=} \btt{CDL}(k,b,\inflow \constr, \outflow \emp) \\

\!\!\! (s,h,l,g) \models \btt{Latch}(v,\outflow \constr) & \!\!\!\!\!\! \btt{iff} \!\!\!
& v \in \myit{dom}(s) \wedge \myit{dom}(l) {=} \set{s(v1)}  {\wedge} \myit{dom}(h) {=} \emptyset  \\
\!\!\! & & {\wedge} \exists k,b \cdot l(s(v)) {=} \btt{CDL}(k,b,\inflow \emp, \outflow \constr) \\

\!\!\! (s,h,l,g) \models \btt{CNT}(v1,v2) & \!\!\! \!\!\!\btt{iff} \!\!\!
& v1,v2 {\in} \myit{dom}(s) {\wedge} s(v1) {\in} \myit{dom}(l)  {\wedge} \myit{dom}(h) {=} \emptyset \\
\!\!\! & &  {\wedge} ({\exists} k,k_1,b,\constr_1,\constr_2 \cdot \\
\!\!\! & &  l(s(v1)) {=} \btt{CDL}(k,b,\inflow \constr_1,\outflow \constr_2) {\wedge} k_1{=}s(v2)\\ 
\!\!\! & & {\wedge} 
       ((k_1{\geq}0 {\rightarrow} k=k1) 
       {\vee} (k_1{<}0 {\rightarrow} b=\btt{T})) )\\

\!\!\! (s,h,l,g) \models \btt{WAIT(S)} & \!\!\!\!\!\! \btt{iff} \!\!\!
& {\forall} v_1{\ra}v_2 {\in} \codeE{S} {\cdot} (s,h,l,g) {\models} \btt{WAIT(\{v_1{\ra}v_2\})}\\

\!\!\! (s,h,l,g) \models  \btt{WAIT(\{v_1{\ra}v_2\})}  & \!\!\! \!\!\!\btt{iff} \!\!\!
& v1,v2 \in \myit{dom}(s) \wedge s(v1),s(v2) \in \myit{dom}(l) \\
\!\!\! & &{\wedge} (s(v1),s(v2)) \in g \wedge \myit{dom}(h) {=} \emptyset ~{\wedge} \\
\!\!\! & &({\exists} k_1,k_2,b_1,b_2,\constr_1,\constr_2,\constr_1',\constr_2' \cdot \\
\!\!\! & & l(s(v1)) {=} \btt{CDL}(k_1,b_1, \inflow \constr_1,\outflow \constr_1') \\
\!\!\! & & {\wedge} l(s(v2)) {=} \btt{CDL}(k_2,b_2,\inflow \constr_2,\outflow \constr_2') \\
\!\!\! & & {\wedge} k_1{>}0 {\wedge} b_2{=}\btt{F}) \\



\!\!\! \state \models {\exists} v {\cdot} \constr & \!\!\!\!\!\! \btt{iff} \!\!\!
& {\exists} v_1 \in \pval \cdot \state \models [v_1/v]\constr \\


\!\!\! \state \models \constr_1 \sep \constr_2 &\!\!\! \!\!\! \btt{iff} \!\!\!
& {\exists} \state_1,\state_2 \cdot \state_1 \circ \state_2 {=} \state ~{\wedge} ~ \state_1  {\models} \constr_1  {\wedge}  \state_2  {\models} \constr_2 \\

\!\!\! \state \models \constr_1 {\wand} \constr_2 &\!\!\! \!\!\! \btt{iff} \!\!\!
& {\forall} \state' \# \state \cdot \state' \models \constr_1 ~\text{implies}~
\state' \circ \state \models \constr_2\\
\end{array}
\]
\end{scriptsize}





==> old-3c-long-interpretation.tex <==
We have introduced three concurrent abstract predicates, namely  \LatchIn{c}{P},  \LatchOut{c}{P} and \CNT{c}{n},
for the specification of {\CDL}, where the first two  carry
some logical resources (\code{P}), and the third one is used to
track the shared counter. A simple
implementation of this {\CDL} concurrency
protocol can be described by the following methods.

%\begin{verbatim}
% CDL newCDL(int n) { i=malloc(1); i.val=n; return i;  }
% void countDown(CDL i) { <if (i.val>0) i.val=i.val-1;> }
% void await(CDL i) { while (i.val>0) skip; }
%\end{verbatim}

$
\begin{array}{l}
\code{{\CDL}\, {\createlatch}(int\, n) \{}
%\\
%\quad
%\code{{\CDL}\, i=malloc(1);\, i.val=n; return i;  \}}
%\code{{\CDL} i = new \CDL(n); return i;  \}}
\code{return new \CDL(n); \}}
\\
\code{void\,countDown({\CDL} i) \{ }
%\\
%\quad
\code{\criticalSec{if (i.val>0) i.val = i.val-1;\hide{else notifyAll();}}\ \}}
\\
\code{void await({\CDL} i) \{ while (i.val>0) skip; \}}
\end{array}
$

%% Take note that the flow-aware resources are
%% phantom resources tha
Of the two concurrent methods, only the {\CD} method
may cause interference. Following \cite{Dinsdale-Young:ECOOP10},
this potential interference
can be described by a {\DEC} action
where the shared global counter \GLOBAL{i}{n}
is decreased by \cc{1} if it is non-zero.

%\begin{verbatim}
%   DEC   : [i->n] & n>0  ~~> [i->n-1]
%         : [i->0]        ~~> [i->0]
%\end{verbatim}

\begin{small}
$
\begin{array}{l}
\DEC: \begin{array}[t]{ll}
\GLOBAL{i}{n}\,{\wedge}\,\code{n{>}0} & \rightsquigarrow \GLOBAL{i}{n{-}1}
\end{array} \\
\end{array}
$
\end{small}

We use this implementation to show how our concurrent abstract
predicates may be defined, and also to illustrate
how the correctness of {\CDL} may be verified.
In the {\CD} method, this action is currently wrapped
by an atomic operation, marked with \code{\criticalSec{$\cdots$}}.
While this \cc{DEC} action is formulated using the global view of
shared counter, it would be better to support
a {\em thread-local} view for such shared counters.
For this, we introduce a new
{\em thread-local} abstraction \LOCAL{i}{n} to denote a
shared counter whose value is always
\cc{n{\geq}0}.
 %% {\em always}.
Such a thread-local 
abstraction is related to its
global counter by the following property.

\begin{small}
$
\LOCAL{i}{n} \longrightarrow \GLOBALF{i}{m}{\code{m}{\geq}\code{n}{\geq}\code{0}}
$
\end{small}
%

%% Based on this thread-local abstraction of the counter, we can 
%% now formalize the \cc{DEC} as a thread-local operation, as follows: 
%% %% \scsay{Should we drop the 2nd line which has no action on local state?}

%% %\begin{verbatim}
%% %   DEC   : {|i->n\} & n>0 ~~> {|i->n-1\}
%% %         : [i->0]         ~~> [i->0]
%% %\end{verbatim}

%% \begin{small}
%% $
%% \DEC: \begin{array}[t]{ll}
%% \LOCAL{i}{n}\,{\wedge}\,\code{n{>}0} & \rightsquigarrow \LOCAL{i}{n{-}1}
%% \\[0.5ex]
%% %% \GLOBAL{i}{0} & \rightsquigarrow \GLOBAL{i}{0}
%% \end{array}
%% $
%% \end{small}

%% As a special case,
%% %% for the count down counter,
%% we also provide a special thread-local view \cc{\LOCAL{i}{-1}}
%% to denote shared counter reaching its final zero state.
%% %%  we shall
%% %% use a special thread-local view:
%% \[
%% \LOCAL{i}{-1} {\eqlr} \GLOBAL{i}{0}
%% \]

%% \hide{
%% To truly two-way conversions between global view
%% and thread-local view, we must attach a permission to
%% each thread-local view and then support the following

For such a thread-local abstraction, we  also
provide the following 
combine/split operations that can be used
to normalize or split thread-local counters.

\begin{small}
$
\LOCAL{i}{n}{\wedge}\code{a,b}{\geq}\code{0}{\wedge}{\code{n=a+b}} ~{\longleftrightarrow}~ \LOCAL{i}{a}{\sep}\LOCAL{i}{b}
$
\end{small}

%% \noindent
Contrast this to the global view of a shared counter with the conjunctive property:

\begin{small}
$
\GLOBAL{i}{a}{\sep}\GLOBAL{i}{b} 
~{\longleftrightarrow}~\GLOBAL{i}{a}{\wedge}\code{a{=}b}
$
\end{small}

\noindent which  signifies that all threads have the same view for the shared counter (the \sm{\longrightarrow} direction) and
 that the global view 
can be  duplicated and shared among threads (the \sm{\longleftarrow} direction).
%% For simplicity, we avoid fractional permission on
%% this thread-local counter, but will instead use exhaustive
%% normalization for thread-local views at each reasoning
%% step, to provide the most accurate thread-local view.
%% The permission on shared counter is thus tracked by
%% the \cc{DEC} action, which can be inter-converted
%% with the global state as follows:

%% \begin{verbatim}
%%     DEC * {|i->a|} & a{>=}0 <-> DEC * [i->a]
%% \end{verbatim}
%% }

%% With this thread-local abstraction, our \cc{DEC} action
%% can now be described by the thread-local actions. 
%% \begin{verbatim}
%%    DEC   : {|i->n|} & n>0  ~~> {|i->n-1|}
%%          : {|i->0|}        ~~> {|i->0|}
%% \end{verbatim}

With this use of thread-local abstraction, we are now ready 
to provide interpretations
for our concurrent abstract predicates that are
stable, as follows:

\begin{small}
$
\begin{array}{lll}
% \LatchIn{i}{P} &\defs & [\DEC]_{\fracpermc} {\sep} {\OM} \code{P} {\sep}\GLOBAL{i}{m} {\wedge}\code{m>0} 
 \LatchIn{i}{P} &\defs &  \code{P}   ~{\septract}~  ([\DEC]_{\fracpermc}  {\sep}\GLOBAL{i}{m} {\wedge}\code{m>0} )
 \\
 \LatchOut{i}{P} & \defs & \GLOBAL{i}{0} {\ourimply} \code{P}
 %lc(i,+R) = R 
\\
\CNT{i}{n} &\defs & \LOCAL{i}{n} {\wedge}\code{n${\geq}$0} ~{\vee}~ \GLOBAL{i}{0}{\wedge}\code{n=-1}
% CNT(i,n) = {|i->n|}&n>0 \/ [i->0] & n=-1
\end{array}
$
\end{small}
\\
We use the {\em septraction} operator \sm{\septract} (\cite{Vafeiadis:CONCUR07}) to specify the
{\em consumption} of resource \code{P} into the {\CDL},  when  \code{countDown(i)} 
is called with  \code{\LatchIn{i}{P}}. 
Note also that we can always attach a fractional permission \sm{\fracpermc} to the {\DEC} action, to signify that
the current thread has permission  \sm{\fracpermc} to perform the action. For ease in presentation, we omit
its tracking at the predicate level.
Our use of \cc{\LOCAL{i}{n}} remains stable since
it is based on the thread-local view. The shared
global state \cc{\GLOBAL{i}{0}} is also stable,
as the \cc{\DEC} operation does not modify this final state
of the shared counter.
The condition \cc{\GLOBALF{i}{m}{m{>}0}} of the shared global state 
in \cc{\LatchIn{i}{P}} is stable since it is always 
used with \cc{\CNT{i}{n}} in the pre-condition
of {\CD} method, which results in
\cc{\GLOBALF{i}{m}{m{>}0}{\sep}\LOCALF{i}{n}{n{>}0}}.
%which is stable, despite interference from
%other
% \cc{\addperm{{[\DEC]}}{\fracperm}}.
%% \wnsay{is LatchOut stable?}
By itself the global view \cc{\GLOBALF{i}{m}{m{>}0}} would not be
stable in the presence of concurrent \cc{\addperm{{[\DEC]}}{\fracperm}}.
However, the combined state 
\cc{\GLOBALF{i}{m}{m{>}0}{\sep}\LOCALF{i}{n}{n{>}0}} would be
stable since the thread-local view of
\cc{\LOCALF{i}{n}{n{>}0}} is not affected
by the  
%% never changed,
%% despite the presence of
concurrent operations \cc{\addperm{{[\DEC]}}{\fracperm}} from 
other threads.
Therefore, \cc{\GLOBALF{i}{m}{m{>}0}} always holds
since \cc{m{\geq}n}.
\LatchOut{i}{P} is stable since it depends
on a pure and stable \GLOBAL{i}{0}.
%% The {\DEC} action taken by {\CD} method
%% can also be denoted using this thread-local abstraction.
%% \begin{small}
%% $
%% \DEC: \begin{array}[t]{ll}
%% \LOCAL{i}{n}\,{\wedge}\,\code{n{>}0} & \rightsquigarrow \LOCAL{i}{n{-}1}
%% \\[0.5ex]
%% %% \GLOBAL{i}{0} & \rightsquigarrow \GLOBAL{i}{0}
%% \end{array}
%% $
%% \end{small}

\dknay{ not sure if \GLOBALF{i}{m}{m{>}0}{\sep}\LOCALF{i}{n}{n{>}0}
is indeed stable, for example:
\[%$
\begin{array}{l}
\GLOBALF{i}{m}{m{>}0}{\sep}\LOCALF{i}{n}{n{>}0}
\\
\Rightarrow
\GLOBALF{i}{m}{m{>}0}{\sep}
\GLOBAL{i}{m} {\wedge} m{\geq}n{>}0
\\
\Rightarrow \GLOBALF{i}{m}{m{\geq}0}
\end{array}
\]%$
\GLOBALF{i}{m}{m{>}0} is exactly the LHS of the action DEC,
hence it is not stable under the interference of DEC.
 }
\wnnay{Above do not hold due to thread-local
{|i->n|} that is not affected by other threads}

For the purpose of creating and later destroying this
shared global counter, we provided another action, called \cc{\KILLR} action, 
that allows a global counter to be made local by
the following equivalence lemma:
%% \scsay{Is \sm{\PointTo{i}{n}} below a heap formula?
%% It's a bit confusing here as we have both global/local points-to. If it's meant for heap representation,
%% perhaps we should use \sm{i{\mapsto}\CDL(n)}?}
%% \scsay{Is the following correct?}
%\begin{verbatim}
%   i->a & a>=0 <-> DEC*{|i->a|}
%\end{verbatim}
\begin{small}
$
\begin{array}{l}
\KILLR: \begin{array}[t]{ll}
\addperm{\KILLR}{1} \,{\sep}\,\addperm{\DEC}{1} \,{\sep}\, \GLOBAL{i}{n} & \rightsquigarrow \PointTo{i}{\CDL(n)}
\\[0.5ex]
%% \GLOBAL{i}{0} & \rightsquigarrow \PointToF{i}{\CDL(n)}
\end{array}
\end{array}
$
\end{small}
\scsay{I don't quite get the above: it looks like an action definition for KILL but KILL itself is used in it; if it's an equivalence
lemma, then maybe we should use \sm{\longleftrightarrow}? For the latter case, do we need to give the action definition of KILL?}

\noindent 
Our action is a generalization of \cite{Dinsdale-Young:ECOOP10}, as
it allows both local and shared states in 
its transitions.
This action is also supported by
the following equivalence lemma:

\begin{small}
\[
%\PointToF{i}{n}{\code{n}{\geq}\code{0}}
\begin{array}{ll}
\PointToF{i}{\CDL(n)}{\code{n}{\geq}\code{0}}
 & {\longleftrightarrow}~ \addperm{{[\DEC]}}{1} {\sep}
\addperm{{[\KILLR]}}{1} {\sep}  \GLOBALF{i}{n}{\code{n}{\geq}\code{0}} \\
& {\longleftrightarrow}~
\addperm{{[\DEC]}}{1} {\sep} \addperm{\LOCAL{i}{n}}{1} {\sep} \GLOBAL{i}{n}%% {\code{n}{\geq}\code{0}}
\end{array}
\]
\end{small}

This {\KILLR} action permits the creation of
a thread-local heap state.
By tracking the permissions of both \cc{\DEC} action
and thread-local counter, 
we could recover the full permission needed for the 
thread-local counter to be converted to
just the global view, prior to its
conversion back to a local heap for
explicit disposal.

\input{read-3f-compare-fictional}


==> proglang-locks.tex <==
\begin{figure}[!htb]
%% \savespace
%% \savespace
%% \savespace
%% \savespace
\begin{center}
\begin{minipage}{22pc}
\begin{frameit}
\savespace
%% \savespace
%% \savespace
\[
\begin{array}{rlll}

\morespace

\nonterm{type} & ::= & \ldots \mid \code{lock} & \textsf{Type}\\

\nonterm{stmt} & ::= &
	\begin{array}{ll}
	
	& \hspace{-2.3mm} \nonterm{v} = \lit{new} ~ \code{lock} \lit{(} \lit{)} \\

	\mid &  \lit{acquire} \lit{(} \nonterm{v} \lit{)} \mid 
        \lit{release} \lit{(} \nonterm{v} \lit{)}~~~~~ \\

        \mid & \ldots \\ 
			
	\end{array} & \textsf{Statement}		

\end{array}
\]
%% \savespace
%% \savespace
\end{frameit}
%\savespace
\savespace
\caption{Added Language Components for Manipulating Locks}
\label{fig.proglang-locks}
\end{minipage}
\savespace\savespace
\savespace\savespace
\savesmallspace
\end{center}
\end{figure}


==> proof.tex <==
\hide{
Soundness of each primitives with respect to
their specification.

Properties:

(1) race free

(2) resource reservation (no leak) by imposing restrictions
on the specifications.

(3) deadlock free: need a way to construct wait-for graph based on traces.

We need to distinguish (i) predicate transformer
(ii) asyn transfer (iii) write to global memory.

} %% END HIDE


\paragraph{Semantics of Programs}

The semantics $\interpret{c}$ : $\fpstate \rightarrow \pset{\fpstate}^{\!\top}$ 
of a primitive command $c$ is defined
as the best local action
of a specification $\fpspec$ over $\fpstate$.
The best local action of $\fpspec$ is defined as:
\[
bla[\fpspec](\fstate) \defs \bigsqcup_{\fstate' \preceq \fstate, \fstate' \in A, (A,B) \in \fpspec} \set{\fstate - \fstate'} \sep B
\]
For most of the primitives, the specification $\fpspec$ 
is just the specification $\pspec$ given in the proof
system, interpreted over $\fpstate$ in straightforward manners.
Only primitives such as \code{\createlatch}, \code{countDown}, and
\code{await} need to deal with flow-aware tags.

\input{refined-axioms}

The axioms presented in Section~\ref{sec:latch} are called
coarse axioms. Here we present refined ghost axioms which
implement the coarse axioms.
The refined axioms are presented
in Fig.~\ref{fig:refined}.
Refined ghost axioms are provided during the verification
process in order to provide additional information
about the flow-ware resource $\btt{P}$
associated to each latch $\btt{c}$.
The semantics for coarse axioms
such that \code{\createlatch(c)}, \code{countDown}, and \code{await}
are more complicated with ghost parameter \code{P},
%% and compose of ghost primitives,
defined as follows:

\begin{small}
\begin{equation*}
\begin{array}{l}

\code{\createlatch(c,P)} \defs 
\code{atomic} \{ \code{c=create(\btt{n},\btt{P});} \} \\

\\
\code{countDown(c,P)} \defs 
\code{atomic} \{ \\
\myspace \code{if (c.count > 0) \{ c.count=c.count-1; inflow(c,\btt{P})};\}
\} \\

\\

\code{await(c,P)} \defs 
\code{atomic} \{ \\
\myspace \code{if (c.count = 0) \{ c.count=c.count-1; outflow(c,\btt{P});}\}
\}
\end{array}
\end{equation*}
\end{small}

The semantics for \code{\createlatch} is the simplest.
When creating a new CDL with account \btt{n} and the resource
\btt{P}, a new fresh identifier $c$ is created.
The identifier will later be used to tag
the heap that flows via the latch.
The $\code{inflow}$ ghost primitive consumes the inflow resource \btt{P},
and logs the state being acquired
with the inflow tag (i.e. $\langle \inflow \mytag \rangle \fstate $).
Similarly, the $\code{outflow}$ ghost primitive introduces
the outflow resource \btt{P},
and logs a copy of the state being introduced.
In the code,
$\code{c.count}$ gets the count \btt{n} locally captured
in \btt{CNT(c,n)}.

\paragraph{Soundness}

Since the soundness of the whole proof system
is established by the sole soundness of
all primitives, we establish the soundness
of the primitives with respect to their corresponding
ghost primitives' axioms.

\begin{mydef}[Implementation]
A specification $\fpspec$ over $\fpstate$ implements
a specification $\pspec$ over $\pstate$
if $\forall (\constr_{pr},\constr_{po}) \in \pspec \cdot \exists ({\hat \constr_{pr}},{\hat \constr_{po}})
\in \fpspec, \myit{now}^{-1}(\constr_{pr}) \sqsubseteq {\hat \constr_{pr}} \wedge
\myit{now}({\hat \constr_{po}}) \sqsubseteq \constr_{po}$.
\end{mydef}

\begin{lmm}[Soundness of Implementation]
For all local function $f$,
if $\fpspec$ implements $\pspec$ and
$f \models \fpspec$, then $f \models \pspec$.
\end{lmm}

\begin{lmm}[Soundness of CDL Primitives]
Given a primitive $P$ with 
its corresponding pre/post-conditions ($\constr_{pr}$/$\constr_{po}$), for all $\fstate, now(\fstate) \models \constr_{pr}$ implies
$now(\interpret{P}(\constr_{pr})) \sqsubseteq \constr_{po}$.
\end{lmm}

We can show that the refined ghost axiom for \code{\createlatch} directly
implement its corresponding coarse axiom.
The refined sub-primitives composed together can be shown to
derive the \code{countDown} and \code{await} coarse axioms.
Based on abstract separation logic, we can conclude
that the proof system proposed in Section~\ref{sec:latch}
is sound.

\begin{thm}[Soundness of Flow-Aware Resource Predicates for CDL]\label{thm:tar-sound}
Given a program with a set of procedures and primitives $P^i$ together with 
their corresponding pre/post-conditions ($\constr_{pr}^i$/$\constr_{po}^i$),
$\vdash$ \{$\constr_{pr}^i$\}$P^i$\{$\constr_{po}^i$\} implies $\models$ \{$\constr_{pr}^i$\}$P^i$\{$\constr_{po}^i$\}.
\end{thm}

It is easily derived from the theorem that
every provable program is race-free and
deadlock-free, since
the semantics is based on race-free
and deadlock-free traces.
Any racy or deadlocked traces will be forced to fault.
%% \khanh{due to norace() in trace}
%% Provable program is also non-blocking
%% with respect to each CDL, since
%% program states are restricted to only
%% legal states with respect to each tag
%% (each CDL has a unique tag).
%% \khanh{hopefully able to prevent these as illegal traces}
It also follows that if the specification of
the main procedure is 
\{$\emp$\} \code{main()} \{$\emp$\},
the program is leak-free. This is due to
the fact that, in our model, well-formed
tagged memory states respect resource preservation.
%% \khanh{due to resource preservation, needed to be defined}


==> read-3g-flow-awareness.tex <==
\subsection{Importance of Flow-Annotation}

Flow-annotation is important to support sound communications in
concurrency control mechanisms.
As a simple example, consider a latch that is being used as a channel to pass some heap
node with property \sm{\code{x}{\mapsto}\code{cell(v)} {\wedge} \code{v{>}2}}
from a sender process to another process, acting
as a receiver.

\hide{
\begin{verbatim}
 l = create_latch(1) with x::cell<v> & v>2
 x=new cell<5>    ||  await(c)
 countDown(c)     ||  assert x::cell<v> & v>1
\end{verbatim}
}

\begin{center}
\begin{small}
\code{c = \createlatch(1) ~with}~~\SPEC{\code{x}{\sm{\mapsto}}\code{cell(v)} \sm{\wedge} \code{v{>}2}}
\\
\vspace{-8pt}
\[
{
\left(
\begin{tabular}{ l@{\extracolsep{\fill}}  || l@{\extracolsep{\fill}} }
\code{x = new cell(5);~~} &~~\code{await(c);}\\
\code{countDown(c)} &~~\code{assert}~\SPEC{\code{x}\sm{\mapsto}\code{cell(v)} \sm{\wedge} \code{v{>}1}}\\
\end{tabular}\right)
}
\]
\end{small}
\end{center}



This communication essentially sends a cell with value 5
to a process that is expecting a cell with value greater
than 1. Automated verification is capable of supporting
such formal reasoning. Consider now the scenario, where one would like to
write procedures for both the sender and receiver threads,
as follows, where the {\CDL} itself is being passed as a 
parameter.

\hide{%
\begin{verbatim}
 void sender(c,x)
  requires c::Latch{-x::cell<5>}*c::CNT<n> & n>0
  ensures  c::CNT<n-1>
 {
    x = new cell<5>;
    countDown(c);
 }
 void receiver(c,x)
  requires c::Latch{+x::cell<v>&v>1}*c::CNT<0> 
  ensures  c::CNT<-1>*x::cell<v> & v>=1
 {
    await(c);
 }
\end{verbatim}
}%

\[
\begin{array}{l}
\code{void~sender(\CDL~c, cell~x)}\\
\indent\quad \SPEC{\requires~\LatchIn{c}{x\sm{\mapsto}cell(5)}{\sep}\code{CNT(c,n)}\sm{\wedge}\code{n{>}0}}\\
\indent\quad \SPEC{\ensures~ \code{CNT(c,n{-}1)}};\\ 
\code{\{}
\\
\qquad \code{x = new cell(5);}
\\
\qquad \code{countDown(c);}
\\
\code{\}}
\end{array}
\]

\[
\begin{array}{l}
\code{void~receiver(\CDL~c, cell~x)}\\
\indent\quad \SPEC{\requires~\LatchOut{c}{x\sm{\mapsto}cell(v)\sm{\wedge}v{>}1}{\sep}\code{CNT(c,0)}}\\
\indent\quad \SPEC{\ensures~ \code{CNT(c,{-}1)}{\sep}\code{x}\sm{\mapsto}\code{cell(v)} \sm{\wedge} \code{v\sm{\geq}1}};\\ 
\code{\{}
\\
\qquad \code{await(c);}
\\
\code{\}}
\end{array}
\]


%sender(c,x)  || 
Modular verification for the two methods can easily proceed.
However, we also need a
more systematic method to pass latch as first-class
citizens. Our new program would look like:

\hide{
\begin{verbatim}
 l = create_latch(1) with x::cell<v> & v>2
 // l::Latch<-x::cell<v> & v>2> 
 // * l::Latch<+x::cell<v>& v>2> * l::CNT<1>
 sender(l,x)   ||  receiver(l,x)
\end{verbatim}
}
\begin{center}
\begin{small}
\code{c = \createlatch(1) ~with}~~\SPEC{\code{x}{\sm{\mapsto}}\code{cell(v)}{\sm{\wedge}}\code{v{>}2}}
\\
%% \code{\CSPEC
%% {\LatchIn{c}{\code{x}{\sm{\mapsto}}\code{cell(v)}{\sm{\wedge}}\code{v{>}2}} {\sep}
%%     \LatchOut{c}{\code{x}{\sm{\mapsto}}\code{cell(v)}{\sm{\wedge}}\code{v{>}2}} {\sep} CNT(c,1)}}
%% \\
\vspace{-8pt}
\[
{
\left(
\begin{tabular}{ l@{\extracolsep{\fill}}  || l@{\extracolsep{\fill}} }
\code{sender(c,x);~~} &~~\code{receiver(c,x);}\\
\end{tabular}\right)%\code{;}
}
\]
\end{small}
\end{center}

When dealing with the sender process, we encounter the
following entailment which exploits
the contravariant subsumption that is induced
by the \sm{\OM} annotation. 
%
\hide{
\begin{verbatim}
    x::cell<5> |- - x::cell<v> & v>2 
   -----------------------------------
   - x::cell<v> & v>2 |-  -x::cell<5>
 ----------------------------------------------------
  l::Latch<-x::cell<v> & v>2> |- l::Latch<-x::cell<5>
\end{verbatim}}
\[
\begin{array}{c}
\begin{array}{c}
\entailS{\code{x\sm{\mapsto}cell(5)}}{\OM\code{x\sm{\mapsto}cell(v)}{\wedge}\code{v{>}2}}
\\
\hline
\entailS{\OM\code{x\sm{\mapsto}cell(v)}{\wedge}\code{v{>}2}}{\OM\code{x\sm{\mapsto}cell(5)}}
\end{array} \\
\hline
\entailS{\LatchIn{c}{\code{x\sm{\mapsto}cell(v)}\sm{\wedge}\code{v{>}2}}}{\LatchIn{c}{\code{x\sm{\mapsto}cell(5)}}}\\
\end{array}
\]

Similarly, when dealing with the receiver process, we meet with the
following entailment where covariant subsumption is required.
\hide{
\begin{verbatim}
    x::cell<v> & v>2 |-  x::cell<v> & v>1
   -----------------------------------
   + x::cell<v> & v>2 |-  +x::cell<v> & v>1
 ----------------------------------------------------
  l::Latch<+x::cell<v> & v>2> |- l::Latch<+x::cell<v> & v>1
\end{verbatim}}
\[
\begin{array}{c}
\begin{array}{c}
\entailS{\code{x\sm{\mapsto}cell(v)}\sm{\wedge}\code{v{>}2}}{\code{x\sm{\mapsto}cell(v)}{\wedge}\code{v{>}1}}
\\
\hline
\entailS{\OP\code{x\sm{\mapsto}cell(v)}\sm{\wedge}\code{v{>}2}}{\OP\code{x\sm{\mapsto}cell(v)}{\wedge}\code{v{>}1}}
\end{array} \\
\hline
\entailS{\LatchOut{c}{\code{x\sm{\mapsto}cell(v)}\sm{\wedge}\code{v{>}2}}}{\LatchOut{c}{\code{x\sm{\mapsto}cell(v)}\sm{\wedge}\code{v{>}1}}}\\
\end{array}
\]

Without such flow-annotation, we would not be able
to deal so readily with first-class latches that are
being passed as parameters to methods, or stored
inside data structures. The flow annotations are
extremely important to help reason soundly with
concurrent programs.




==> read-3h-type-resource.tex <==
\subsection{Types of Resources}

Apart from heap nodes and their properties and permissions, we can
also pass variables as resources
%% and their properties and permissions
into flow-aware predicates. Such passing of
resources into concurrency mechanisms are
important to ensure race-freedom and
resource-preservation. Let us look at
the \CDL example in Fig~\ref{fig:latch_wait_for_consume}, where 
\sm{T_1} and \sm{T_2} have been invoked to
compute values for variables \code{h} and \code{r}
respectively. These two pieces of information would later
be read by process \sm{T_3}, so as to compute the
volume \code{V}. For this example, our latch can be 
used to pass the entire variable permissions for both
\code{h} and \code{r}, as follows:

%% \begin{verbatim}
%%  c = create_latch(2) with h*r
%% \end{verbatim}
\[
 \code{c = create\_latch(2) with}~\code{h}_{1}{\sep}\code{r}_{1}
\]

Alternatively, since \code{h,r} are only used in read-mode,
we could also pass a fractional permission, as follows:

\[
 \code{c = create\_latch(2) with}~\code{h}_{\frac{1}{2}}{\sep}\code{r}_{\frac{1}{2}}
\]


This would allow the sending processes \sm{T_1} and \sm{T_2}
to continue to have shared read privileges for the computed
\code{h} and \code{r}, respectively.



==> refined-axioms.tex <==
\begin{figure*}%[b]
\begin{center}
\begin{minipage}{30pc}%{42pc}
\begin{frameit}

\begin{small}
\savespace
\savespace
\savesmallspace
\begin{equation*}
\begin{array}{c}
\frac{
\begin{array}{c}
\myit{fresh}~\code{c}
\end{array}
}
{
\begin{array}{c}
\{ \emp {\wedge} n{>} 0 \} 
\myit{\btt{c}=create}(\btt{n},\btt{P})
\{ \LatchIn{c}{P} {\sep}\LatchOut{c}{P}{\sep}\code{CNT(c,n)} \}
\end{array}
}\\

\\

\frac{
\begin{array}{c}
\fstate \models \LatchIn{c}{P} \sep \btt{P}
\end{array}
}
{
\begin{array}{c}
\{ \fstate \} 
\myit{inflow}(\btt{c},\btt{P})
\{ \langle \inflow \mytag \rangle \fstate \}
\end{array}
}%\\

\qquad%\\

\frac{
\begin{array}{c}

\fstate \models \LatchOut{c}{P}\quad
\code{P} \sqsubseteq \langle \now \sep \outflow \! \mytag \rangle \fstate
\end{array}
}
{
\begin{array}{c}
\{ \fstate \} 
\myit{outflow}(\btt{c}, \code{P})
\{ \langle \now \sep \outflow \! \mytag \rangle \fstate \}
\end{array}
}\\

\end{array}
\end{equation*}
\end{small}

\end{frameit}
\savesmallspace
\caption{Refined Axioms}\label{fig:refined}
\end{minipage}
%\savespace%
\savespace
\end{center}
\end{figure*}


==> related-more.tex <==

Traditional works on concurrency verification
such as
Owicki-Gries \cite{Owicki:CACM76} and
Rely/Guarantee reasoning \cite{Jones:IFIP83}
have often concentrated
on the simple parallel composition, rather than fork/join.
The fork/join concurrency is more general than
the parallel composition for two main reasons.
First, fork/join supports dynamic thread creation
and termination. Second, while threads in a parallel composition
are lexically scoped, threads in fork/join programs are
non-lexically scoped.
Therefore, fork/join programs are
more challenging for verification.
Even recent approaches such as CSL \cite{OHearn:CONCUR04},
SAGL \cite{Feng:ESOP07}, RGSep \cite{Vafeiadis:CONCUR07},
LRG \cite{Feng:POPL09}, CAP \cite{Dinsdale-Young:ECOOP2010},
and Views \cite{Dinsdale-Young:POPL2013},
omit fork/join concurrency from their languages.
Our ``threads as resource'' is complementary to
the above approaches
and hence can be integrated into them
for verifying fork/join programs.

There also exists approaches that can handle fork and
(possibly) join operation. Both Hobor et al. \cite{Hobor:ESOP2008},
and Feng and Shao \cite{Feng:ICFP2005}
support fork and omit join with the claim that
thread join can be implemented using synchronization. 
However, without join, the former allows threads
to leak resources upon termination
while the latter requires global specification of
inter-thread interference.
Approaches that can handle both fork and join can
be grouped into those modeling
threads as unique tokens \cite{Gotsman:APLAS07,Jacobs:POPL11,Leino:ESOP2010}
and those modelling threads as \lit{and}-conjuncts
\cite{Le:ICFEM2012,Le:ATVA13}.
Though syntactically different, they are semantically similar
in that the tokens and the \lit{and}-conjuncts are used
to specify the post-states of forked threads.
However, they are often used in a very limited way:
they are created once when fork, transfered as a whole,
and joined once when join.
As such, they are insufficiently flexible
to verify programs with more intricate fork/join
behaviors such as the multi-join patterns.
Inspired by the key notation of resource in separation
logic \cite{Bornat:ENTCS06,OHearn:CONCUR04}, we propose
to model threads as resource, thus allow ownerships
of threads to be flexibly split and distributed
among multiple joiners.
This enables verification of the intricate
multi-join pattern as well as helps improve
the delayed lockset checking technique.
To the best of our knowledge, only 
Haack and Hurlin \cite{Haack:AMAST08}
can reason about some multi-join scenarios.
In their approach, a thread token can be
associated with a fraction and this allows
multiple joiners to join with the same joinee
in order to read-share the joinee's resource.
However, this simple multiplicative treatment
of thread tokens is not as expressive as our
``threads as resource'' as
it is unable to verify programs that require
the joiners to write-share resource of
the joinee such as that in Fig~\ref{fig.example}.

\hide{
Most existing work consider thread as a unique token, hence
do not support reasoning about complicated join patters.
We consider threads as resource, hence, threads (more precisely
post-state of threads) can be flexibly split and distribute among
multiple joiners.

Represent thread as tokens and only one thread can hold
a token in order to join with the thread.

Oracle semantics does not support join() operation.
Gotsman et al., Verifast and Chalice consider threads as tokens
which are transfered as a whole and joined once.
Our previous works (VPERM and ParaHIP)
represent threads as a separation and-conjunct
and threads are also transfered as a whole and joined once.

Approaches to model concurrent threads:
(1) threads as tokens and (2) threads as AND-conjuncts.
They share the same idea that threads are considered as
linear resource, can only be forked and joined once.

\todo{TODO: mention Haack and Hurline \cite{Haack:AMAST08}. They
briefly mention that thread tokens can be fractional
in order to allow multi join. They do not give any
concret example. They are not flexible enough to
handle the program in Fig.1.}

Distinguish ours from nested fractional permissions.
}

\hide{
- parallel composition -> syntatically scope. Limit by non lexical or nested fork/join/thread creation.. Owicki-Gries, CSL, Smallfoot.
They do not support dynamic thread creation and termination.''


More recent works such as RGSep \cite{Vafeiadis:CONCUR07},

\cite{Fu:tase09}: parallel composition.

LG: CAP: parallel composition

iCAP and HOCAP seems to support fork concurrency only.

VIEWs: parallel composition.

SAGL \cite{Feng:ESOP07} :
``The PROG rule of our CSL corresponds to O’Hearn’s parallel composition rule [11].
The number of threads in our machine is fixed, therefore the nested parallel composi-
tion statement supported by Brookes [2] is not supported in our language. We studied
verification of assembly code with dynamic thread creation in an earlier paper [5].''
In [5]:
``The “fork/join” thread model is more general than “cobe-
gin/coend” in that it supports unbounded dynamic thread cre-
ation, which poses new challenges for verification. To our
knowledge, our work is the first to successfully apply the rely-
guarantee method to verify concurrent programs with dynamic
thread creation and termination.''
``we collect all dynamic threads into a single environment
(i.e., the dynamic thread queue) and reason about the envi-
ronment’s assumption and guarantee requirements as a whole.''

DG: thread carry interference (as resources).
``Related work Other work on concurrency verification has generally ignored fork/join,
preferring to concentrate on the simpler case of parallel composition. This is true of all
of the work on traditional rely-guarantee reasoning [10, 11]. This is unsurprising, as the
development of deny-guarantee depends closely on the abstract characterization of sep-
aration logic [3]. However, even approaches such as SAGL [5] and RGSep [12] which
combine rely-guarantee with separation logic omit fork/join from their languages.
There exist already some approaches to concurrency that handle fork. Feng et al. [6]
and Hobor et al. [9] both handle fork. However, both omit join with the justification
that it can be handled by synchronization between threads. However, this approach
is not compositional: it forces us to specify interference globally. Gotsman et al. [7]
propose an approach to locks in the heap which includes both fork and join. However,
this is achieved by defining an invariant over protected sections of the heap, which
makes compositional reasoning about inter-thread interference impossible (see the next
section for an example of this). Haack and Hurlin [8] have extended Gotsman et al.’s
work to reason about fork and join in Java, where a thread can be joined multiple times.''

LG:

View, ..., are based on CSL and thus they do not support
dynamic thread creation. => hence complementary to our ``threads as resource''.


-  Following CSL, ... for fork/join concurrency or dynamic thread creation 
}


==> sec-5-ent-rule.tex <==
%\vspace*{-4mm}
\begin{small}
\begin{equation*}
\frac{
\begin{array}{c}
\entrulen{[RP-MATCH]}\\
\rho = [\vlist{v}_1 / \vlist{v}_2]

\quad

(\rsrvar, \fann \constr_{3}, \D, \code{b}) {=} 
\myit{addVar}(\rpreds{\btt{R}}{\code{x}, \fann (\rho(\constr_{2})),\vlist{v}_1})
\\
%\quad
\entailAnyVHO
    {\constr_{1}}%1
    {\constr_{3}}%2
    {\hvardef}%3
    {E \cup \{\rsrvar\}}%4
%
\quad%\\

%\hvardef_1 \defs \{ (\rsrvar, \D_{\rsrvar} \wedge \myit{freeEqn}(\rho,\rsrvar) \mid (\rsrvar, \D_{\rsrvar}) \in \hvardef  \}

%\qquad

\D_1 {=} \myit{subst}(\hvardef, \heap_1 {\wedge} \pure_1)

\\
%\quad

\D_2 {=} \myit{subst}(\hvardef, \D)

\quad 

\D_3 {=} \myit{subst}(\hvardef, \rho(\heap_2 {\wedge} \pure_2))

%\qquad
\\

\entailC{E \bagsubtract \{\vlist{v}_2\}}
	{\D_1 \sep \D_2 \wedge \myit{freeEqn}(\rho,E)}
	{\D_3}
  {(\hvardef_1,\D_4)}
  
\\

\hvardef_2 {=} \code{if b then} ~ \hvardef_1 ~ \code{else} ~ \hvardef \cup \hvardef_1

\end{array}
}
{
  \entailCV
      {\rpreds{\btt{R}}{\code{x}, \fann \constr_{1}, \vlist{v}_1} \sep \heap_1 {\wedge} \pure_1}%1
      {\rpreds{\btt{R}}{\code{x}, \fann \constr_{2},\vlist{v}_2} \sep \heap_2 {\wedge} \pure_2 }%2
      {(\hvardef_2,\D_4)}%3
}
\end{equation*}

\begin{equation*}
\begin{array}{lll}
\myit{addVar}(\rpreds{\btt{R}}{\code{x}, \fann \rsrvar,\vlist{v}}) &\defs&
(\rsrvar, \fann \rsrvar, \emp, \false)\\

\myit{addVar}(\rpreds{\btt{R}}{\code{x}, \fann (\heap {\wedge} \pure),\vlist{v}}) &\defs&
(\rsrvar, \fann (\heap {\sep} \rsrvar {\wedge} \pure), \rpreds{\btt{R}}{\code{x}, \{\fann \rsrvar\},\vlist{v}}, \true),
%\\ & &
\textit{fresh~\code{V}}
\end{array}
\end{equation*}

\vspace*{-8mm}

\begin{center}
\begin{multicols}{2}
\begin{equation*}
\frac{
  \begin{array}{c}
    \entrulen{[RP-IN]}\\
    \entailCV
          {\constr_{2}}%1
          {\constr_{1}}%2
          {\hvardef}%3
  \end{array}
}{
  \entailInVHO
      {\constr_{1}}%1
      {\constr_{2}}%2
      {\hvardef}%3
      {\myit{E}}%4
}
%\end{equation*}
\qquad%\break
%\begin{equation*}
\frac{
  \begin{array}{c}
    \entrulen{[RP-OUT]}\\
    \entailCV
          {\constr_{1}}%1
          {\constr_{2}}%2
          {\hvardef}%3
  \end{array}
}{
  \entailOutVHO
      {\constr_{1}}%1
      {\constr_{2}}%2
      {\hvardef}%3
      {\myit{E}}%4
}
\end{equation*}
\\%\break
\begin{equation*}
\frac{
  \begin{array}{c}
    \entrulen{[RP-L-INST]}\\
    \rsrvar \in \myit{E}
  \end{array}
}{
  \entailCV
            {\rsrvar}%1
            {\constr}%2
            {\{(\rsrvar, \constr)\}}%3
}
%\end{equation*}
\qquad%\break
%\begin{equation*}
\frac{
  \begin{array}{c}
    \entrulen{[RP-R-INST]}\\
    \rsrvar \in \myit{E}
  \end{array}
}{
  \entailCV
            {\constr}%1
            {\rsrvar}%2
            {\{(\rsrvar, \constr)\}}%3
}
\end{equation*}
\end{multicols}
\end{center}
\end{small}



==> smallstep.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!htb]
\savespace
\begin{center}
%\begin{minipage}{26pc}%{42pc}
\begin{frameit}
%% \savespace
%% \savespace
\savespace
\begin{small}
\[
\hspace{-3mm}
\begin{array}{c}
%%%%%%%%%%%%%%%%%%%%
%IF TRUE
%%%%%%%%%%%%%%%%%%%%

\begin{array}{c}

( \threadspec, \{ (\tid , \lit{run}(\lit{if} ~\nonterm{true} ~\lit{then} ~ \nonterm{$s_1$} ~ \lit{else} ~ \nonterm{$s_2$} ; s,\envir)) \} \bagunion \threads)
\to\\
( \threadspec, \{ (\tid ,\lit{run}(\nonterm{$s_1$} ; s , \envir)) \} \bagunion \threads)

\end{array} \savesmallspace \\ \\

%%%%%%%%%%%%%%%%%%%%
%IF false
%%%%%%%%%%%%%%%%%%%%

\begin{array}{c}

( \threadspec, \{ (\tid , \lit{run}(\lit{if} ~\nonterm{false} ~\lit{then} ~ \nonterm{$s_1$} ~ \lit{else} ~ \nonterm{$s_2$} ; s,\envir)) \} \bagunion \threads)
\to \\
( \threadspec, \{ (\tid ,\lit{run}(\nonterm{$s_2$} ; s , \envir)) \} \bagunion \threads)

\end{array}\savesmallspace  \\ \\

%%%%%%%%%%%%%%%%%%%%
% Ifthen else
%%%%%%%%%%%%%%%%%%%%

\begin{array}{c}
\frac{
\begin{array}{c}

eval(e,\envir)=b

\end{array}
}{
\begin{array}{c}

(\threadspec, \{ (\tid , \lit{run}(\lit{if} ~\nonterm{e} ~\lit{then} ~ \nonterm{$s_1$} ~ \lit{else} ~ \nonterm{$s_2$} ; s,\envir) ) \} \bagunion \threads)
\to \\
(\threadspec, \{ (\tid ,\lit{run}(\lit{if} ~\nonterm{b} ~\lit{then} ~ \nonterm{$s_1$} ~ \lit{else} ~ \nonterm{$s_2$} ; s , \envir)) \} \bagunion \threads)

\end{array}
}
\end{array}\savesmallspace  \\ \\

%%%%%%%%%%%%%%%%%%%%
%CALL
%%%%%%%%%%%%%%%%%%%%

\begin{array}{c}
\frac{
\begin{array}{c}

\hide{
\forall i \in \{1,\ldots,n\} \bullet \envirof{v_i} = o_i \\
}
spec(pn) := \code{pn}(w_1, \dots, w_n) ~ \lit{requires} ~\constr_{pr} ~\lit{ensures}~
\constr_{po}\lit{;} ~\{~s_{1}~\}
\\

s_1' = [v_1/w_1,\ldots,v_n/w_n]s_1

\end{array}
}{
\begin{array}{c}

( \threadspec, \{ ( \tid , \lit{run}(pn(v_1, \ldots, v_n\lit{)}; s, \envir)) \} \bagunion \threads)
\to \\
( \threadspec, \{ ( \tid , \lit{run}(s_1'; s, \envir)) \} \bagunion \threads)

\end{array}
}
\end{array} \savesmallspace \\ \\

%%%%%%%%%%%%%%%%%%%%
%FORK
%%%%%%%%%%%%%%%%%%%%

\begin{array}{c}
\frac{
\begin{array}{c}

spec(pn) := \code{pn}(w_1, \dots, w_n) ~ \lit{requires} ~\constr_{pr} ~\lit{ensures}~
\constr_{po}\lit{;} ~\{~s_{1}~\}
\\

\forall i \in \{1,\ldots,n\} \bullet \envirof{v_i} = o_i

\quad\quad

\fresh(\tid_1)

\quad\quad

\envir'= \envir [ v \mapsto \tid_1]

\\

\envir_1= [w_1 \mapsto o_1,\ldots,w_n \mapsto o_n]

\quad\quad

typeof(\tid_1)=\code{thrd}

\\

\threadspec_1 = \threadspec[ \tid_1 \mapsto \constr_{po}]

\end{array}
}{
\begin{array}{c}

( \threadspec, \{ ( \tid , \lit{run}(\nonterm{v} = \lit{fork} \lit{(} pn \lit{,} v_1, \ldots, v_n\lit{)}; s, \envir)) \} \bagunion \threads)
\to \\
( \threadspec_1, \{ ( \tid , \lit{run}(s, \envir')) \} \bagunion \{ ( \tid_1 , \lit{run}(s_1;\myhalt, \envir_1)) \} \bagunion \threads)

\end{array}
}
\end{array} \savesmallspace \\ \\
%%%%%%%%%%%%%%%%%%%%
% HALT
%%%%%%%%%%%%%%%%%%%%

\begin{array}{c}

(\threadspec, \{ ( \tid , \lit{run}(\myhalt, \envir)) \} \bagunion \threads)
\to
(\threadspec, \{ ( \tid , \lit{dead}) \} \bagunion \threads)

\end{array} \savesmallspace \\  \\

%%%%%%%%%%%%%%%%%%%%
%JOIN
%%%%%%%%%%%%%%%%%%%%

\begin{array}{c}
\frac{
\begin{array}{c}

\highlightd{ \exists ( \tid_1,\lit{dead}) \in \threads \bullet \envirof{v} = \tid_1  }

\end{array}
}{
\begin{array}{c}

( \threadspec, \{ ( \tid , \lit{run}(\lit{join} \lit{(} v \lit{)}; s, \envir)) \} \bagunion \threads)
\to
( \threadspec, \{ ( \tid , \lit{run}( s, \envir)) \} \bagunion \threads)

\end{array}
}
\end{array}  \\

\end{array}
\]
\end{small}
%% \savespace
\end{frameit}
\savesmallspace
\caption{Selected Small-step Operational Semantics of Well-formed Programs}
\label{fig:smallstep}
\savespace\savespace
%\savespace\savespace
%\end{minipage}
\end{center}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> soundness-new.tex <==
%% \khanh{Not sure if we could have a generalized proof
%% for both threads and CDL. They seem to share the notion
%% of count. fork() is similar to countdown() where count=1;
%% join() ~ await() when the count $\leq$ 0.
%% Will be specific in the meantime and think
%% about generelization later}

\khanh{would it be possible to have soundness proof for
FARP in general, instead of just focusing on CountDownLatch
as we did below?}

Our flow-aware resource predicates allow
resource flows to be precisely tracked.
Due to space limitation and to demonstrate
the key ideas, in this section, we mainly focus the
soundness proof for CountDownLatch (CDL) primitives whose
flow-aware resources can be flexibly split and ``flowed''.
Soundness of
thread and lock primitives can
also be derived,
as discussed in Section~\ref{sec:thrdlock}.
%% and are left in the technical report
%% \cite{}.\khanh{we can also ignore this,
%% just discuss possible extension.}

Our proof is based on soundness proof of
Villard et al. \cite{Villard:APLAS09}
which is tailored towards copyless message-passing
channels.
Their proof is based on the following key ideas.
First, they restrict program states
to race-free legal states
where a receive operation must have received
not more
%% less 
than what the corresponding send operation has sent.
Second, messages sent over a channel are tagged
with timestamps in order to ensure that the content
received matches what was sent.
By relying on abstract separation logic \cite{Calcagno:LICS2007}
the soundness of their whole proof system
is established by the sole soundness of
all primitive commands.

Our proof is based on a similar idea.
First, we also restrict program states to
race-free legal states where await operations must have produced
``outflow'' resource which is not more
%% less 
than the ``inflow''
resource that
the corresponding countdown operations have consumed.
%% \scsay{Do
%% we need to explain what we meant by "send" here?}.
A count is used to make sure that a pre-defined
number of countdown operations has reached before
any await operations are executed.
Second, CDLs and memory cells are associated with flow-aware tags.
Our approach then ensures that, for a given tag,
the inflow content matches the outflow content.
The legal states are also deadlock-free 
since their corresponding wait-for graphs are
guaranteed to be acyclic.
Our approach, therefore, ensures race-freedom, deadlock-freedom
and leak-freedom.

For simplicity in the soundness proof,
we adopt the following simplified language
from  \cite{Calcagno:LICS2007,Villard:APLAS09}:

$p ~ {::=} ~ c ~\mid~ p;p ~\mid~ p\,||\,p ~\mid~ p+p ~\mid~ p* $

{\noindent}where $c$ is among our {\CDL} primitives
(introduced in Section~\ref{sec:latch}).
We assume that the primitives are atomic.
We also make the following simplifications on the
specification language.
We consider objects of type
\btt{Cell} and \btt{CDL} only.
User-defined data types can be supported by
extending from \btt{Cell} to objects with fields.
This, however, unnecessarily complicates the memory model.
We also do not consider permission-based
heaps, which could be separately extended.

%% \khanh{Need to discuss restriction on the language
%% used for soundness proof}

\subsection{Basic Memory Model}
\input{model}

\subsection{Trace-based Semantics and Model of Synchronization}
\input{trace}

\subsection{Tagged Memory Model}
\input{tagged}

\subsection{Soundness Proof}
\label{sec:proof}
\input{proof}

%% \subsection{Extensions for Threads and Locks}
%% \label{sec:thrdlock}
%% \input{extensions}


==> soundness.tex <==
We discuss the soundness of our
``threads as resource'' approach.
We first present the interleaving operational semantics
of the language.
We then prove the soundness of our approach
with respect to the operational semantics.

%% \subsection{Operational Semantics}
%% \label{sec:tar:semantics}
\subsubsection*{Operational Semantics.}
We define the interleaving operational semantics of programs
with fork/join concurrency. Our semantics resembles the semantics
of well-known concurrent languages such as Java, C\#, and C/C++.

\begin{mydef}[Well-formedness]
A program is well-formed if the following conditions hold:
\begin{itemize}
  \item In the program text, there exists a procedure called main,
which indicates the entry point of the program.
  \item Procedure names are unique within a program. Procedure
parameters are unique within a procedure. Free variables
in the body of a procedure are the procedure parameters.
  \item A normal procedure call or a fork statement mentions
only procedure names defined in the program text.
The number of actual parameters and formal parameters
are equal.
\end{itemize}
\end{mydef}

A thread can be in one of three states: \myit{running}, \myit{dead}, and \myit{aborted}.
Our verification framework ensures that 
no thread ends up in an \myit{aborted} state.
A program state is \myit{non-aborting} if no thread is in an
\myit{aborted} state. A program state is \myit{final} if 
all threads are in a \myit{dead} state.

%% \savespace
\begin{mydef}[Thread State]\label{def:tar:state}
A thread state $\state$ is one of the following states:
\begin{itemize}\savesmallspace
  \item $\lit{run}(s,\envir)$ stating that the thread is running with
remaining statement $s$ and environment $\envir$.
For brevity, $\envir$ is assumed to be 
a partial function from object names to object references and
from stack variables to values. Environment $\envir$ resembles stack
and heap in programs. An update at $v$ with $o$ in $\envir$
is denoted as $\envir [ v \mapsto o]$.
  \item $\lit{dead}$ stating that a thread has completed its execution.
%% in the enviroment $\envir$.
  \item $\lit{aborted}$ stating a thread has performed an illegal operation,
such as null-pointer dereference.
\end{itemize}
\end{mydef}%% \savesmallspace

%% \savespace
\begin{mydef}[Program State]
A program state $\config$ consists of a thread specification pool
$\threadspec$ and a set of threads $\threads$.
$\threadspec$ maps from a thread identifier
to its aggregate resource (which is book-kept when the thread
is forked).
Each thread in $\threads$ is a pair of
($\tid,\state$) representing thread identifier $\tid$ and
thread state $\state$. The thread identifier $\tid$ is of type
\code{thrd} while the thread state $\state$ is defined above.
\end{mydef}

We use $m$ to indicate the identifier of the main thread,
i.e. the thread executing the main procedure of the program.
We denote $\threadspec_{m}$ as a thread specification pool containing
only information of the main thread. In other words,
$\threadspec_{m}(i)= \emp$ if $\tid {=} m$,
and $\threadspec_{m}(\tid)$ is undefined
otherwise.

%% \savespace
\begin{mydef}[Execution]
Execution of a program starts in the initial program state:
$(\threadspec_{m},\{(m , \lit{run}({s},\emptyset))\})$, where
$s$ is the code fragment of the main procedure.
\end{mydef}%% \savesmallspace

\input{smallstep}

Fig.~\ref{fig:smallstep} shows the small-step operational semantics.
A premise marked with \highlightd{\text{box}} denotes the fact that threads must
block and wait for the premise to become true. For example,
joining with a thread blocks until the thread is dead.
In Fig.~\ref{fig:smallstep},
$spec(pn)$ denotes the specification of the procedure $pn$
in the program,
$eval(e,\envir)$ denotes the evaluation of the expression $e$
in the environment $\envir$.
The rules for fork and join are of special interest.
In the fork rule, a new thread is spawned and the return
value $v$ points to its identifier $\tid_1$ of type \code{thrd}.
The resource carried by $\tid_1$ is book-kept in $\threadspec_1$.
We explicitly add a {\myhalt} statement
%% that is automatically added
to signify the end of each newly spawned thread.
As a quick observation, a thread identifier corresponds
to a thread node in our logic.
Any threads (joiners) knowing the identifier can perform a join operation
to join with the newly-created thread (joinee).
In the join rule, if the joinee has not yet finished its execution
(i.e. it is not in a \lit{dead} state), the joiners have to wait
for the joinee to finish its execution.
Note that when a joinee is joined,
it will not be removed from the set of threads.
This allows for the multi-join pattern
and enables the
joiners to immediately proceed without waiting
in case the joinee has already finished its execution.
There is a direct relation between the \lit{dead} state
of a thread during run-time and its
{\em dead} predicate during verification-time.

\subsubsection*{Semantics}

We impose a restriction whereby thread nodes can only
be passed between the caller and callee of the same
thread, or between different threads
(i.e. from forker to forkee, or from joinee to joiner).
Thread nodes, therefore, are not allowed
to belong external environment such as
lock invariants. This is to avoid
circularity when the two thread nodes
of two different threads refer to each other
as their carried resource.

An separation formula is interpreted with respect
to a thread identifier $k$ of the active thread
and the program state $(\threadspec,\threads)$.
The interpretation of most parts of our separation logic
formulae is standard and can be found
elsewhere \cite{Gotsman:APLAS07}.
Here we focus on the most interesting part.
The interpretations of the thread node $\permsto{t}{\thread{ \constr }}{}$
and the $dead(t)$ predicate are as follows:

\begin{small}
$(\threadspec,\{ (k ,\lit{run}(\nonterm{$s$}, \envir)) \} \bagunion \threads)
\models_{k}
\permsto{t}{\thread{ \constr }}{}
~\Longleftrightarrow~
\exists\tid \cdot
\envir(t) {=} \tid \wedge
\threadspec(\tid) {=} \constr_1 \wedge \constr {\bagsubsumeeq} \constr_1
$

$(\threadspec,\{ (k ,\lit{run}(\nonterm{$s$}, \envir)) \} \,{\bagunion}\, \threads)
\,{\models_{k}}\,
\dead{t}
\Longleftrightarrow
\exists ( \tid,\lit{dead}) {\in} \threads \cdot  \envir(t) {=} \tid
$
\end{small}

Intuitively, $\constr {=} \constr_1$ when there is only one thread
node of the thread $t$ in the program.
$\constr {\bagsubsume} \constr_1$ indicates
the presence of multiple nodes of the same thread $t$.
Even though the above interpretation does not describe
the exact resource belong to the thread $t$,
the interpretation is sound due to two reasons.
First, our approach respects separation property,
i.e. the resources carried by two thread nodes
of the same thread are well-separated (Lemma~\ref{lmm:tar:separation}).
Second, 
our approach ensures that the total resource
carried by all thread nodes of the same thread $t$
is equal to the aggregate resource $\constr_1$ captured
in $\threadspec$.
The resource $\constr_1$  is book-kept when the thread $t$
is forked and is flexibly split off and combined
by our approach.
To prove the above claim,
we show that our ``threads as resource''
approach neither invents new resource nor destroys
existing resource.
Therefore, it guarantees that the total resource of the program
is not changed by our verification rules (Lemma~\ref{lmm:tar:total}).
Note that our verification-time {\em dead(t)} predicate resembles the \lit{dead} state
of a thread during run-time.


\begin{lmm}[Separation of Resources]\label{lmm:tar:separation}
If there exist two thread nodes \permsto{t}{\thread{ \constr_1 }}{}
and \permsto{t}{\thread{ \constr_2 }}{} of the same thread $t$,
$\constr_1$ and $\constr_2$ are well-separated. In other words,
$\constr_1 {\sep} \constr_2$ is a valid separation logic
formula.
\end{lmm}

\begin{proof}
%% We adopt the standard notion of preciseness of
%% separation logic formulae as described in \cite{Gotsman:APLAS07}.
Splitting and combining thread nodes resort to
splitting and combining their carried resources
(described in the rule \entrulen{R-THRD2} of Fig.~\ref{fig:perm-rules}).
The splitting and combining of the resources follow
the standard fractional permission accounting
\cite{Bornat:POPL05,Boyland:SAS03}.
Therefore, this lemma could
be proven by induction on the structure of separation formulae
(Fig.~\ref{fig:speclang}).
Note that although the resource carried in a thread node
could refer to other thread node(s), as discussed previously,
our approach prevents circularity from occurring.
Hence, the induction is guaranteed to terminate.
\end{proof}%% \savespace\savespace

\begin{lmm}[Conservation of Total Resource]\label{lmm:tar:total}
The total resource of a program
is unchanged under ``threads as resource'' verification
approach.%% \savespace
\end{lmm}

\begin{proof}
Except for fork and join,
the verification rules in Fig.~\ref{fig:fwdrules}
and sub-structural rules in
Fig.~\ref{fig:perm-rules}
neither invent new resource nor destroy existing resource.
Fork and join create and respectively consume
thread nodes. Thread nodes can be considered
as placeholders for the resources that they carry.
Hence, this lemma can be proven
by induction on the sub-structural rules
(Fig.~\ref{fig:perm-rules}).
\end{proof}%% \savespace\savespace


\begin{lmm}[Soundness of Threads as Resource]\label{lmm:tar-sound}
Given a program with a set of procedures $P^i$ together with 
their corresponding pre/post-conditions ($\constr_{pr}^i$/$\constr_{po}^i$),
if our verifier derives a proof for every procedure $P^i$, 
i.e. \{$\constr_{pr}^i$\}$P^i$\{$\constr_{po}^i$\} is valid, then
the program is functionally correct.
\end{lmm}
\begin{proof}
It directly follows from Lemma~\ref{lmm:tar:separation},
Lemma~\ref{lmm:tar:total}, and induction on the operational
semantics presented in Fig~\ref{fig:smallstep}.
\end{proof}


==> speclang-locks.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!hb]
%\savespace
\savespace
\savespace
%\savespace
\begin{center}
\begin{minipage}{25pc}%{32pc}
\begin{frameit}
\savespace
\savespace
\savespace
\[
\begin{array}{rcll}
%% \textsf{Shape predicate} & \nonterm{spred} &::=&
%% [\self{::}]\predfo{\term{c}}{\term{v}^*}{\fracperm} \veq
%% \constr~[\lit{inv}~\pure_0]\\

\textsf{Separation formula} & \constr &::=& \bigvee ( \exists v^* \cdot
\heap \wedge \pure \wedge \lockf ) \\

\textsf{Lock formula} & \lockf &::=& {\bigwedge} \locksetf \\

\textsf{Atomic heap formula} & \aheap &::=&
\permsto{\term{v}}{C({\term{v}}^*)}{\fracperm}
\mid \permsto{\term{v}}{ \thread{\delayedf ~ \eimply{w^*} ~ \constr} }{} \\

\textsf{Delayed formula} & \delayedf &::=& \bigvee ({\bigwedge} \locksetf \wedge \pconstr) \\

%% {\term{p}{::}\predfo{\term{c}}{{\term{v}}^*}{\fracperm}} \\ 

\textsf{Lockset formula} & \locksetf &::=& \nonterm{v} \in \alockset \mid 
\nonterm{v} \notin \alockset \\

\textsf{Pure formula} & \pure &::=& \ldots \mid \mset \\

\textsf{Set formula} & \mset &::=& \mterm_1 \bagsubsume \mterm_2 \mid \mterm_1 = \mterm_2 \hide{\mid \nonterm{v} \in \mterm} \\

\textsf{Set term} & 
	\mterm &::=& \alockset \mid \set{} \mid \set{v} \mid \mterm_1 \bagunion \mterm_2 \mid
	\mterm_1 \bagintersect \mterm_2 \mid \mterm_1 \bagsubtract \mterm_2 \\

\ldots

\end{array}
\]
\savespace
\[
\begin{array}{c}

\term{C} \in \textsf{Data names} \bagunion \{ \code{LOCK} \}

\end{array}
\]

%% \savespace
\savesmallspace
\end{frameit}
%\savespace
\savespace
\caption{Grammar for Core Specification Language with Locks}\label{fig.speclang-locks}
\end{minipage}
%% \savespace\savespace
%% \savespace\savespace
%% \savesmallspace
\end{center}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> speclang.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb]
%\savespace
%% \savespace
%% \savespace
%\savespace
\begin{center}
%\begin{minipage}{25pc}%{32pc}
\begin{frameit}
\savespace
\savespace
\savespace
\begin{small}
\[
\begin{array}{rcll}
%% \textsf{Shape predicate} & \nonterm{spred} &::=&
%% [\self{::}]\predfo{\term{c}}{\term{v}^*}{\fracperm} \veq
%% \constr~[\lit{inv}~\pure_0]\\

%\textsf{Separation formula} 

\!\!\!\!\btt{Shape~ pred.} & \!\! \nonterm{spred} &\!\!{::=}\!\!\!\!&
\code{pred}~\term{P}(\self,\vlist{v}) \veq
\constr~[\lit{inv}~\pure]\\

\!\!\!\!\btt{Resource~pred.} & \!\! \nonterm{rpred} &\!\!{::=}\!\!\!\!&
\code{pred}~\btt{R}[[\vlist{v}]](\self,\overbar{\rsrvar},\vlist{v}) ~[\lit{inv}~\pure]\\

\!\!\!\!\btt{Disj.~ formula} & \!\! \constr &\!\!{::=}\!\!\!\!& \bigvee ( \exists \vlist{v} \cdot
\heap \wedge \pure) \\

%\textsf{Composite formula} 
\!\!\!\!\btt{Comp.~formula} & \!\! \D &\!\!{::=}\!\!\!\!& \constr \mid \D_1 {\vee} \D_2 \mid \D_1 {\wedge} \pure \mid
\D_1 {\sep} \D_2 \mid {\exists} \code{v} {\cdot} \D \\

%\textsf{Heap formula} 
\!\!\!\!\btt{Sep~ formula} & \!\! \heap &\!\!{::=}\!\!\!\!& \emp \mid \aheap \mid \WAIT{\overbar{v_1{\ra}v_2}} \mid  \heap_1 \sep \heap_2 \\
 
%\textsf{Atomic heap formula} 
\!\!\!\!\btt{Atomic~heap}
& \!\! \aheap &\!\!{::=}\!\!\!\!&
\permsto{\code{v}}{C(\vlist{v})}{}
\mid \term{P}(\overbar{\code{v}}) \mid \rsrvar
\mid \rpredl{\btt{R}}{\vlist{v}}{\code{v},\overbar{\fconstr},\vlist{v}} \\

\!\!\!\!\btt{Flow.~ formula} & \!\! \fconstr & \!\!{::=} & \inflow \constr \mid \outflow \constr \\

%% {\term{p}{::}\predfo{\term{c}}{{\term{v}}^*}{\fracperm}} \\ 

%\textsf{Pure formula} 
\!\!\!\!\btt{Pure~formula}
& \!\! \pure &\!\!{::=}\!\!\!\!& \arith \mid \pure_1
{\wedge} \pure_2 \mid \pure_1 {\vee} \pure_2 \mid {\neg} \pure
\mid {\exists} \code{v} {\cdot} \pure \mid {\forall} \code{v} {\cdot} \pure\\

%\textsf{Arithmetic formula} 
\!\!\!\!\btt{Arith.~formula}
& \!\! \arith &\!\!{::=}\!\!\!\!& \aterm_1 {=} \aterm_2 \mid \aterm_1 {\neq} \aterm_2 \mid 
			\aterm_1 {<} \aterm_2 \mid \aterm_1 {\leq} \aterm_2  \\

%\textsf{Arithmetic term} 
\!\!\!\!\btt{Arith. term} 
& \!\! \aterm &\!\!{::=}\!\!\!\!& \code{k} \mid \code{v} \mid \code{k} \times \aterm \mid \aterm_1 + \aterm_2 \mid -\aterm \\

\end{array}
\]
\end{small}
\savespace
\[
\begin{array}{ll}
%% \myit{Frac.~ perm.~ var.}~\fracperm \in \lit{(} 0 \lit{,} 1
%% \lit{]}	 & \code{v} \in \myit{Variables} \\
k \in \myit{integer~constants} &
\code{v} \in \myit{variables} , \vlist{v} \veq \code{v}_1,\ldots,\code{v}_n\\
\term{C} \in \myit{data.~names} &  \myit{P} \in \myit{shape~pred.~names}\\
\rsrvar \in \myit{resource~variables} & 
\btt{R} \in \myit{resource~pred.~names}  \\


\end{array}
\]

%% \savespace
\savesmallspace
\end{frameit}
%\savespace
\savesmallspace
\caption{Grammar for Core Specification Language}\label{fig:speclang}
%\end{minipage}
%\savespace\savespace
%% \savespace
\savespace
%\savesmallspace
\end{center}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> tagged.tex <==
\paragraph{Tagged Model}

We present our refined memory model,
where $\fpheap$ and $\fpCDL$ are associated with
flow-aware tags.
Recall that flow type $\flow \defs \inflow \mid \outflow$.
\morespace

\hide{
Tag: $\mytag \in \mytagset$ (new tag for each synchronizer).
\khanh{not call it timestamp. timestamp is a bit misleading
since it is related to time. Tag is not related to time,
it only mark which heaps belong to which synchronizer}

Our idea is that for each synchronizer s,
a tag is associated to it when it is created.
Then, the sum of its inflow-tagged resources is
equal to the sum of its outflow-tagged resources.

Tag heaps with flows.

Flow types: $\flow \defs \inflow \mid \outflow$.
} % END HIDE

$ \fpstate \defs \pstack \times \fpheap \times \fpCDL \times \pgraph$

$ \pstack \defs \pvar \rightharpoonup \pval $

$\fpheap \defs \ploc \times \ptagset  \rightharpoonup \btt{Cell}(\pval)$

$\fpCDL \defs \platch \times \ptagset \rightharpoonup \btt{CDL}(\pval \times \boolset \times \inflow \cdlR \times \outflow \cdlR) $

$\pgraph \defs \pset{\platch \times \platch} $
\morespace

In the tagged model,
in addition of a count and
a flow-aware resource $\flow \cdlR$,
each CDL has its own tag.
%% Possibly: memory state $[\inflow]\fstate_1 \sep [\outflow]\fstate_2$
%% will be defined as legal if and only if $\fstate_1 < \fstate_2$
%% (cannot produce more than what have been consumed).
We define polarized tags $\ptagset \defs (\platch \times \set{\inflow,\outflow}) + \set{\now}$.
We use the $\hat{~}$ notation to differentiate between
the basic model and the tag model where
${\hat h}$, ${\hat l}$ ranges over
$\fpheap$ and $\fpCDL$.
%% $(\fpstate,\circ,u)$ defines a separation algebra. 

We define the projection \myit{now}:  $\fpstate \rightarrow \fpstate$ which associates
a state $\state {=} (s,h,l,g)$ to a state $\fstate {=} (s,{\hat h},{\hat l},g)$
where $h {=} {\hat h}(\cdot,\now)$ and $l {=} {\hat l}(\cdot,\now)$
where tags are erased.
Let $\myit{now}^{-1}(A)$ denote the set of
all $\fstate {=} (s,{\hat h},{\hat l},g) \in \fpstate$ such that
$\fstate {=} \fstate\!\! \downharpoonright_{\now}$
and $now(\fstate) \in A$, where
$\fstate\!\! \downharpoonright_{\now}$ denotes
the state
defined by restricting ${\hat h}$ and ${\hat l}$ to the tag $\now$.
We now define the semantic of Hoare's triple
under the tagged semantics.

\begin{mydef}[Semantic Hoare Triple]
If $A,B \in P(\fpstate)^{\!\fault}$
and $f : \fpstate \rightarrow P(\fpstate)$, we write $\semHoare{A}  f \semHoare{B}$ 
iff $\forall \fstate \cdot now(\fstate) \in A$ implies $now(f(\fstate)) \sqsubseteq B$.
We write $\models \set{A} p \set{B}$ iff $\forall tr \in T(p) \cdot \semHoare{A}  \denote{tr} \semHoare{B}$
\end{mydef}

\hide{
Expect: Given a program trace $tr$
and a CDL object $o$,
$[\inflow]tr \!\! \downharpoonright \!\! o {=} [\outflow]tr \!\! \downharpoonright \!\! o $
where $tr \!\! \downharpoonright$ is the projection of
trace $tr$ on heap object $o$ and $[\flow]tr$
is the projection to flow \flow.
\khanh{may still need a tag to differentiate between
different CDL}
\khanh{how APLAS09 deals with different channels?}

(may not hold for predicate transformer for threads)
}

\paragraph{Semantics of Assertions}
We shall show the semantics of assertions under
the tagged memory model.

Let $logs(\fstate)$ denote the set of polorized tags
that appear in $\fstate$, i.e. $snd(\myit{dom}({\hat h})) \cup snd(\myit{dom}({\hat l}))$.
And denote $\fstate \!\! \downharpoonright_{\mytag \flow }$ as the state with tag $\mytag \flow$ 
defined by restricting ${\hat h}$ and ${\hat l}$ to the tag $\mytag \flow$.
%% \khanh{seems that we only result one state, instead of set of states. No, it's a set of states since a location can have different
%% tags, e.g. now for current state, \flow for historical states.}
We denote $\langle \mytag \flow \rangle \fstate$ the set of states
that result from
$\fstate$ by tagging  all heap cells with the tag $\mytag \flow$, defined as: $
\fstate' {=} (s,{\hat h},{\hat l},g) \in \langle \mytag \flow \rangle \fstate ~\btt{if}~ logs(\fstate) {=} \set{\mytag \flow}
$.
We now give semantics of formulas over $\fpstate$:
for any $\fstate \in \fpstate$,
and for any formula $\constr$,
$\fstate \models \constr$ iff (1) $logs(\fstate) {\subseteq} \set{\now}$
and (2) $\fstate \!\! \downharpoonright_{\now} \models \constr$.

We restrict tagged memory states to well-formed ones
by limiting the composition of states in such a way
that, for a given tag $\mytag$, the inflow-tagged
content is equal to the outflow-tagged content.

\begin{mydef}[Tagged memory state] The separation algebra
$(\fpstate,\bullet,{\hat u})$ of well-formed tagged memory states
is obtained from $(\fpstate,\circ,{\hat u})$ by restricting
$\fpstate$ to state $\fstate$ such that $now(\fstate) \in \pstate$,
and strengthening the compatibility relation
$\perp$ by:

{\noindent}{\bf Resource Preservation:} $\fstate {=} \fstate_1 \bullet \fstate_2$ is defined if $\fstate_1 \circ \fstate_2
\in \fpstate$ and for all $\mytag \neq \now$, 
$\fstate \!\! \downharpoonright_{\mytag \inflow} {=} \fstate \!\! \downharpoonright_{\mytag \outflow})$

\end{mydef}

We then define meanings of important assertions:

\begin{scriptsize}
\[
\begin{array}{lll}

\!\!\! (s,{\hat h},{\hat l}, g) \models \permsto{v1}{\btt{Cell}(v2)}{} & \!\!\! \btt{iff} \!\!\!
& v1,v2 {\in} \myit{dom}(s) {\wedge} \myit{dom}({\hat h}) {=} \set{(s(v),\now)} \\
\!\!\! & &  {\wedge} {\hat h}(s(v1),\now) {=} s(v2)  \\

%% \!\!\!  (s,{\hat h},{\hat l}, g) \models \btt{Latch}(v,\flow \constr) & \!\!\! \btt{iff} \!\!\!
%% & \exists \mytag \cdot
%% (s,{\hat h},{\hat l}, g) \models \btt{Latch}(v,\flow \constr, \mytag)\\

%% \!\!\!  (s,{\hat h},{\hat l}, g) \models \btt{Latch}(v,\flow \constr) & \!\!\! \btt{iff} \!\!\! 
%% & v {\in} \myit{dom}(s) {\wedge} \myit{dom}({\hat l}) {=} \set{(s(v),\now)} \\
%% \!\!\!  & & {\wedge} \myit{dom}(h){=}\emptyset {\wedge} (\exists k \cdot {\hat l}(s(v),\now) {=} \btt{CDL}(k,\flow \constr)) \\

%% \!\!\!  (s,{\hat h},{\hat l}, g) \models \btt{CNT}(v1,v2) & \!\!\! \btt{iff} \!\!\!
%% & v1,v2 {\in} \myit{dom}(s) {\wedge} (s(v1),\now) {\in} \myit{dom}({\hat l}) {\wedge} \myit{dom}({\hat h}) {=} \emptyset \\
%% \!\!\!  & & {\wedge} (\exists k, \constr \cdot {\hat l}(s(v),\now) {=} \btt{CDL}(k,\flow \constr) {\wedge} k{=}s(v2))\\

%% \!\!\! (s,{\hat h},{\hat l}, g) \models \btt{WAIT(S)} & \!\!\! \btt{iff} \!\!\!
%% & \forall v_1{\ra}v_2 {\in} {\codeE{S}} \cdot (s,{\hat h},{\hat l}, g)  \models \btt{WAIT(\{v_1{\ra}v_2\})}\\

%% \!\!\! (s,{\hat h},{\hat l}, g) \models  \btt{WAIT(\{v_1{\ra}v_2\})}  & \!\!\! \btt{iff} \!\!\!
%% & v1,v2 {\in} \myit{dom}(s) {\wedge} (s(v1),\now),(s(v2),\now) {\in} \myit{dom}({\hat l}) \\
%% \!\!\! & & {\wedge} (s(v1),s(v2)) {\in} g  {\wedge} \myit{dom}({\hat h}) {=} \emptyset\\
%% \!\!\! & & {\wedge} ({\exists} k_1,k_2,\constr_1, \constr_2 \cdot k_1{>}0 {\wedge} k_2{<}0  \\
%% \!\!\! & & ~~~~~{\wedge} {\hat l}(s(v1),\now) {=} \btt{CDL}(k_1,\flow \constr_1) \\
%% \!\!\! & & ~~~~~{\wedge} {\hat l}(s(v2),\now) {=} \btt{CDL}(k_2,\flow \constr_2) )\\
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%

\!\!\! (s,{\hat h},{\hat l},g) \models \btt{Latch}(v,\inflow \constr) & \!\!\! \btt{iff} \!\!\!
& v \in \myit{dom}(s) \wedge \myit{dom}({\hat l}) {=} \set{(s(v1),\now)} 
\\
\!\!\! & & 
{\wedge} \myit{dom}({\hat h}) {=} \emptyset   {\wedge} \exists k,b \cdot \\
\!\!\! & & {\hat l}(s(v),\now) {=} \btt{CDL}(k,b,\inflow \constr, \outflow \emp) \\

\!\!\! (s,{\hat h},{\hat l},g) \models \btt{Latch}(v,\outflow \constr) & \!\!\! \btt{iff} \!\!\!
& v \in \myit{dom}(s) \wedge \myit{dom}({\hat l}) {=} \set{(s(v1),\now)} 
\\
\!\!\! & & 
 {\wedge} \myit{dom}({\hat h}) {=} \emptyset {\wedge} \exists k,b \cdot \\
\!\!\! & &  {\hat l}(s(v),\now) {=} \btt{CDL}(k,b,\inflow \emp, \outflow \constr) \\

\!\!\! (s,{\hat h},{\hat l},g) \models \btt{CNT}(v1,v2) & \!\!\! \btt{iff} \!\!\!
& v1,v2 {\in} \myit{dom}(s) {\wedge} (s(v1),\now) {\in} \myit{dom}({\hat l})   \\
\!\!\! & &  {\wedge} \myit{dom}({\hat h}) {=} \emptyset {\wedge} ({\exists} k,k_1,b,\constr_1,\constr_2 \cdot \\
\!\!\! & &  {\hat l}(s(v1),\now) {=} \btt{CDL}(k,b,\inflow \constr_1,\outflow \constr_2)
\\
\!\!\! & &
 {\wedge} k_1{=}s(v2)\\ 
\!\!\! & & {\wedge} 
       ((k_1{\geq}0 {\rightarrow} k=k1) 
       {\vee} (k_1{<}0 {\rightarrow} b=\btt{T})) )\\

\!\!\! (s,{\hat h},{\hat l},g) \models \btt{WAIT(S)} & \!\!\! \btt{iff} \!\!\!
& {\forall} v_1{\ra}v_2 {\in} \codeE{S} {\cdot} (s,{\hat h},{\hat l},g) {\models} \btt{WAIT(\{v_1{\ra}v_2\})}\\

\!\!\! (s,{\hat h},{\hat l},g) \models  \btt{WAIT(\{v_1{\ra}v_2\})}  & \!\!\! \btt{iff} \!\!\!
& v1,v2 \in \myit{dom}(s) \wedge  (s(v1),s(v2)) \in g
\\
\!\!\! & &
 \wedge \myit{dom}({\hat h}) {=} \emptyset\\
\!\!\! & &{\wedge} (s(v1),\now),(s(v2),\now) \in \myit{dom}({\hat l})  ~{\wedge}\\
\!\!\! & &({\exists} k_1,k_2,b_1,b_2,\constr_1,\constr_2,\constr_1',\constr_2' \cdot \\
\!\!\! & & {\hat l}(s(v1),now) {=} \btt{CDL}(k_1,b_1, \inflow \constr_1,\outflow \constr_1') \\
\!\!\! & & {\wedge} {\hat l}(s(v2),now) {=} \btt{CDL}(k_2,b_2,\inflow \constr_2,\outflow \constr_2') \\
\!\!\! & & {\wedge} k_1{>}0 {\wedge} b_2{=}\btt{F}) \\


\end{array}
\]
\end{scriptsize}


==> thread.tex <==
\subsection{First-Class Threads}

%\input{exp-mapreduce}

%This section shows how flow-aware
%resource predicates can be used to support
%first-class threads.
Each thread is first created
from a method \codeE{f(\vlist{v})} that requires
precondition \code{P} and ensures postcondition
\code{Q}, as specified below:

\code{thrd~create\_thread(f)~\SPEC{with~P,Q}}\\
\indent\quad \SPEC{\requires~ \emp} \\%\qquad
\indent\quad
\SPEC{\ensures ~ \thrdpredone{\vlist{w}}{res}{P}{Q}{\vlist{v}};} %{\sm{\wedge}} \code{\res{=}t}

\noindent%
For simplicity, we require pre/post
to be explicitly declared, though this could
be inferred from the specification of \code{f} itself.
This method explicitly builds a resource predicate instance
\thrdpredone{\vlist{w}}{t}{P}{Q}{\vlist{v}} 
where
\codeE{\vlist{w}} denotes logically bound variables
that link precondition \code{P} with postcondition
\code{Q}. Note that this resource predicate has both
inflow (\codeE{{\OM}P}) and outflow (\codeE{{\OP}Q}) resources as arguments. 
%We use the flow annotation 
%\codeE{\OM} to denote an inflow (from the
%current thread) into the resource predicate,
%while annotation 
%\codeE{\OP} will denote an outflow 
%from the resource predicate
%(into the current thread). 
Resource predicates
with \underline{both} inflow and outflow resources are
effectively predicate transformers, used to model
methods. 
Once such a thread has
been created, the \code{fork} operation can be used to
start the thread, as denoted by the specification:

\code{void~fork(thrd~t,\vlist{v})} \\
\indent\quad%
\SPEC{\requires~ \thrdpredone{\vlist{w}}{t}{P}{Q}{\vlist{v}} {\sep} \code{P}}
\\
\indent\quad%
\SPEC{\ensures~ \thrdpredtwo{t}{Q};}


\noindent
which consumes the thread's precondition,
and yields another resource predicate
%\codeE{Thrd2(t,{\OP}Q)}. 
\thrdpredtwo{t}{Q}.
This new
predicate denotes a thread under execution,
whose postcondition \code{Q} is only made available, after
its thread has finished execution (or joined).
%% This specification of
%% fork is said to be {\em resource-preserving}, since
%% it never loses any incoming or outgoing resources. \scsay{Is it resource-preserving modulo 
%% the effect of the forked thread, namely \sm{\code{P}{\rightsquigarrow}\code{Q}}? I noticed
%% this is addressed later in 2nd paragraph of sec 2.1}
The specification of
the join operation is itself captured below, which 
would mark its thread as having completed
execution, through a \code{\dead{t}}
predicate.

\code{void~join(thrd~t)}\\
\indent\quad%
\SPEC{{\requires}~ \thrdpredtwo{t}{Q}}
\\
\indent\quad%
\SPEC{{\ensures}~  \code{Q} {\sep} \dead{\code{t}};}
\\
\indent\quad%  
\SPEC{{\requires}~ \dead{\code{t}}}
\\
\indent\quad%   
\SPEC{{\ensures}  \dead{\code{t}};}

If the thread is
already dead at the point of joining, its state
remains unchanged, as captured by the second
pair of pre/post specification.
Prior approaches, e.g. \cite{Dodds:POPL11},
that use concurrent abstract predicate for reasoning
have only considered the property of data-race freedom,
but have not considered 
%% the properties of 
{\em resource-preservation}
and {\em deadlock-freedom}. We present our solution to these
problems, initially in the context of modelling for
first-class threads.

\subsubsection{Ensuring Resource-Preservation}
%% \noindent{\bf Ensuring Resource-Preservation\qquad}
%% \noindent
\hide{%start-hide%
We intend to track all concurrency resources accurately
and flexibly.
We shall do it in three ways with classical
separation logic. 

Firstly, the flow annotations are important
for ensuring the soundness of our resource predicates,
since it can help ensure that all resources are being
tracked precisely, by the resource-preserving 
concurrency primitives.
%% For example,
%% each predicate \codeE{Thrd[w*](t,{\OM}P,{\OP}Q,v*)}
%% would denote a predicate transformer since it has both an
%% incoming \codeE{{\OM}P} and an outgoing \codeE{{\OP}Q}
%% resource. The fork operation itself would denote a primitive
%% that consumes some resource  \codeE{{\OM}P}, while 
%% the join
%% operation would denote a primitive that yields
%% (or produces) some resource  \codeE{{\OP}Q}. 
With this property, we can easily show
that every concurrency primitive always track
its resources in a precise manner.
}%end-hide%
%In the case of threads, both 
The \code{fork} and \code{join} primitives
are {\em resource-neutral} since the number of incoming and
outgoing resources are perfectly balanced. This classification
is \underline{not} possible if flow-annotations are not suitably 
marked for our resource predicates.
However, the \codeE{create\_thread} primitive has a
net resource of \codeE{\{{\OM}P,{\OP}Q\}} since the thread's
execution acts as a {\em predicate transformer}.
Note that the concept of resource preservation
is not contradicted by the presence of predicate transformer.
Resource preservation requires us to account for every
resource created, destroyed and transferred through communication
channels (or global memory). We can do so in
our specification logic by
disallowing ambiguous disjunction with 
different net resources. Two formulas (from a disjunction)
are ambiguous if their conjunction is satisfiable.
(This concept is related
to the notion of precise predicates.)

%Secondly, we 
We permit that incoming and outgoing
resources to be {\em flexibly split}, where possible.
This will allow us to support more
complex concurrency patterns. For example, to support
multi-join pattern where a thread may be joined
at multiple locations; we shall achieve it using a
split lemma that is
resource-preserving:

%\quad 
\SPEC{\thrdpredtwo{t}{(Q_1{\sep}Q_2)} \sm{\longrightarrow} \thrdpredtwo{t}{Q_1} {\sep} \thrdpredtwo{t}{Q_2}}

Lemmas for splitting resources have been
proposed before for concurrency reasoning. For example, \cite{Dodds:POPL11}
uses \codeE{P \sm{\wand} (Q{\sep}R)} to denote the ability for resource \code{P} 
to be split into two resources \code{Q} and \code{R}. Our paper clarifies the
importance of flow-aware resource splitting, and provides support
to enable splitting in scenarios that permits aggregated
commands. A list of commands \codeE{e_1,\ldots,e_n} can be 
aggregated into a single command \code{e} if the former 
\codeE{e_1,\ldots,e_n} can be replaced
by the latter \code{e}, without any change in its 
observable meaning. For example, two joins on the same thread
in a concurrent program can always be replaced by a single join at an
earlier forking point. Due to this aggregation property, we allow
split to occur for \code{\thrdpredtwo{t}{(Q_1{\sep}Q_2)}} whose
resources are needed for pre-conditions of multi-join operations.
%% In our flow-aware predicates, incoming resources are
%% captured via preconditions (of library primitives),
%% while outcoming resources are made available via 
%% postconditions (of library primitives).

%Lastly, with 
With the help of classical separation logic, we shall
further classify our resources into the following categories:

\begin{mydef}[Resource-Loaded]\label{def:loaded}
A {\RLoaded} predicate is a predicate which definitely captures
some resource. Each of its occurrences \underline{must}
be tracked precisely to
avoid resource leakage. Two examples of {\RLoaded} predicates
are 
%\codeE{Thrd2(t,{\OP}Q)}
\thrdpredtwo{t}{Q}
and %\codeE{Thrd[w*](t,{\OM}P,{\OP}Q,v*)}.
\thrdpredone{\vlist{w}}{t}{P}{Q}{\vlist{v}}.
\end{mydef}

\begin{mydef}[Resource-Less]\label{def:less}
A {\RLess} predicate is a predicate which no longer captures
any resources. 
An example of this predicate is  \code{\dead{t}}
which denotes a thread that has expired
(finished execution).
%% predicate which said to have expired\scsay{What does this mean?}.
Such a
predicate is also a pure predicate.
\end{mydef}

This classification can help ensure that
each {\RLoaded} predicate
%% such as \code{Thrd[w*](t,-P,+Q,v*)} and 
%% \code{Thrd2(+Q)},
is never lost by our classical reasoning system.
 %% given program unit.
In contrast, {\RLess} predicates,
like \code{\dead{t}}, can be lost as
they are classified
as pure predicates, with 
%% as denoted by 
the following idempotent lemma:

\quad \SPEC{\dead{t} \sm{\longleftrightarrow} \dead{t} {\sep}\dead{t}}

For each dead thread, we allow its {\RLoaded}
predicate with only outgoing resource to be
automatically released,
%% at the end of synchronization,
thus:
%% \begin{verbatim}
%%  Thrd2(t,-P) * Dead(t) --> Dead(t) * P
%% \end{verbatim}
%% \scsay{Should the above be +Q?}

\quad\SPEC{\thrdpredtwo{t}{Q} {\sep} \dead{t} \sm{\longrightarrow} \dead{t} {\sep} \code{Q}}

This is to help with resource-preservation when a
resource is known to have terminated.
We ensure that each lemma used is resource-preserving,
and the specification of each method used
be resource-precise with no ambiguous disjunction.
%% (unless they have equivalent net resources)

\subsubsection{Ensuring Deadlock Freedom}
%% \noindent{\bf Ensuring Deadlock Freedom\qquad}
%% \noindent
%We now consider how (intra-resource) deadlock errors 
%(from a single resource) are detected through the use of synchronization lemmas.
%In particular, e
Each {\RLoaded} predicate
with an incoming resource cannot co-exist
with its
{\RLess} predicate state, as highlighted below,
for each thread.
%%  since this would
%% denote a deadlock scenario, as follows: 
%\begin{verbatim}
% Thrd[w*](t,-P,+Q,v*) * Dead(t) --> ERROR
%\end{verbatim}

\quad \SPEC{\thrdpredone{\vlist{w}}{t}{P}{Q}{\vlist{v}} {\sep} \dead{t} \sm{\longrightarrow} \ERR}

%%Note that {\ERR} is distinct from \code{false},
%%since each of its occurrences would be flagged by our
%%verification, while \code{false} simply denotes unreachability.
%
%Furthermore, we refer to these as synchronization lemmas, 
%since these errors are meant to capture single-resource deadlock scenarios.
%In this example, it
\noindent
This is a deadlock caused by a \code{join} operation 
being invoked before the \code{fork} operation. It is
wrong to terminate a thread before it has even started.
Nevertheless, this synchronization scenario never arises in our current
modelling for threads, since the resource predicates are being
created in the following orders (based on usage protocol
specified via its pre/post):
\codeE{\thrdpredone{\vlist{w}}{t}{P}{Q}{\vlist{v}} 
\rightarrow \thrdpredtwo{t}{Q} 
\rightarrow \dead{t}}, where the third \code{\dead{t}}
could not have co-existed with the first uninitiated
\code{\thrdpredone{\vlist{w}}{t}{P}{Q}{\vlist{v}}}
for any thread \code{t}.
Any such deadlock
errors would have been detected as a pre-condition
failure 
%\codeE{Thrd2(t,{\OP}Q)}
for \code{join} which requires a \code{fork} to occur before
hand.
%% , since it has \code{\thrdpredtwo{t}{Q}} as its pre-condition. \scsay{It seems we are talking about
%% usage protocols  here. Is it right to say that desired protocols are implicitly implied by our pre/post?}
%% have
%% been executed.
%% never loses any of its resources.
%% \input{old-fig1-desc}
%% \scsay{The following requires revision to match the new example}


Inter-resource deadlocks may also have occurred,
as illustrated by our next example on two threads:

\begin{center}
\code{t1 = create\_thread(f1)}~\SPEC{\code{with}~\sm{\code{P}_1},\sm{\code{Q}_1}}; \\
\code{t2 = create\_thread(f2)}~\SPEC{\code{with}~\sm{\code{P}_2},\sm{\code{Q}_2}};

\code{\saying{\thrdone{}{t1}{P1}{Q1}{} {\sep} \thrdone{}{t2}{P2}{Q2}{}  }}
%% \hspace*{25mm}

\vspace{-12pt}
\[
{
\left(
\begin{tabular}{ l@{\extracolsep{\fill}}  || l@{\extracolsep{\fill}} }
%\code{\ldots} &~~\code{\ldots}\\
\code{\saying{\thrdone{}{t2}{P2}{Q2}{}}} &~~\code{\saying{\thrdone{}{t1}{P1}{Q1}{} }}\\
\code{join(t2);~~} &~~\code{join(t1);}\\
\code{\saying{pre-cond fails}} &~~\code{\saying{pre-cond fails}} \\
\code{fork(t1);~~} &~~\code{fork(t2);}\\
%\code{\ldots} &~~\code{\ldots}\\
\end{tabular}\right)\code{;}
}
\]

\end{center}

Here, waiting could only have occurred for \code{join}
commands. Inter-thread deadlock would have occurred in this scenario,
since each of the two \code{join} commands
is waiting for the other thread to
initiate the \code{fork} operation.
However, due to strict order of the three resource
predicates, such a scenario would have been detected
as a pre-condition failure for the \code{join} commands.
Hence, synchronization lemma
is not required for preventing deadlocks amongst multiple threads
due to its usage protocol.
%% In principle, if every wait
%% command (such as \code{join}) 
%% does not depend on an incoming-resource predicate,
%% we are guaranteed to prevent deadlocks via pre-condition
%% failures, rather than through via the synchronization lemma.
%% Hence, 
Once verified, we guarantee our thread resources to
be deadlock-free.

\hide{%%% no need the following%%%
\subsubsection{A Map-Reduce Example}

We now illustrate an example of
multi-join concurrency pattern
%% with a program
in Fig.~\ref{fig:mapreduce}, based on the map/reduce
paradigm.
%%  shows a C-like program posing challenges
%% to existing verification systems.
In this program, the \code{main} thread
concurrently forks three threads: a mapper \code{m} to
produce two lists, and two reducers \code{r1} and \code{r2} to process
a list each. Both the reducers each take \code{m} as 
a parameter and joins it at an appropriate place to
recover their respective lists from \code{m}.
The main thread subsequently joins up the two
reducers before completing its execution.
%% executing the procedure \code{main}
%% %% (called \code{main} thread)
%% forks a new thread \code{t1} executing the procedure \code{thread1}.
%% \code{thread1} will swap the values of the cells
%% \code{x} and \code{y}.
%% \code{main} then forks another thread \code{t2} executing the procedure \code{thread2}
%% with \code{t1} passed as one of its arguments.
%% Afterward, \code{t2} will join with \code{t1}
%% and manipulate the cell \code{y}, while \code{main}
%% will also join with \code{t1} but manipulate the cell \code{x}.
%% In separation logic, a heap node $\code{\permsto{x}{cell(vx)}{}}$
%% represents the ownership of an object of type $cell$
%% pointed to by $x$ and having the field \code{val} of $vx$
%% (called ownership of $x$ for short).
%% %% represents the fact that $x$ points to an object of type $cell$
%% %% having the field \code{val} of $vx$.
The program is challenging to verify 
because (i) fork and join operations on the mapper \code{m} are
non-lexically scoped 
%% (i.e. they are in different scopes)
(i.e. \code{m} is forked in \code{main} but joined in threads
\code{r1} and \code{r2}), and
(2) part of the computed resources from \code{m} is made
available to \code{r1}, while another part is made available to \code{r2}.
This concurrency  pattern is referred to as
a multi-join. 
%% Therefore, 
In this program,
the ownerships of two lists produced by the mapper must be
flexibly transferred across thread boundaries,
%% between \code{main}, \code{t1} and \code{t2}, 
via fork/join calls.
To the best of our knowledge, we are not aware of
any existing approaches capable of verifying this program.
%% The program can be verified soundly and modularly by our proposed
We propose 
``\myit{flow-aware resource predicates}''
to verify such programs soundly and modularly.
The key points to handle this program are (1) considering
the executing thread of
\code{m} as flow-aware resource predicate, and (2) allowing its expected
output to be
split and transferred between \code{main}, \code{r1}
and \code{r2} via fork/join calls.
%
%% Our approach is based on the following observation:
%% when a thread (joiner) joins with another thread (joinee),
%% the joiner expects to receive (in order to later read or write)
%% certain resource transferred
%% from the joinee.
%%
%% In the example program, \code{main} joins with \code{t1}
%% and expects the ownership of \code{x} transferred from \code{t1},
%% while \code{t2} joins with \code{t1}
%% and expects the ownership of \code{y}.
%% Hence, the verification of the program in Fig.~\ref{fig.example}
%% is achieved by introducing the thread ownership
%% %$\permsto{\term{v}}{ \thread{\constr} }{}$ 
%% \thrdpredtwo{v}{\sm{\constr}}
%% indicating that
%% $\code{v}$ points to a possibly live thread (as resource) carrying certain resource
%% $\sm{\constr}$.
%% %% (i.e. the resource obtained after the thread is joined).
%%
\hide{%%%
A thread having the ownership \thrdpredtwo{v}{\sm{\constr}}
can perform a \code{join(v)}, and yield the resource
$\constr$ and a pure predicate $\dead{v}$ after joining.
This special predicate
$\dead{v}$ explicitly
indicates that thread $\code{v}$ is no longer alive.
%% has already finished its execution.
In Fig.~\ref{fig.example},
when \code{m} is forked (line~22),
its pre-condition is consumed and
exchanged for the thread's ownership
%$\permsto{t1}{\thread{ \permsto{x}{cell(2)}{} \sep  \permsto{y}{cell(1)}{} }}{}$
\thrdpredtwo{t1}{(\permsto{x}{cell(2)}{} \sep  \permsto{y}{cell(1)}{})}
carrying the post-state of \code{thread1} (i.e. \code{t1}'s state after
it has finished its execution). }
%% This is sound and modular as
%% other threads can only observe the post-state of \code{thread1}
%% when they join with \code{t1}.
%% Our approach enables the thread's ownership to be split into
%% %$\permsto{t1}{\thread{ \permsto{x}{cell(2)}{} }}{}$
%% \thrdpredtwo{t1}{\permsto{x}{cell(2)}{}}
%% and %$\permsto{t1}{\thread{\permsto{y}{cell(1)}{} }}{}$
%% \thrdpredtwo{t1}{\permsto{y}{cell(1)}{}}
%% (from line~23 to line~24). This allows the latter to be transferred
%% to \code{t2} while the former remains with \code{main}.
%% %% A thread having the ownership $\permsto{\term{v}}{ \thread{\constr} }{}$
%% %% can perform a \code{join(v)} and obtain the resource
%% Consequently, having the ownerships of \code{t1}, both \code{t2} and \code{main}
%% can perform \code{join(t1)} and get the corresponding resource:
%% \code{t2} obtains the ownership of \code{y} to write to it,
%% while \code{main} obtains and writes to \code{x}
%% (i.e. \code{t2} and \code{main} write-share the resource
%% transferred from \code{t1}).
%% After join, \code{t2} writes to the
%% cell \code{y} while \code{main} writes to the cell \code{x}
%% (i.e. \code{t2} and \code{main} write-share the resource
%% transferred from \code{t1}).
Using our flow-aware predicates,
%% threads as resource'' approach, 
the program
can be verified as both data-race-free and 
resource-preserving.
%
\hide{%%%
Our treatment
%% of ``threads as resource'' 
allows 
the ownership
of a thread to be flexibly split and transferred. For example,
in a program similar to
%% that in 
Fig.~\ref{fig.example},
instead of having exclusive accesses to the two
lists for 
%% writing to cells \code{x} and \code{y},
%% after joining with \code{t1},
\code{r1} and \code{r2}, we may share
the two lists to concurrently read 
%% (i.e. read-share)
the value of itscells. Using fractional permissions
\cite{Boyland:SAS03}, we could now
split the ownership of \code{m} from
%% , i.e.
\thrdpredtwo{m}{?}
into
\thrdpredtwo{m}{(?{0.6})}
and\\
\thrdpredtwo{m}{(?{0.4})},
and transfer them into the corresponding codes
for \code{r1} and \code{r2}.
This allows \code{r1} and \code{r2} to
read concurrently the cells the two lists
after joining with the \code{m} thread.
}%

%% In summary, we propose to treat threads as resource, thus allowing
%% threads' ownerships to be soundly split and transferred across
%% procedure and thread boundaries. 
%% This supports first-class threads
%% and enables modular reasoning of intricate concurrent programs
%% with non-lexically-scoped fork/join and multi-join.
%% We will give more details in the rest of this paper.

}%%%end of hide (no need the following)%%%

\hide{%%%%no need%%%

\subsubsection{Soundness}
\label{sec:soundness-thread}

Thread's \code{fork/join} is similar to {\CDL}'s
\code{coundDown/await}
in the following ways. In terms of resource flows,
a \code{fork} can be modeled as a \createlatch{} initialized
to 1 and immediately followed by a \code{countDown}, allowing
resource to inflow from the forker to the forkee's
thread abstraction.
A \code{join} is similar to an \code{await}, where
resource outflows from the joinee thread's abstraction
to the joiner.
Therefore, we extend the tagged memory model $\fpstate$
with a thread pool:

$ \fpstate \defs \pstack \times \fpheap \times \fpCDL \times \pgraph \times \fpthreads$

 $\fpthreads \defs \tids \times \ptagset \rightharpoonup \btt{THRD}(\tstates \times \flow \cdlR)) $

{\noindent} where $\tids$ is the set of unique thread identifiers
and $\tstates \defs \set{\btt{C},\btt{F},\btt{D}}$ is the set
of threads' states ($\btt{C}$ = created, $\btt{F}$ = forked,
and $\btt{D}$ = dead). The composition of threads can be defined
as the composition of its flow-aware resources, in a similar
way to CDLs.
However, the critical difference between threads
and CDLs is that while CDLs guarantee
that the inflow resource
is the same to the corresponding outflow resource,
the predicate transformer nature of threads does not give
such guarantee, but this occurs only at the {\createthrd}
command.
%%  have such a guanrantee
%% (since spawn threads can dispose
%% or create new resources). 
However, threads does guarantee race freedom
and resource-preservation for the \code{fork}
and \code{join} primitives.
As a result, we can freely use the resource-preserving
behaviour of the split lemmas.
%% since the inflow resource is consumed
%% by the abstraction and the outflow resource
%% can be soundly introduced by the sound
%% flow-aware split rules
%% (i.e. thread's execution acts as a predicate
%% transformer).

}%%%end of hide (no need)%%%


==> threadsasresource.tex <==
\subsection{Forward Verification Rules}

Our verification system is built on top of entailment checking:
\savespace
\begin{equation*}
\entailS{\D_A}{\D_C \rewrite \D_R}
\savespace
\end{equation*}

\noindent
%% Intuitively, 
This entailment checks if antecedent $\D_A$ is precise
enough to imply consequent $\D_C$, and computes the residue $\D_R$ 
for the next program state. For example:\morespace

$\entailS{\permsto{x}{cell(1)}{0.6} \sep  \permsto{y}{cell(2)}{0.6}}{\permsto{x}{cell(1)}{0.6}~ \rewrite ~\permsto{y}{cell(2)}{0.6}} $\morespace

\input{fwdrules}

Fig.~\ref{fig:fwdrules} presents our forward verification rules.
Here we only focus on three key constructs
affecting threads' resource:
%% statements
%% that enable ownership transfers: 
procedure call, fork, and join.
Forward verification is formalized using Hoare's 
triple
for partial correctness:
%% the form 
$\{ \constr_{pr} \} P \{ \constr_{po} \}$.
Given a program
$P$ starting in a state satisfying the pre-condition $\constr_{pr}$,
if the program terminates, it will do so in a state satisfying
the post-condition $\constr_{po}$.

In order to perform a procedure call (\entrulen{CALL}),
the caller should be in
a state $\D$ that can entail the pre-condition $\constr_{pr}$
of the callee (i.e the procedure $pn$).
$spec(pn)$ denotes the specification of the procedure $pn$.
For conciseness, we omit
the substitutions that link actual and formal parameters
of the procedure prior to the entailment. After the entailment,
the caller subsumes the post-condition $\constr_{po}$ of the callee
with the residue $\D_1$ to form a new $t{-}consistent$ state $\D_2$.
Ownerships are transferred across procedure boundaries,
from the caller to the callee via the entailment of the pre-condition
and from the callee to the caller via the spatial
conjunction 
%% subsumption 
on the post-condition.

Similarly, when performing a fork (\entrulen{FORK}),
the forker should be in
a state $\D$ that can entail the pre-condition $\constr_{pr}$
of the forkee (i.e the newly-created thread executing the procedure $pn$).
Afterward, a new thread node
$\permsto{\term{v}}{ \thread{\constr_{po}} }{} $
carrying the post-condition $\constr_{po}$ of the forkee is created.
The thread node is then combined with the residue 
$\D_1$ to form a new $t{-}consistent$ state $\D_2$.
The thread node is considered as resource in $\D_2$;
hence, it can be flexibly split and transferred in subsequent
parts of the program.
The \entrulen{FORK} rule is sound since other threads can only observe
the post-state of the forkee when joining with it.
It also ensures modularity as the forker
only knows the pre/post-conditions of the forkee.

When joining a thread (\entrulen{JOIN-1}), the joiner simply
exchanges the thread node, which carries a resource $\constr_{po}$,
with the resource itself.
Each joinee could be joined by multiple joiners.
Our verification rules are based on
the observation that when a joiner joins with a joinee,
the joiner is expecting to receive certain resource transferred
to it from the joinee. Hence, each joiner will receive
the current resource carried by the thread node.
After a thread has been joined, it becomes dead
(indicated by the pure {\em{dead}} predicate).
Joining a dead thread is equivalent
%% considered as 
to a no-op
(\entrulen{JOIN-2}).
 %% (for both verification and run-time execution).

Using our verification rules, a \entrulen{CALL}
can be modeled as a \entrulen{FORK} immediately
followed by a \entrulen{JOIN}. As threads are considered
as resource, fork and join operations can be in different
lexical scopes and thread nodes can be transferred across
procedure and thread boundaries. Furthermore, if there is a
recursive fork call in a procedure (also called nested fork)
such as the parallel Fibonacci program\footnote{Available on \toolurl},
the verification proceeds normally: a new thread node
corresponding to the newly-created thread executing
the procedure is created. Therefore, in our system,
a nested fork is handled in the same way as a normal fork.

\hide{spec(PT) means the specification of procedure pn.
This ensure encapsulation (no code is required)}

%\savespace
\subsection{Manipulating ``Threads as Resource''}
\label{sec:tas}

The notion of ``threads as resource'' plays a critical
role in our approach as it enables threads to be treated
in a similar way as other objects: a thread node
can be created, stored, split, and transferred (or shared)
among multiple threads,
allowing them to join and to receive suitable resource
after joining.

\input{perm-rules}

Our sub-structural rules for manipulating resource
are presented in Fig.~\ref{fig:perm-rules}.
%
\hide{The first part rearranges resource in a separation
logic formula into equivalent forms.}%
We denote resource equivalence as $\Longleftrightarrow$.
By resource equivalence, we mean that the total resource
on the left and the right sides of $\Longleftrightarrow$ are the same.
Our approach allows resource to be split, combined,
and transferred across procedures and threads,
while it guarantees that the total resource remains unchanged.
The rearrangement
rules \entrulen{R-DISJ}, \entrulen{R-CONJ}, \entrulen{R-SCONJ},
and \entrulen{R-EMP} are straightforward. With fractional
permissions $\fracperm$, heap nodes
can be split and combined in a standard way (\entrulen{R-FRAC}).
The left-to-right direction indicates permission splitting
while the right-to-left indicates permission combining.
We also allow thread nodes to be split and combined
(\entrulen{R-THRD1}). Splitting a thread node (left-to-right)
will split the resource carried by the node while combining
thread nodes (right-to-left) will combine the resource of
the constituent nodes.
%
\hide{%%
Fractional thread nodes can always be rearranged into
non-fractional forms (\entrulen{R-THRD2}). The rule
\entrulen{R-THRD2} requires a separation logic formula to
be multiplicative, as explained in the multiplication rules
of Fig.~\ref{fig:perm-rules}.
\khanh{\entrulen{R-THRD2} and multiplication rules could
be redundant}
}%%

\hide{
An example of equivalence via sub-structural rules is illustrated
in Fig.~\ref{fig.equiv}. In the figure, we gently
abuse the notation, e.g. we use
$\stackrel{\text{\ensuremath{\entrulen{M-FRAC},\entrulen{R-THRD1}}}}{\Longleftrightarrow}$
to indicate that the resource equivalence $\Longleftrightarrow$
can be obtained using the rule \entrulen{M-FRAC} and then \entrulen{R-THRD1}.

\input{fig-equiv}
}

\hide{

%% \savespace
%% \subsection{Soundness}
%% \savesmallspace
{\noindent \textbf{Soundness.}}
We discuss the soundness of our
``threads as resource'' approach with respect to the
language described in Section~\ref{sec:proglang}.
%% operational semantics defined in Appendix~\ref{sec:semantics}.
The soundness of our approach is
%% could be 
proven by adapting
the proof presented in \cite{Gotsman:APLAS07} to additionally
allow for multi-join and ``threads as resource".
%% The adaptation is not a difficult task as the soundness of
%% a 
The soundness of permission-based resource logic must ensure 
that the total number of permissions
on each heap object never exceeds the full permission
(i.e. 1 in the fractional permission system~\cite{Boyland:SAS03}).
At any time, at most one thread can write to a heap object,
and when a thread has a read permission to a heap object,
all other threads similarly hold
%% holding a permission to the heap object
%% must have a 
read permissions as well.
This ensures that verified programs are data-race free.
%% Hence, 
To guarantee soundness, we show that our
approach neither invents new resource nor destroys
existing resource.
 %% in a program while it
Moreover, it guarantees that the total resource of the program
is not changed by our verification rules.
%% remains unchanged.

\savesmallspace
\begin{lmm}[Conservation of Total Resource]\label{lmm:soundness}
The total resource of a program
is unchanged under ``threads as resource'' verification
approach.\savespace
\end{lmm}

\begin{proof}
Except for fork and join,
%% Intuitively, except ``threads as resource'' (i.e. thread nodes),
the verification rules in Fig.~\ref{fig:fwdrules}
and sub-structural rules in
Fig.~\ref{fig:perm-rules}
neither invent new resource nor destroy existing resource.
\hide{A program can leak resource, but only when users deliberately
intend to do so.}
%% Each thread node is created to carry an existing resource, 
%% and neither lose nor add new resources.
%% either
%% invent or destroy it.
Hence, this soundness property can be proven
%% obtained
by induction on the sub-structural rules
(Fig.~\ref{fig:perm-rules}).
{\qed}
\end{proof}\savespace\savespace

%% \todo{emphasize somewhere that a verified program is race-free
%% and functionally correct}

%% \hide{Dinh luat bao toan resource: resource ko tu sinh ra va
%% cung ko tu mat di. No chi chuyen tu thread nay sang thread khac.}
} %%END HIDE

\subsection{Soundness}
\label{sec:tar:sound}
\input{soundness}


==> trace.tex <==
\paragraph{Syntactic traces}

%% \khanh{TODO: extend with thread identifier
%% to define traces of programs with dynamic threads}

%% \khanh{cannot define nodeadlock(c1,c2) since
%% deadlock may involve more than 2 threads}

We adopt the interleaving semantics based on
action traces, which was proposed in \cite{Calcagno:LICS2007}.
Traces $T(P)$ of a program $P$ is a set of sequences
of actions $\alpha \in$ $\{ c,$ $\btt{norace}(c1,c2),$ $\btt{DLF}(p1,p2) \}$ for
all atomic primitives
$c$, $c_1$, $c_2$, and  non-atomic code $p_1$, $p2$.
Trace semantics of important commands are defined as follow:

\begin{scriptsize}
\[
\begin{array}{l}
T(\alpha) {=} \{ {\alpha} \}
\qquad
T(p^*) {=} (T(p))^*
\quad
T(p_1 ; p_2) {=} \{ tr_1; tr_2 \mid tr_i \in T(p_i) \}\\

T(p_1 + p_2) {=} T(p_1) \bagunion T(p_2) \\


T(p_1 || p_2) {=} \{tr_1 ~ zip ~ tr_2;\btt{DLF}(p1,p2) \mid tr_i \in T(p_i) \} \\

(c_1 ; tr_1) ~ zip ~ (c_2 ; tr_2) {=} \\
\myspace \btt{norace}(c_1,c_2);
( (c_1 ; (tr_1 ~ zip ~ (c_2 ; tr_2))) \bagunion
  (c_2 ; ((c_1,tr_1) ~ zip ~ tr_2))
)

\end{array}
\]
\end{scriptsize}

Parallel composition $||$ is a set of
syntactic interleaving of primitives, generated
by $zip$.
The deadlock-freedom check $\btt{DLF}(p_1,p_2)$ is placed
at the end to make sure that
the parallel composition does not result in deadlocks.
Intuitively, $\btt{DLF}(p_1,p_2)$ checks if the corresponding wait-for graphs
of $p_1$,$p_2$ can be composed,
i.e. the resulting the wait-for graph is acyclic.
Similarly, all racy programs are also forced to fault ($\top$)
by placing the check $\btt{norace}(c_1,c_2)$ for each
pair of primitives $c_1$ and $c_2$ which
may happen in parallel. Intuitively, $\btt{norace}(c_1,c_2)$
checks if $c_1$ and $c_2$ can execute on disjoint
portions of a state and they do not create
cycles in the state's wait-for graph.

\paragraph{Semantics of Traces} Denotational semantics of traces
is defined as the composition of the interpretation of
actions.
Interpretation of a primitive, \interpret{$c$}, is simply its specification
interpreted over program states $\pstate$ (more details
are discussed in Section~\ref{sec:proof}).
%% \khanh{need to define these}
The semantics of $\btt{DLF}(p_1,p_2)$ and
$\btt{norace}(c_1,c_2)$ 
are the local functions
$\btt{DLF}(\interpret{$p_1$},\interpret{$p_2$})$
and
$\btt{norace}(\interpret{$c_1$},\interpret{$c_2$})$
defined as follows:

\begin{scriptsize}
\begin{equation*}
\btt{DLF}(f_1,f_2)(\fstate) \defs 
\begin{cases}
    \set{\fstate}& \!\!\!\!\!\! ,~\btt{if} ~ \exists \fstate_{\!f_1}=(\_,\_,\_,g_1), \fstate_{\!f_2}=(\_,\_,\_,g_2) \cdot \\
    & ~~~~~acyclic(g_1 {\bagunion} g_2) \wedge \fstate_{\!f_1} \bullet \fstate_{\!f_2} {=} \fstate \\
    & ~~~~~\wedge f(\fstate_{\!f_1}) {\neq} \top \wedge g(\fstate_{\!f_2}) {\neq} \top \\
    \top & \!\!\!\!\!\! \text{,~otherwise}.
  \end{cases}
\end{equation*}
\end{scriptsize}


\begin{scriptsize}
\begin{equation*}
\btt{norace}(f_1,f_2)(\fstate) \defs 
\begin{cases}
    \set{\fstate}& \!\!\!\!\!\! ,~\btt{if} ~ \exists \fstate_{\!f_1}, \fstate_{\!f_2} \cdot \fstate_{\!f_1} \bullet \fstate_{\!f_2} {=} \fstate \\
    & ~~~~~\wedge f(\fstate_{\!f_1}) {\neq} \top \wedge g(\fstate_{\!f_2}) {\neq} \top \\
    \top & \!\!\!\!\!\! \text{,~otherwise}.
  \end{cases}
\end{equation*}
\end{scriptsize}

Based on the above semantics, the soundness
of the parallel composition can be easily derived:
$\denote{ $P_1 || P_2$}(\state_1 \bullet \state_1)
\sqsubseteq \denote{ $P_1$}(\state_1) \sep
\denote{ $P_2$}(\state_2)$. In other words,
parallel threads work on disjoint memory states
and the resulting wait-for graph is acyclic.
However, this semantic modelling is insufficient 
for the class
of programs that we are considering
%% in this paper,
where resources can be flexibly ``flowed''
among threads (e.g. via latches).
Therefore, we need a more precise semantics
to capture the resource exchanges
carried out by concurrency synchronization
mechanisms.
%% -aware semantics.

%% Define nodeadlock(tr) where tr is a trace \khanh{how?}

\paragraph{Model of Synchronization}

The flow-aware semantics that we shall discuss in
subsequent parts is based on 
%% Jules et al.
Villard et al. \cite{Villard:APLAS09}
where they successively refine the basic
semantics. The key idea is to record
the history of all post synchronizations
including the content of the resources transferred.
In the context of CDL, we associate memory heaps
with flow-aware tags, indicating
which CDLs flow the heaps and the direction
of the flow. Specifically,
\code{countDown(c)} operations associate
the heaps with inflow tags $\inflow \mytag$ since
it is to transfer the heaps from the current thread
to the CDL abstraction. In contrast, \code{await(c)}
operations associate the heaps with
outflow tags $\outflow \mytag$
since the heaps are transferred from
the CDL abstraction to the current thread.
Then, the whole program is considered.
We restrict program states to legal
states (also called well-formed
tagged memory states) where
\code{await} operations
can only happen when a predefined
number of \code{countDown} operations
has reached. In other words,
based on flow-aware tags,
the content that \code{await} operations
outflow must match the content that
\code{countDown} operations inflow.


\hide{

Global semantics: restrict states produced by a primitive to
\myit{legal} ones.

\paragraph{Synchronization}

Legal states are those such that 
outflow primitives must have produced less than
what its peer-inflow primitive(s) consumed.

CountDownLatch: number of countDown() >= count
(or count=0)

Thread: state = dead.

This could also indicate blocking of outflow primitives
where there isn't enough pending resource for
outflow primitives to produce.

Well-separated flow could ensure race freedom \khanh{TOCHECK}.

\paragraph{Communication}

Inflow resources match outflow resources 
(with predicate transformer in mind)

Tagged with (timestamps, flow type)

We may not need timestamps since
it is used to differencitate different msg.
Our CDL and fork/join is non-reusable.

Legal states: sum(in) = sum(out)

countDown() : deallocate inflow resource
P, allocate the log [t,in]P

await() : allocate outflow resource P,
allocate the log [t,in]P

History-preserving (refined) memory model and semantics of Hoare's triple

} %%END HIDE

